A Comprehensive Study of Native Code Bugs in Python Applications

The impact of Python applications has been evidenced by their widespread presence in some of the most impactful software domains, such as machine learning frameworks and scientific computing platforms. These applications often integrate native code components written in a lower-level programming language like C. This multilingual construction brings various benefits such as greater performance efficiency and easier interoperability with diverse runtime environments. However, bugs in the native code (i.e., native code bugs), which are usually stealthy, also constitute a major additional challenge to the quality of the Python applications as a whole. Yet despite existing relevant studies, there remains a lack of comprehensive understanding of native code bugs in Python applications. In this paper, we aim to mitigate this knowledge gap through the first in-depth study of such bugs, dissecting their common symptoms, introducing locations, manifestation characteristics, root causes, and fixes. Based on our extensive automated and manual analyses of 216 native code bugs in real-world Python projects on GitHub, we obtained novel findings about and new insights into the occurrence mechanisms and resolution strategies of those bugs.

==> RQ-fix-cai.tex <==
\vspace{-10pt}
\subsection{RQ5: Fixing Strategies of Multilingual Bugs}\label{RQ5}
%Our study comprehensively showcases the fixing strategies for bugs.
%
%From the 216 MLBF commits, we focused on the prior-commit (i.e., buggy) version of the respective code to understand each bug for answering the previous four RQs. 
%We further analyzed how these bugs were fixed based on the post-commit (i.e., fixed) versions. 
%
We further analyzed how the studied multilingual bugs were fixed based on the 
fixed versions of respective code according to the confirmed MLBF commits. 

\subsubsection{Fix Location}
%Among the total of 216 cases,  a significant majority (214 cases) 
Almost all (214) of the 216 multilingual bugs were fixed within a function. 
%, while only a small portion (2 cases) were fixed outside of a function. 
In the other two cases, the bug was fixed outside of any 
function---specifically pertaining to changes in function/variable and {\tt struct} declarations. 
This suggests that most of the bug fixes required adjustments within specific functional units of code, indicating that the majority of these bugs were localized (at the function level) and context-dependent. 
%In contrast, the few bugs fixed outside of functions pertained to broader structural or definition issues in the code, indicating a scope that extends beyond local functional contexts.
In particular, such contexts include the following 7 categories: 

%The following are the categories of bug-fixing locations:
\ul{Cross-language API callsite (77).} 
These bugs were fixed right where a cross-language API is invoked. 
The specific bug-fixes were to address misuse of the API due to 
differences in data types, conventions, and syntax between the two languages. 

\underline{If structure (36).} 
%This points towards logical errors 
These fixes are located within %{\tt if} 
conditional structures. Different from the "conditional expression" and "true/false branch" bug-fixing locations, these fixes involve the whole {\tt if} statement, rather than only a conditional or one of the branches. 
For instance, both the conditional and the {\tt else} body were fixed. 
%This could mean an incorrect or incomplete condition, or perhaps problems within the block of code to be executed if the condition is met.

\underline{Conditional expression (27).} 
Fixing these bugs required changing a conditional expression. 
In particular, the changes were to correct a misused variable within a predicate 
in that expression or a mistaken logical operator. 
%These bugs arise in conditional expressions. Issues here could include logical errors, or possibly the use of incorrect variables or data types.

\underline{True/false branch (19).} 
In these cases, the bug fix was constrained in one of the two branches of an {\tt if} conditional structure. 
The fix involved various code changes, mainly addressing logic errors and correcting incorrect assumptions. 
%This could imply bugs in the blocks of code that get executed based on a condition's truth value. They might have resulted from logic errors, incorrect assumptions, or other mistakes in these specific branches.

\underline{Function call (19).} 
These bug fixes were right on a callsite. 
While the callee is not a cross-language function/API, it is 
on the cross-language information flow path responsible for the bug. 
The fixes mainly addressed incorrect arguments. 
%Bugs here were fixed at the location of a function call. This could indicate issues with how the function was called, such as the use of incorrect arguments, or problems with the function's definition itself.

\underline{Whole function (12).} 
These fixes were changes to an entire function (i.e., typically across multiple code lines within that function).  
%suggesting significant issues with the function's logic, structure, or perhaps its interaction with the rest of the code.

\underline{Assignment (12).} 
In such cases, the bug was fixed by changing an assignment statement. 
Particularly, the changes involved correcting misused variable names or names and 
incompatible data types. 
%Bugs here were fixed at variable assignment statements. Problems could include the use of incorrect values, incorrect variable names, or incompatible data types.

%\underline{Other (12):} This category likely includes a variety of less common bug locations not captured by the other categories, e.g., asset, loop body, etc.
While the types of code locations of %multilingual bug 
fixes are generally similar to those of bug-introducing locations ($\S$\ref{RQ2}), the distribution of the locations over the bugs is notably different from that over the fixes. 
In particular, while 47 of the bugs were introduced at cross-language API function/API callsite, 77 of the bugs were fixed at that kind of locations, meaning many other %(albeit not necessarily 30) 
bugs that occurred at other kinds of locations were also fixed by correcting a 
cross-language function call. 
Similarly, fixing conditional expressions enabled patches of not only bugs introduced in those kinds of places but also others. 

\subsubsection{Bug-Fixing Approach}
Across the above kinds of locations (i.e., \textit{where} the fixes were made), we further looked into the kinds of code changes involved in the fixes (i.e., \textit{how} the fixes were made). 
We found four major types of such code changes: % (i.e., fixing approach): 
%In terms of the approaches to fixing these multilingual bugs, we found four major strategies: 

\ul{Use appropriate data types and casting (15).} 
In these fixes, the changes made were primarily about correcting data type errors, including the use of strong type conversion (casting). For example, using an integer variable in the native language (C) to hold floating-point data passed from the foreign language (Python) led to data-corruption bugs. The 
fix was to use the right data type (i.e., {\tt float}). 
%number is needed can cause precision loss. 
%Therefore, always use the correct data type that suits the requirement. Also, be careful when casting between types. Always check if the cast is valid before performing it.

\ul{Add missing checks or input validations before critical operations (13).} 
This approach involved checking/validating against null pointers, container (e.g., array) boundaries, and (logically) invalid values, among similar situations. 
Such checks/validations guard critical operations such as pointer dereferencing, array indexing, and arithmetics (e.g., division). 
%Before performing operations that can potentially crash your program or cause unexpected behavior, you should always check the inputs. For instance, before accessing a key in a dictionary, make sure the key exists. Before performing division, check if the denominator is zero. These checks help prevent exceptions from being thrown during runtime.


\underline{Fix logical errors in conditions or loops. (9)} 
%Logic errors are hard to catch because the program doesn't crash; it just doesn't produce the expected output. Logic errors can be present in condition checks, loop iterations, or algorithm implementations. Always validate your logic with different test cases to catch these bugs. 
Bugs fixed by this strategy were generally caused by logic errors (one of the primary types of root causes as discussed earlier). 
One common instance of this approach in our study was to \textit{replace a misused cross-language API with a correct one}, which was used to fix 35 of the bugs. 


\underline{Handle errors and exceptions properly (6).} 
These fixes concerned adding or fixing error/exception handling logic. 
In contrast to the approach above, which aims to prevent failures in critical operations from happening (hence adding checks/validations \textit{before} a critical operation is launched), 
this approach focuses on properly dealing with consequences of possible failures with a critical operation \textit{after} the operation has occurred. 
The most typical example of this approach in our study was to 
\textit{change the condition against a foreign function call return value}, as used for fixing 23 of the bugs. 

%after (e.g., calling a foreign function that may return a value indicating failure in the function) 

%It's important to handle errors gracefully in your code. In critical operations, your program should not proceed if an error occurs. Instead, it should exit gracefully or move to a safe state.







==> RQ-fix.tex <==
\subsection{Fixing Strategy}\label{RQ5}
Our study comprehensively showcases the fixing strategies for bugs.

\subsubsection{location}
Among the total of 216 cases,  a significant majority (214 cases) were fixed within a function, while only a small portion (2 cases) were fixed outside of a function. The two cases fixed outside of a function specifically pertained to 'function/variable declarations' and 'struct declarations'. This suggests that most of the bug fixes required adjustments within specific functional units of code, indicating that the majority of these bugs were localized and context-dependent. In contrast, the few bugs fixed outside of functions pertained to broader structural or definition issues in the code, indicating a scope that extends beyond local functional contexts.

The following are the categories of bug-fixing locations:
\ul{Cross-language API call site (77):} These bugs were fixed at points in the code where an API call crossed language boundaries. Such issues could arise due to differences in data types, conventions, or syntax between the languages, or misunderstanding about how an API function behaves when called from a different language.

\underline{If structure (36):} This points towards logical errors within 'if' conditional structures. Different from the "conditional expression" and "true/false branch" bug-fixing type, this fix involves the whole if structure not only a conditional statement or if branch. This could mean an incorrect or incomplete condition, or perhaps problems within the block of code to be executed if the condition is met.

\underline{Conditional expression (27):} These bugs arise in conditional expressions. Issues here could include logical errors, or possibly the use of incorrect variables or data types.

\underline{True/false branch (19):} This could imply bugs in the blocks of code that get executed based on a condition's truth value. They might have resulted from logic errors, incorrect assumptions, or other mistakes in these specific branches.

\underline{Function call (19):} Bugs here were fixed at the location of a function call. This could indicate issues with how the function was called, such as the use of incorrect arguments, or problems with the function's definition itself.

\underline{Whole function (12):} These bugs required changes to an entire function, suggesting significant issues with the function's logic, structure, or perhaps its interaction with the rest of the code.

\underline{Assignment (12):} Bugs here were fixed at variable assignment statements. Problems could include the use of incorrect values, incorrect variable names, or incompatible data types.

\underline{Other (12):} This category likely includes a variety of less common bug locations not captured by the other categories, e.g., asset, loop body, etc.



\subsubsection{Bug-fixing approach}

\ul{Add missing checks or input validations before critical operations:} Before performing operations that can potentially crash your program or cause unexpected behavior, you should always check the inputs. For instance, before accessing a key in a dictionary, make sure the key exists. Before performing division, check if the denominator is zero. These checks help prevent exceptions from being thrown during runtime.

\underline{Handle errors and exceptions properly:} It's important to handle errors gracefully in your code. In critical operations, your program should not proceed if an error occurs. Instead, it should exit gracefully or move to a safe state.

\underline{Use appropriate data types and casting:} Using the wrong data type can cause bugs. For example, using an integer variable when a floating-point number is needed can cause precision loss. Therefore, always use the correct data type that suits the requirement. Also, be careful when casting between types. Always check if the cast is valid before performing it.

\underline{Fix logical errors in conditions or loops:} Logic errors are hard to catch because the program doesn't crash; it just doesn't produce the expected output. Logic errors can be present in condition checks, loop iterations, or algorithm implementations. Always validate your logic with different test cases to catch these bugs. 




==> RQ-introducing-location-cai.tex <==
\subsection{RQ2: Bug Introducing Locations}\label{RQ2}
At a high level, 
%In terms of high-level structural/syntactic contexts, 
the studied multilingual bugs were introduced either within a function or outside any function. 
%in terms of coarse syntactic context. 

\subsubsection{Within Function} 
For the bugs introduced within a function $f$, we found 9 major structural/syntactic contexts they occurred in. 

\underline{{Cross-Language API callsite (47).}} 
%With 47 cases, bugs are most frequently introduced at the sites where APIs from different languages interact. This suggests that the interplay of languages can lead to misunderstandings or misuse, potentially due to differences in language specifications, data types, or conventions.
The bug was introduced right at a cross-language API callsite within the function $f$. This is the most common type of introducing location of multilingual bugs. 

\underline{{Function call (31).}} 
The bug occurred at a callsite of a function within $f$, but the callee is not a cross-language function/API---although the function call is on the cross-language information flow responsible for the bug. 
%This means 
The callee is misused or itself faulty. 
%This is the specific location in the code where a function is invoked with 31 cases. This bug indicates problems with the function being called - possibly it is not behaving as expected, or the return value is handled in an incorrect way.

\underline{{Assignment (29).}}
The bug happened when a variable is assigned a specific value on an assignment statement. 
In these cases, the variables often refer to foreign data, immediately or indirectly. 
%This is the location where a variable is assigned a specific value in the code with 29 cases. This location account for 29 cases. Misunderstandings or incorrect assumptions about data types or values when assigning variables could lead to bugs.

\underline{{True/False branch (24).}}
The bug was introduced in a conditional code structure within $f$, either on the true branch (i.e., in the {\tt if} body) or the false branch (i.e., in the {\tt else} body). 
%This refers to the sections of code that are conditionally executed based on the evaluation of a condition with 24 cases. Bugs in true/false branches could be due to incorrect logical conditions, leading the program to take the wrong path.

\underline{{Return (23).}}
The bug occurred at one of the return sites of the function $f$. 
The return site does not always have a return value. 
%This is the location in the code where control flow returns back from a function along with an optional return value with 23 cases. These bugs could signify that the function is returning an incorrect or unexpected result.

\underline{{Following a foreign function call (14).}}
The bug was introduced at a statement of $f$ that immediately follows a call to a foreign function. 
Typically, the statement depends on that call. 
%14 cases occurred at the lines of code that are executed immediately after a function call to a function defined in a different programming language or module. These could be bugs resulting from misunderstandings or incorrect assumptions about what the foreign function does or the state it leaves the system in.

\underline{{Conditional expression (13).}}
In these cases, the bug occurred in a conditional expression (e.g., a predicate there) at a conditional statement in the function $f$. 
This expression often directly impacts the cross-language control flow underlying the bug. 
%With 13 cases, this location refers to the conditions that dictate which code blocks are executed.  These could be bugs resulting from misunderstandings or incorrect assumptions about what the foreign function does or the state it leaves the system in.

\underline{{Loop body (9).}}
The bug happened within an iterative control-flow structure (i.e., the body of a loop) where there is no previous kind of multilingual bug introducing locations. 
%This is the location in the code where a set of instructions is repeated until a certain condition is met with 9 cases. Bugs in loop bodies could be due to incorrect loop conditions, or problems with the code that is executed in each loop iteration.

\underline{{Other (4).}}
In these few cases, the bug was introduced in %miscellaneous 
other locations, such as 
object instantiation and {\tt struct} declaration. 
%This includes all other locations within a function that do not fit into the above categories with 4 cases. Bugs categorized under "Other" locations emerge from a variety of contexts: Accessing arrays, assertion conditions, object instantiation, and struct declarations. Array access bugs often arise from out-of-bound accesses or accessing uninitialized arrays, pointing towards the need for careful management of array indices and proper initialization. Bugs related to assert statements signify unexpected states in the program, emphasizing the need for extensive testing and careful handling of such conditions. Errors during object instantiation occur due to improper constructor definitions, incorrect usage, or insufficient memory, underscoring the importance of proper class definitions and effective memory management. Lastly, bugs in struct declarations can be caused by incorrect field types, accessing non-existent fields, or memory allocation issues, reminding developers of the importance of diligent struct definitions, adherence to field types, and careful memory management. 


\subsubsection{Outside Function}
From the 22 bugs identified as occurring outside of any functions, the majority (19 cases) were found in the global area (e.g., declaring and/or initializing a global variable). 
%or outside any specific function. 
The multilingual bugs also arose in function or variable declarations and preprocessor directives, in 3 cases in total. %with 1 and 2 cases respectively, 
%pointing to potential difficulties in these areas as well, perhaps due to misunderstandings or misuses of language-specific syntax or constructs in a multilingual context. 

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/intoducing.pdf}
	\caption{Distribution of studied multilingual bugs across high-level (within/outside function) introducing locations overall (left) and main within-function locations (right).}
	\label{fig:introducing}
	\vspace{-4pt}
\end{figure}

As shown in Figure~\ref{fig:introducing}, 
%multilingual bugs are much more likely to occur within a function's body than outside of any function. 
out of the 216 cases analyzed, 194 bugs (nearly 90\%) occurred within a function, indicating these bugs are generally tied to functional logic (rather than global areas, for instance). 
%that a large portion of multilingual issues are tied to the functional logic of the code.
Among the within-function bugs, callsites are a dominating location where these bugs occurred. 

\find{
%Multilingual bugs can be introduced both within and outside functions. Within functions, common bug locations include cross-language API call sites, function calls, and assignments, indicating a need for clear understanding of API interactions and language specifications. Other areas, like branches, return statements, and loop bodies, require careful attention to logical conditions and system state. Outside functions, bugs often occur in the global area or during function/variable declarations, suggesting the importance of proper handling of global variables and a thorough understanding of language-specific syntax in a multilingual context. 
Multilingual bugs can be introduced in a variety of code locations/structures, but they 
most commonly occurred within a function, especially at a cross-language API callsite.
}

==> RQ-introducing_location.tex <==
\subsection{RQ2: Introducing location of multilingual bugs}\label{RQ2}

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/intoducing.pdf}
	\caption{Introducing bug location distribution among multilingual bugs
(left), and the distribution of all the within function locations (right). }
	\label{fig:introducing}
	\vspace{-4pt}
\end{figure}

As shown in~\ref{fig:introducing}, multilingual bugs are more likely to occur within a function than outside of it. Out of 216 cases analyzed, 194 bugs, or approximately 90\%, occurred within a function, indicating that a large portion of multilingual issues are tied to the functional logic of the code.

\subsubsection{Within function} There are 9 different introducing bug locations within the function.

\underline{\textbf{Cross-Language API call site.}} With 47 cases, bugs are most frequently introduced at the sites where APIs from different languages interact. This suggests that the interplay of languages can lead to misunderstandings or misuse, potentially due to differences in language specifications, data types, or conventions.

\underline{\textbf{Function call.}} 
This is the specific location in the code where a function is invoked with 31 cases.
This bug indicates problems with the function being called - possibly it is not behaving as expected, or the return value is handled in an incorrect way.

\underline{\textbf{Assignment.}}
This is the location where a variable is assigned a specific value in the code with 29 cases. This location account for 29 cases. Misunderstandings or incorrect assumptions about data types or values when assigning variables could lead to bugs.

\underline{\textbf{True/False branch.}}
This refers to the sections of code that are conditionally executed based on the evaluation of a condition with 24 cases. Bugs in true/false branches could be due to incorrect logical conditions, leading the program to take the wrong path.

\underline{\textbf{Return.}}
This is the location in the code where control flow returns back from a function along with an optional return value with 23 cases. These bugs could signify that the function is returning an incorrect or unexpected result.

\underline{\textbf{Following a foreign function Call.}}
14 cases occurred at the lines of code that are executed immediately after a function call to a function defined in a different programming language or module. These could be bugs resulting from misunderstandings or incorrect assumptions about what the foreign function does or the state it leaves the system in.

\underline{\textbf{Conditional expression.}}
With 13 cases, this location refers to the conditions that dictate which code blocks are executed.  These could be bugs resulting from misunderstandings or incorrect assumptions about what the foreign function does or the state it leaves the system in.

\underline{\textbf{Loop body.}}
This is the location in the code where a set of instructions is repeated until a certain condition is met with 9 cases. Bugs in loop bodies could be due to incorrect loop conditions, or problems with the code that is executed in each loop iteration.

\underline{\textbf{Other.}}
This includes all other locations within a function that do not fit into the above categories with 4 cases. Bugs categorized under "Other" locations emerge from a variety of contexts: Accessing arrays, assertion conditions, object instantiation, and struct declarations. Array access bugs often arise from out-of-bound accesses or accessing uninitialized arrays, pointing towards the need for careful management of array indices and proper initialization. Bugs related to assert statements signify unexpected states in the program, emphasizing the need for extensive testing and careful handling of such conditions. Errors during object instantiation occur due to improper constructor definitions, incorrect usage, or insufficient memory, underscoring the importance of proper class definitions and effective memory management. Lastly, bugs in struct declarations can be caused by incorrect field types, accessing non-existent fields, or memory allocation issues, reminding developers of the importance of diligent struct definitions, adherence to field types, and careful memory management. 


\subsubsection{Outside function}
From the 22 bugs identified as occurring outside of functions, the majority, or 19 cases, were found in the global area or outside any specific function. Bugs also arose in function or variable declarations and preprocessor directives, with 1 and 2 cases respectively, pointing to potential difficulties in these areas as well, perhaps due to misunderstandings or misuses of language-specific syntax or constructs in a multilingual context. 


\find{
Multilingual bugs can be introduced both within and outside functions. Within functions, common bug locations include cross-language API call sites, function calls, and assignments, indicating a need for clear understanding of API interactions and language specifications. Other areas, like branches, return statements, and loop bodies, require careful attention to logical conditions and system state. Outside functions, bugs often occur in the global area or during function/variable declarations, suggesting the importance of proper handling of global variables and a thorough understanding of language-specific syntax in a multilingual context.
}

==> RQ-manifestation-cai.tex <==
\subsection{RQ3: Manifestation Characteristics}\label{RQ3}
To understand how multilingual bugs are manifested, we mainly examined two manifestation characteristics: 
(1) the type of cross-language function/API involved in terms of its functional semantics and (2) the direction/complexity of the underlying cross-language information (data/control) flow. 
%Our study comprehensively explores these two core aspects, namely the semantic type of the cross-language API involved and the direction/complexity of control/data flow.

\subsubsection{Type/Semantics of Cross-Language Function/API}
%In our study of 216 multilingual bugs, we have classified them according to the semantic type of the cross-language API involved into 6 categories. The 34 bugs that involved more than one API category underscores the complexity of some multilingual bugs, as they can span multiple semantic types. 
Per its nature and definition, a multilingual bug involves one directly, most responsible cross-language function/API. 
%---we found the majority of the bugs involved only one
The semantics of these functions/APIs immediately inform the semantic nature of the bug, which mainly fell in 6 categories: 

\underline{{Reference counting (88).}}
Reference counting is a fundamental aspect of memory management in Python. It helps ensure that memory is efficiently allocated and deallocated. 
However, this result suggests that it is a primary type of code semantics 
via which the studied multilingual bugs were manifested. 
%source of bugs in multilingual applications. 
These bugs often arise from improper increments or decrements of reference counts, leading to memory leaks or premature disposal of objects.

\underline{{Object manipulation (68).}} 
Another major category of 
%cross-language APIs via which multilingual bugs have been manifested in our study are those 
cross-langu age semantics of multilingual bugs includes those aimed at manipulating (e.g., creating, accessing, and managing) foreign (Python) objects. 
These bugs involve 
%This category may represent bugs related to creating, using, or managing Python objects in a multilingual environment. Bugs here might include 
incorrect object creation, misuse of object methods, or issues with object lifetime management.  
This result points to difficulties in managing %complex 
objects %hierarchies 
across languages.

\underline{{Exception handling (68).}}
Python's foreign function APIs allow for error signaling and exception handling. 
68 of the bugs were manifested in cross-language semantics related to  
%could be due to 
incorrect handling of exceptions, such as failing to catch exceptions thrown by foreign code or incorrectly propagating %Python 
exceptions to the foreign language unit. 
This number suggests a significant challenge in managing error conditions across language boundaries.

\underline{{Parsing (14).}}
Parsing involves translating a string into a data structure according to certain rules or specific grammar. 
In our study, multilingual bugs manifested in this kind of semantics 
commonly resulted from inconsistencies or errors in how the respective cross-language APIs parse data from foreign languages or translate foreign data to a format the native language can understand. 
%The lower number of bugs suggest that parsing is less problematic than other categories, or perhaps less frequently used in the bugs' context studied.

\underline{{Protocol (5).}}
A few bugs in our study were manifested when the responsible cross-language API 
implements or uses network protocols, communication protocols, or protocol-based 
foreign functions. 
The number suggests the relative rarity of such situations. 
%APIs in the foreign language. The low number of bugs suggests that protocol-related issues are less common in multilingual development.

\underline{{Other (10).}}
In these 10 cases, the bug-manifesting cross-language APIs have 
miscellaneous semantics. For instance, they include foreign functions that target operating-system-level utilities %(in 3 cases). 
APIs for importing modules or setting handlers for asynchronous events. 

%Although the majority of the studied bugs involved primarily only one of the above categories of semantics, there are 34 bugs that involve more than one. 

\subsubsection{Control/Data Flow Direction}
In order to effectively understand and address the cause of a specific multilingual bug, it is helpful to understand the direction of its underlying cross-language control/data flow. 
In particular, we identify the information flow path of the cross-language data
traversing through different languages, starting at where the data was originated and leading to the point where the bug was manifested. 
%For example, a data object was first created in Python and then incorrectly manipulated in C. This attribution is based on the order of the languages involved in the manipulation of the data object and, more importantly, the bug occurrence. In this case, the direction of the control/data flow could be defined as from Python to C. In other words, we determine this direction by tracing the flow prior to the occurrence of the bug, examining how it traverses the language boundary.

For 199 of the bugs, the responsible information flow goes 
from the native (C) to foreign (Python) language, while in the other 17 cases the flow goes in the opposite direction (from Python to C). 
We further found that this dominance of {\tt native}$\rightarrow${\tt foreign} language information flow direction can be explained by two reasons:  
%The study indicates that there have been 199 cases where issues arose when transferring data from C to Python, but only 17 cases when transferring data from Python to C. This suggests that the main direction of data transfer issues is from C to Python. Here are some potential reasons:

\underline{Type system}: As a dynamically typed language, Python allows more flexibility with types (for example, a variable can change its type during execution), where C as a statically typed language does not have flexibility. 
Thus, more issues arose when data originated in C must be handled in Python 
than when the data is from Python. 
%C is statically typed, whereas Python is dynamically typed. This means that Python allows more flexibility with types (for example, a variable can change its type during execution), which can cause issues when data comes from a statically typed language like C.

\underline{Memory management}: C requires manual memory management, whereas Python manages memory automatically. When transitioning from manual to automatic memory management (C to Python) for data objects not handled correctly, bugs arose. 

% Another potential reason is the \ul{disparity in knowledge Background}. It's possible that the developer's proficiency differs between Python and C. Their understanding and usage of C may not be as extensive as Python, making it more prone to errors when handling data flow from C to Python. And the other possible reason is \underline{insufficient error handling}. There might not be ample error checking and handling mechanisms during the transfer from C to Python, potentially causing any minor mistakes to escalate into a bug.

\find{
The multilingual bugs studied were mostly manifested in code semantics on cross-language memory management (reference counting in particular), foreign object manipulation, and inter-language error handling. 
Moreover, the majority of the bugs were manifested in information flowing from the native to the foreign language. 
%In the study of 216 multilingual bugs, we identified two core characteristics: the semantic type of cross-language APIs and the direction of data flow. The bugs were majorly associated with Reference Counting (88), Objects (68), and Exception Handling (68), signifying that these areas pose significant challenges in multilingual coding. Furthermore, we discovered that the predominant direction of data flow issues was from C to Python (199 cases), as opposed to Python to C (17). 
}

==> RQ-manifestation.tex <==
\subsection{RQ3: Manifestation characteristics of multilingual bugs}\label{RQ3}
Our study comprehensively explores these two core aspects, namely the semantic type of the cross-language API involved and the direction/complexity of control/data flow.

\subsubsection{Manifestation characteristics}
In our study of 216 multilingual bugs, we have classified them according to the semantic type of the cross-language API involved into 6 categories. The 34 bugs that involved more than one API category underscores the complexity of some multilingual bugs, as they can span multiple semantic types. 

\underline{\textbf{Reference Counting (88).}}
Reference counting is a fundamental aspect of memory management in Python. It helps ensure that memory is efficiently allocated and deallocated. However, this result suggests that it's a major source of bugs in multilingual applications. These bugs can result from improper increment or decrement of reference counts, leading to memory leaks or premature disposal of objects.

\underline{\textbf{Objects (68).}}
This category may represent bugs related to creating, using, or managing Python objects in a multilingual environment. Bugs here might include incorrect object creation, misuse of object methods, or issues with object lifetimes. This could also include difficulties in managing complex object hierarchies across languages.


\underline{\textbf{Exception Handling (68).}}
Python's foreign function APIs allow for error signaling and exception handling. These bugs could be due to incorrect handling of exceptions, such as failing to catch exceptions thrown by foreign code or incorrectly propagating Python exceptions to foreign code. This number suggests a significant challenge in managing error conditions across language boundaries.

\underline{\textbf{Parsing (14).}}
Parsing involves translating a string into a data structure according to certain rules or a specific grammar. Bugs in this category could result from inconsistencies or errors in how Python's APIs parse data from foreign languages or translate Python data to a format the foreign language can understand. The lower number of bugs suggest that parsing is less problematic than other categories, or perhaps less frequently used in the bugs' context studied.

\underline{\textbf{Protocol (5).}}
This category could involve bugs in implementing or using network protocols, communication protocols, or protocol-based APIs from Python. The low number of bugs suggests that protocol-related issues are less common in multilingual development.

\underline{\textbf{Other (10).}}
This category encompasses a variety of Python's foreign function APIs. Operating System Utilities API, which accounts for three bugs, suggests potential complexities or errors when leveraging OS-level utilities in a multilingual context. Other API categories include Importing Modules, Set handlers for asynchronous events, etc.


\subsubsection{Control flow direction}
In order to effectively understand and address the cause of a specific bug, it is crucial to establish the direction of its control/data flow. What this means is identifying the path or sequence that the data object has traversed through different programming languages leading to the point where the bug emerged. For example, a data object was first created in Python and then incorrectly manipulated in C. This attribution is based on the order of the languages involved in the manipulation of the data object and, more importantly, the bug occurrence. In this case, the direction of the control/data flow could be defined as from Python to C. In other words, we determine this direction by tracing the flow prior to the occurrence of the bug, examining how it traverses the language boundary.

The study indicates that there have been 199 cases where issues arose when transferring data from C to Python, but only 17 cases when transferring data from Python to C. This suggests that the main direction of data transfer issues is from C to Python. Here are some potential reasons:

\underline{Type System}: C is statically typed, whereas Python is dynamically typed. This means that Python allows more flexibility with types (for example, a variable can change its type during execution), which can cause issues when data comes from a statically typed language like C.

\underline{Memory Management}: C requires manual memory management, whereas Python manages memory automatically. When transitioning from manual to automatic memory management (C to Python), if data objects are not handled correctly, it could lead to bugs.

% Another potential reason is the \ul{disparity in knowledge Background}. It's possible that the developer's proficiency differs between Python and C. Their understanding and usage of C may not be as extensive as Python, making it more prone to errors when handling data flow from C to Python. And the other possible reason is \underline{insufficient error handling}. There might not be ample error checking and handling mechanisms during the transfer from C to Python, potentially causing any minor mistakes to escalate into a bug.

\find{
In the study of 216 multilingual bugs, we identified two core characteristics: the semantic type of cross-language APIs and the direction of data flow. The bugs were majorly associated with Reference Counting (88), Objects (68), and Exception Handling (68), signifying that these areas pose significant challenges in multilingual coding. Furthermore, we discovered that the predominant direction of data flow issues was from C to Python (199 cases), as opposed to Python to C (17). 
}

==> RQ-root-cause.tex <==
\subsection{RQ4: Root Cause of CLBs}\label{RQ4}
%In this section, we dissect the root causes of cross-language bugs.
% We now dive deeper to dissect the root causes of cross-language bugs.
%, and present their distinctiveness.
We traced the data/control flow to determine the root causes of CLBs, and identified 18 (Python-C) and 12 (Java-C) root cause types.

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/rootcause.pdf}
	\caption{Distribution of root causes of cross-language bugs in Python-C (left) and Java-C (right) projects.}
	\label{fig:rootcause}
	\vspace{-4pt}
\end{figure}

\subsubsection{Statistics of Root Causes} 
As shown in Figure~\ref{fig:rootcause}. This analysis of root cause types shows that the most prevalent issues are related to logic errors, boundary conditional errors, and data type errors. 
% Logic errors, accounting for nearly 24.5\% and 32\% in Python-C and Java-C, are highlighted when integrating code written in different languages where complicated data/control flows are error-prone. 
% Boundary conditional errors, representing about 20\% and 23\% of the total bugs in Python-C and Java-C, remind developers to handle edge cases when integrating different languages correctly. 
% Data type error, comprising 10\% and 9.5\% of the total, point to the significance of correctly understanding and handling data types when data is passed between languages. 
The "other" category in our root cause analysis encapsulates some issues that are difficult to classify.
These are related to general concerns such as thread management issues, compilation errors, and compatibility errors.

\subsubsection{Root Causes (\textbf{RC})} 
Derived from the coding procedure, 
a comprehensive set of 
% 18 and 12 distinct 
categories had been identified. 
Subsequently, we presented definitions for these primary categories, conducting an in-depth analysis of their implications. 
Furthermore, we illustrated the concepts by including exemplar bugs representing instances within each category.


% \begin{figure}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=0.85\linewidth]{figure/root-cause-1-ref-misuse.pdf}
% 	\caption{A bug with a misused reference count~\cite{casestudy_reference}.}
% 	\label{fig:root-memory}
% 	\vspace{-12pt}
% \end{figure}

% \underline{{RC1: Memory safety (63).}} Memory safety is a critical characteristic of programming that prevents unintentional behaviors due to incorrect memory management. If a program is memory-safe, it efficiently averts bugs and security vulnerabilities where it erroneously accesses memory, allowing it to read from or write to unauthorized memory locations. 

% Given the substantial quantity of bugs linked to memory safety, surpassing the count of the second-most prevalent category (logic errors) by a factor of two,
% We undertook a more intricate classification of these bugs grounded in their distinct attributes. 
% The subcategories we have delineated encompass: Reference Count Misuse (24 cases), Null Pointer References (20 cases), Buffer Overflow (7 cases), Memory Allocation/Releasing (6 cases), Invalid Pointer (3 cases), Stack Overflow (2 cases), and Buffer Permission (1 case).

% This subdivision allows us to delve deeper into the various aspects of memory safety issues and develop more specific strategies to address each subcategory. For instance, with Null Pointer Reference issues, checking whether a pointer is null before dereferencing it is a helpful strategy. For Reference Count Misuse, precise reference count management ensures correct lifecycle management of objects. These specific strategies help us more effectively prevent and fix memory safety issues, thereby improving the reliability and security of our software.

% \textbf{Consequence.} These bugs cause erroneous behavior or crashes due to data corruption or invalid memory access. In certain cases, they even pose security vulnerabilities. For instance, an attacker exploits a buffer overflow to execute malicious code, or manipulate an invalid pointer to access sensitive data. Memory management errors, such as those arising from misuse of reference count or improper memory allocation or release, result in memory leaks or dangling pointers, deleting system performance over time, or leading to unpredictable behaviors.



% \textbf{Illustration.}
% Figure~\ref{fig:root-memory} depicts a memory leak bug resulting from improper reference count management in Numpy. The bug arises when performing a power operation on an array in Python (line p3). Initially, the native function {\tt array\_power} is called, followed by the faulty function {\tt is\_scalar\_with\_conversion} (line c6) in sequential order on the control flow path.
% Carried by the control flow, the Python object {\tt o2}, created from the integer 2 in Python (line p3), eventually reaches the bug function. At line c8, a new reference to {\tt o2} is established as {\tt value}, which continues to occupy memory even after it is no longer required beyond line c9. This occurs because the reference count has not been decremented. Over time, accumulating such memory leaks consumes amounts of memory, leading to system performance degradation or crashes.
% To rectify this bug, it is imperative to decrease the reference count of the Python object as soon as it becomes unnecessary (line c10).


\begin{figure}[tp]
	\vspace{-0pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-logicerror-2.pdf}
	\caption{A Python-C CLB case rooted in 'logic error'~\cite{casestudy_logic}.}
	\label{fig:root-logic}
	\vspace{-12pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-logicerror-2.pdf}
%     \caption{A Python-C CLB case with the root cause of 'logic error'~\cite{casestudy_logic}.}
%     \label{fig:root-logic}
% \end{wrapfigure}


\underline{{RC1: Logic error.}} A logic error is a type of runtime error that causes a program to deviate from its intended behavior through the cross-language information flow. 
Logic errors frequently stem from misconceptions or flawed presumptions made by the programmer during the development process. 
An instance of this is incorporating an incorrect algorithm—a situation where the algorithm devised to resolve a problem is either flawed or incomplete. 


\textbf{Consequence.} Logic errors, while not causing a program to crash outright, lead to negative outcomes, including incorrect output, data corruption, %poor user experience, 
and security vulnerabilities. 
% Logic errors have significant damage in more severe scenarios, particularly in systems dealing with sensitive data. Therefore, it's crucial to identify and rectify these errors. 


\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-logic}, the variable \texttt{keyfunc} is a parameter passed from Python. If this parameter is not NULL, then through the cross-language API \texttt{PyTuple\_New}, the variable \texttt{funcargs} is assigned a tuple object of size 0 (line c7). The purpose of creating \texttt{funcargs} is to receive a single parameter. However, creating a tuple of size 0 with \texttt{PyTuple\_New(0)} is incorrect. This could not only lead to runtime errors but also contradict the logic.

For fixing, the variable \texttt{funcargs} is assigned a tuple object of size 1 via cross-language API \texttt{PyTuple\_New}. This ensures that accessing the first element of \texttt{funcargs} will not result in an error. 



% As depicted in Figure~\ref{fig:root-logic}, 
% a scenario utilizes the caching \texttt{iternext} method of an iterator and then uses this cached method in a loop to get the next item. Caching is generally used to avoid the overhead of repeated operations by storing results that can be reused. However, in this code snippet, caching the \texttt{iternext} function does not provide a performance benefit. Caching the function might even be harmful in certain cases, e.g., the cached iterator could be shared across threads.

% For fixing, accesses the \texttt{iternext} method directly within the loop on each iteration (line c13), which does not use caching;
% thereby, each time the loop iterates, it obtains the \texttt{iternext} method by calling the foreign function \texttt{Py\_TYPE()}.


%  unfolds where a socket timeout is established, 
% and an endeavor is made to transmit a quantity of bytes exceeding the immediate transmission capacity. 
% In this context, the function prematurely throws an error, failing to adhere to the designated timeout duration. 
% To elaborate, if the intention is to transmit 2 bytes, 
% yet only one byte can be dispatched instantaneously, 
% the function proceeds to send just one byte. 
% This anomaly results from positioning the {\tt internal\_select()} call, responsible for monitoring the socket's readiness for transmission, outside the sending loop in its initial implementation.

% For fixing, {\tt internal\_select()} invocation is moved into the do-while loop (line c5);
% thereby, the function undergoes a transformation, 
% compelling it to await the full timeout interval prior to each transmission attempt, thus aligning with the expected behavior.



\ul{RC2: Boundary conditional error.} A boundary conditional error %, often called an edge case error, 
occurs when a condition at the boundary of an interval or at the extreme ends is not correctly handled on the cross-language information flow. These errors often manifest in scenarios like array indexing (accessing an element outside the bounds of an array), looping constructs (incorrect loop termination conditions), and numerical ranges (performing calculations at the limits of numerical ranges). 

\textbf{Consequence.}
These bugs result in incorrect program behavior, leading to inaccurate results or unpredictable operation. 
% In certain cases, these errors cause the program to crash, particularly if they result in attempts to access out of the specific range.
% Occasionally, these errors cause performance issues by unnecessarily overloading computational resources. 
% The potential severity of these outcomes underlines the importance of correctly handling boundary conditions in programming.

\textbf{Illustration.}
In Figure~\ref{fig:root-boundary}, the boundary condition error occurs when assigning the pointer for the implementation of the encryption algorithm obtained from \texttt{EVP\_aes\_128\_gcm()} to the variable \texttt{evp\_gcm\_cipher}.
There is a fixed key length for AES-GCM decryption without a mechanism to choose different versions of the AES-GCM algorithm based on the length of the key provided.

The fix for the bug was to add a check for this boundary condition. Before assigning the encryption pointer to the variable \texttt{evp\_gcm\_cipher}, the added switch-case structure allows the function to select the appropriate AES-GCM algorithm based on the length of the key. 
% This correct handling of the boundary condition prevents incorrect pointer usage from occurring.



% the boundary condition error occurs when the {\tt PyArray\_FromArray} function is called with an array and a data type descriptor that cannot be safely cast to each other. The {\tt PyArray\_FromArray} function is expected to create a new array from an existing array with a specified data type descriptor. However, when the existing array's data type cannot be safely cast to the specified data type descriptor, the function returns NULL (line c18). There was no check to see if {\tt "obj"} was NULL after the call to {\tt PyArray\_FromArray}. This meant that if {\tt PyArray\_FromArray} returned NULL, the code would continue to execute with {\tt "obj"} set to NULL, which leads to a segmentation fault.

% The fix for the bug was to add a check for this boundary condition. After the call to {\tt PyArray\_FromArray}, the code now checks whether the returned array is NULL. If so, a “ValueError” is raised with a message indicating that an array of the proper type fails to be created from the output array, and the function exits with a failure status. This correct handling of the boundary condition prevents the segmentation fault from occurring.


\begin{figure}[tp]
	\vspace{-4pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-boundary.pdf}
	\caption{A Java-C CLB case with the root cause of 'boundary conditional error'~\cite{casestudy_boundary_conditional}.}
	\label{fig:root-boundary}
	\vspace{-8pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-boundary.pdf}
%     \caption{A Java-C CLB case with the root cause of 'boundary conditional error'~\cite{casestudy_boundary_conditional}.}
%     \label{fig:root-boundary}
% \end{wrapfigure}


\underline{{RC3: Data type.}} These bugs manifest when an operation is executed in a manner that contradicts the data type of the value it operates upon. 
This is due to incorrect data type conversion between languages, incompatible data types resulting from assumptions made when integrating different languages, or incorrect usage of data types due to varying data type systems in different languages. 

\textbf{Consequence.} Data type bugs within a cross-language program trigger a cascade of predicaments, spanning from erroneous program conduct and system crashes to compromising security vulnerabilities. 
% Such bugs introduce subtle and elusive defects, making debugging and maintenance endeavors arduous and intricate.
% The intricacies of these issues are further amplified within a multi-language programming milieu, wherein data types are managed disparately across various languages. 

\begin{figure}[tp]
	\vspace{-0pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-datatype.pdf}
	\caption{A Python-C CLB case rooted in 'data type error'~\cite{casestudy_datatype}.}
	\label{fig:root-data-type}
	\vspace{-4pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-datatype.pdf}
%     \caption{A Python-C CLB case with the root cause of 'data type error'~\cite{casestudy_datatype}.}
%     \label{fig:root-data-type}
% \end{wrapfigure}

\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-data-type}, a critical concern emerges when the variable {\tt offset} is initially defined as an {\tt int} (line c16) while the data is transmitted along the cross-language flow from Python. 
When {\tt offset} is used to navigate through these large data arrays, its insufficient range could lead to incorrect memory access. 
% For instance, if an {\tt offset} calculation results in a value that exceeds the maximum or minimum value an int can hold, it might wrap around to a negative value or overflow, leading to an attempt to access a memory location that is out of bounds of the intended data structure. 

This scenario underscores the significance of appropriately managing data types. To rectify this bug, the solution involves defining the variable {\tt offset} with the type {\tt npy\_intp}, which is designed to hold any array index in NumPy (A Python library). This ensures compatibility with large arrays and reduces the potential for overflow or wrap-around errors. 


 
% As depicted in Figure~\ref{fig:root-data-type}, a critical concern emerges when the variable {\tt offset} is initially defined as int (line c16), while the offset of type {\tt long} is transmitted along the data flow from Python, carrying a size surpassing 2GB. In this scenario, a precarious situation arises where an overflow of {\tt bytesread} at line c10 becomes possible, triggering an inexhaustible loop.
% This scenario underscores the significance of appropriately managing data types and ensuring compatibility across the programming interfaces. An oversight in data type compatibility, as demonstrated in this example, can lead to severe runtime issues, such as infinite loops, compromising the functionality and stability of the system.
% To rectify this bug, it is recommended to redefine the variable {\tt bytesread} with the type {\tt Py\_off\_t} (line c3). This adjustment ensures that the two compared variables possess the same data type, and their bit-width aligns with the functional requirements.



\vspace{-4pt}
\find{
% In this study, we analyzed the root causes of cross-language bugs and found thirteen categories. 
The three primary root causes of CLBs were logic errors, boundary conditional errors, and data type errors. 
The number of bugs rooted in logic errors far dominated over those due to any other categories of root causes. 
%The quantity of bugs associated with memory safety exceeded the total of the second most common category, namely logic errors, by a multiplicative factor of two.

% The most prevalent bug was memory safety, emphasizing the significance of correct memory management, especially when dealing with languages that manage memory differently. Logic errors underline the need for comprehensive testing and code reviews to ensure the program behaves as intended. Data type bugs stress the importance of accurate understanding and handling of data types when data is passed between languages, while boundary conditional errors highlight the need to handle edge cases correctly.
}


==> RQ-root_cause-new.tex <==
\subsection{RQ4: Root Causes of Native Code Bugs}\label{RQ4}
%In this section, we dissect the root causes of multilingual bugs.
% We now dive deeper to dissect the root causes of multilingual bugs.
%, and present their distinctiveness.
%
%We traced the data/control flow to determine the root causes of native code bugs, and identified 13 root cause types.
To dissect why native code bugs happen, we conduct root cause analysis of the studied bugs by tracing the underlying data/control flow facts of each bug. 
As a result, we identified 13 root causes of native code bugs in Python applications as elaborated as shown in Table~\ref{fig:root-overview}. 
This analysis of root cause types shows that the most prevalent issues are related to memory safety, logic errors, data type errors, and boundary conditional errors. The dominance of memory safety issues, accounting for nearly 30\% of all bugs, emphasizes the importance of correctly managing memory across Python and C. 
Logic errors, representing about 11.57\% of the total bugs, are highlighted when integrating code written in these two languages where complicated data/control flows are error-prone. Data type bugs, comprising 10.65\% of the total, are also common, pointing to the challenge of correctly understanding and handling data types when data is passed between Python and C. Boundary conditional errors, representing about 9.26\% of the total bugs, pertain to erroneous handling of edge cases in native code behaviors. The "other" category in our root cause analysis encapsulates some issues that are difficult to classify furthermore. These are related to general concerns such as code generation, compilation errors, and installation processes.

% \begin{figure}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=1\linewidth]{figure/root cause-overview.pdf}
% 	\caption{Distribution of root causes of native code bugs.}
% 	\label{fig:root-overview}
% 	\vspace{-4pt}
% \end{figure}


\begin{table}[ht]
\centering
\caption{Distribution of root causes of native code bugs}
\label{fig:root-overview}
\begin{tabular}{lrc}
\toprule
\textbf{Root Cause} & \textbf{Count} & \textbf{Percentage} \\
\midrule
Memory Safety & 63 & 29.17\% \\
Logic Error & 25 & 11.57\% \\
Data Type Error & 24 & 11.11\% \\
Boundary Conditional Error & 20 & 9.26\% \\
API/Function Misuse & 14 & 6.48\% \\
Improper Exception Handling & 13 & 6.02\% \\
Initialization\&Variable Misuse Errors & 12 & 5.56\% \\
Mathematical Errors & 6 & 2.78\% \\
Input and Output Handling & 6 & 2.78\% \\
Compatibility & 6 & 2.78\% \\
Resource Management Errors & 5 & 2.31\% \\
Access and Permission Errors & 4 & 1.85\% \\
Other & 18 & 8.33\% \\
\bottomrule
\end{tabular}
\end{table}


%\subsubsection{Statistics of Root Causes} 

%\subsubsection{Root Causes (\textbf{RC})} 
Next, we elaborate these root causes, as derived from our coding procedure. 
%a comprehensive set of thirteen distinct categories had been identified. 
For each root cause (\textbf{RC}), we start with the definition, followed by an in-depth analysis of it and its implications. 
Furthermore, we illustrated the root cause through representative bug cases. %representing instances within each category.
We focus on the top-4 root causes, which together account for 61.1\% of all of the native code bugs we studied. 

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.55\linewidth]{figure/root-cause-1-ref-misuse.pdf}
	\caption{A native bug case rooted in a misused reference count~\cite{casestudy_reference}.}
	\label{fig:root-memory}
	\vspace{-12pt}
\end{figure}

\underline{{RC1: Memory safety (63).}} Memory safety is a critical characteristic of programming that prevents unintentional behaviors due to incorrect memory management. If a program is memory-safe, it efficiently averts bugs and security vulnerabilities where it erroneously accesses memory, allowing it to read from or write to unauthorized memory locations. 
This prevalent root cause may not be surprising, given the capabilities of the C language in accessing and manipulating memory. 

Given the substantial quantity of bugs linked to memory safety, surpassing the count of the second-most prevalent category (logic errors) by a factor of two,
we undertook a more detailed classification of these bugs grounded in their distinct attributes. 
The subcategories we have delineated encompass: Reference Count Misuse (24 cases), Null Pointer Dereference (20 cases), Buffer Overflow (7 cases), Memory Allocation/Releasing (6 cases), Invalid Pointer (3 cases), Stack Overflow (2 cases), and Buffer Permission (1 case).

This subdivision allows us to delve deeper into the various aspects of memory safety issues and develop more specific strategies to address each subcategory. For instance, with Null Pointer Dereference issues, checking whether a pointer is null before dereferencing it is a helpful strategy. For Reference Count Misuse, precise reference count management ensures correct lifecycle management of objects. These specific strategies help with more effectively preventing and fixing memory safety issues, thereby improving the reliability and security of the native Python applications.

%\textbf{Consequence.} 
These bugs cause erroneous behavior or crashes due to data corruption or invalid memory access. In certain cases, they even pose security threats. %vulnerabilities. 
For instance, an attacker may exploit a buffer overflow in the native code to execute malicious code, or manipulate an invalid pointer to access sensitive data. In other examples, the memory management errors, such as those arising from misuse of reference count or improper memory allocation or release, result in memory leaks or dangling pointers, compromising system performance over time, or leading to unpredictable behaviors.


%\textbf{Illustration.}
%\ref{fig:root-memory} illustrates a specific instance of a memory leak caused by incorrect reference count management in a multi-language programming environment. In this case, the foreign function {\tt PyLong\_AsSsize\_t} is invoked to convert a variable named {\tt "value"} from the {\tt ssize\_t} type to the long type. This function is typically used in the context of Python's C API, which allows C programs to interact with Python's runtime system. The memory leak occurs because the variable {\tt "value"} reference count is not properly decremented after the conversion. In this case, the variable {\tt "value"} continues to occupy memory even after it has been converted and is no longer needed, because its reference count has not been decremented. Over time, if such memory leaks accumulate, they can consume significant amounts of memory, potentially leading to system performance degradation or even crashes. This underlines the importance of correctly managing reference counts when interacting with Python objects in C or other languages, to prevent memory leaks and ensure efficient use of system resources.
Figure~\ref{fig:root-memory} depicts a memory-leak bug resulting from improper reference count management in Numpy~\cite{NumPy}. The bug arises when performing a power operation on an array in Python (line p3). Initially, the native function {\tt array\_power} is called, followed by the faulty function invocation {\tt is\_scalar\_with\_conversion} (line c6) along the control flow path underlying this bug.
Carried by the control flow, the Python object {\tt o2}, created from the integer 2 in Python (line p3), eventually reaches the buggy function. At line c8, a new reference to {\tt o2} is established as {\tt value}, which continues to occupy memory even after it is no longer required beyond line c9. This occurs because the reference count has not been decremented. Over time, accumulating such memory leaks consumes monotonically increasing amounts of memory, leading to system performance degradation or crashes (i.e., out of memory). 
To rectify this bug, it is imperative to decrease the reference count of the Python object as soon as it becomes unnecessary in the native code (line c10).


\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.55\linewidth]{figure/root-cause-2-logic.pdf}
	\caption{A native bug case rooted in a logic error~\cite{casestudy_logic}.}
	\label{fig:root-logic}
	\vspace{-12pt}
\end{figure}


\underline{{RC2: Logic error (25).}} 
% A logic error is a type of runtime error that results in a program producing an incorrect output or deviating from the intended behavior. 
% Logic errors frequently stem from misconceptions or flawed presumptions made by the programmer during the development process. 
% An instance of this is incorporating an incorrect algorithm—a situation where the algorithm devised to resolve a problem is either flawed or incomplete. 
In general, a logic error is a runtime error where a program yields incorrect output or strays from its expected behavior otherwise. 
Such errors often originate from the programmer's misunderstandings or incorrect assumptions while coding. For example, employing an incorrect algorithm occurs when the chosen method to solve a problem is either erroneous or not fully developed. 
In particular, in the context of our studied native code bugs, the bug-causing logic errors are commonly resultant from incorrect understandings and/or assumptions about relevant foreign functions' semantics and the shape of foreign data objects, among other semantic disparities between the two interacting languages (Python and C).


%\textbf{Consequence.} 
% Logic errors, while not causing a program to crash outright, lead to negative outcomes, including incorrect output, data corruption, poor user experience, and potentially even security vulnerabilities. 
Generally, logic errors do not directly cause a program to fail; however, they result in adverse effects such as incorrect output, data corruption, degraded user experience, and even increased security risks, as demonstrated in our studied bug cases.  
These logic errors have even more significant damages in more severe scenarios, particularly in Python applications dealing with sensitive data. 
%Therefore, it is crucial to identify and rectify these errors. 

%\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-logic}, 
a scenario unfolds where a socket timeout is established, 
and an endeavor is made to transmit a quantity of bytes exceeding the immediate transmission capacity. 
In this context, the function prematurely throws an error, failing to adhere to the designated timeout duration. 
To elaborate, if the intention is to transmit 2 bytes, 
yet only one byte can be dispatched instantaneously, 
the function proceeds to send just one byte. 
This anomaly results from positioning the {\tt internal\_select()} call, responsible for monitoring the socket's readiness for transmission, outside the sending loop in its initial implementation.

For addressing this bug, {\tt internal\_select()} invocation is moved into the do-while loop (line c5);
thereby, the function undergoes a transformation, 
compelling it to await the full timeout interval prior to each transmission attempt, thus aligning with the expected behavior.


\underline{{RC3: Data type error (24).}} 
% These bugs manifest when an operation is executed in a manner that contradicts the data type of the value it operates upon. This is due to incorrect data type conversion between languages, incompatible data types resulting from assumptions made when integrating different languages, or incorrect usage of data types due to varying data type systems in different languages.
These bugs occur when an operation is performed in a way that is inconsistent with the data type of the value it operates upon. This inconsistency arise from improper data type conversion between Python and C, mismatched data types stemming from assumptions during Python-C integration, or the misuse of data types because of the differences in data type systems across these two languages.

%\textbf{Consequence.} 
% Data type bugs within a software program trigger a cascade of predicaments, spanning from erroneous program conduct and system crashes to compromising security vulnerabilities. 
Native code bugs caused by data type errors in our study led to a range of issues, including incorrect program behavior, system crashes, and even the exposure of security vulnerabilities.
Such bugs introduce subtle and elusive defects, making debugging and maintenance endeavors arduous and intricate.
The intricacies of these issues are further amplified, hence the consequences further exacerbated, %within a multi-language programming milieu, wherein 
when data objects of types that are incompatible between Python and C have to be involved (e.g., the native code operates on a Python dictionary consisting of elements of heterogeneous data types). 
%managed disparately across various languages. 

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.6\linewidth]{figure/root-cause-3-data-type.pdf}
	\caption{A native bug case rooted in integer overflow~\cite{casestudy_datatype}.}
	\label{fig:root-data-type}
	\vspace{-4pt}
\end{figure}

%\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-data-type}, a critical concern emerges when the variable {\tt bytesread} is initially defined as {\tt int} (line c2), while the offset of type {\tt long} is transmitted along the data flow originating from Python, carrying a size surpassing 2GB. In this scenario, a precarious situation arises where an overflow of {\tt bytesread} at line c10 becomes possible, triggering an inexhaustible loop.
This scenario underscores the significance of appropriately managing data types and ensuring compatibility across the language interfaces. An oversight in data type compatibility, as demonstrated in this example, can lead to severe runtime issues, such as infinite loops, compromising the functionality and stability of the system.
To rectify this bug, it is recommended to redefine the variable {\tt bytesread} with the type {\tt Py\_off\_t} (line c3). This adjustment ensures that the two compared variables possess the same data type, and their bit-width aligns with the functional requirements of this Python application.


\begin{figure}[tp]
	\vspace{-4pt}
	\includegraphics[width=0.6\linewidth]{figure/root-cause-4-boundary.pdf}
	\caption{A native bug case rooted in a boundary conditional error~\cite{casestudy_boundary_conditional}.}
	\label{fig:root-boundary}
	\vspace{-8pt}
\end{figure}

\ul{RC4: Boundary conditional error (20).} 
% A boundary conditional error, often called an off-by-one error or an edge case error, occurs when a condition at the boundary of an interval is not correctly handled. These errors often manifest in scenarios like array indexing (accessing an element outside the bounds of an array), looping constructs (incorrect loop termination conditions), and numerical ranges (performing calculations at the limits of numerical ranges). 
A boundary conditional error, %also known 
such as an off-by-one error or edge case error, arises when a boundary condition within a range is improperly managed. This type of error frequently appears in situations such as array indexing (where an attempt is made to access an array element beyond its boundary), looping constructs (where loop termination conditions are inaccurately defined), and numerical ranges (involving calculations at the extremities of numerical ranges).

%\textbf{Consequence.}
% These bugs result in incorrect program behavior, leading to inaccurate results or unpredictable program operation. 
These bugs lead to incorrect behavior in programs, causing inaccurate results or unpredictable operation.
In certain cases, these errors cause the program to crash, particularly if they result in attempts to access out of the specific range. Occasionally, these errors cause performance issues by unnecessarily overloading computational resources. 
The potential severity of these outcomes underlines the importance of correctly handling boundary conditions in the native code of Python applications.

%\textbf{Illustration.}
In Figure~\ref{fig:root-boundary}, the boundary condition error occurs when the {\tt PyArray\_FromArray} function is called with an array and a data type descriptor that cannot be safely cast to each other. The {\tt PyArray\_FromArray} function is expected to create a new array from an existing array with a specified data type descriptor. However, when the existing array's data type cannot be safely cast to the specified data type descriptor, the function returns NULL (line c18). There was no check to see if {\tt "obj"} was NULL after the call to {\tt PyArray\_FromArray}. This meant that if {\tt PyArray\_FromArray} returned NULL, the code would continue to execute with {\tt "obj"} set to NULL, which leads to a segmentation fault. 
Apparently, the bug is rooted in missing boundary checking, rather than data type errors. 

The fix for the bug was to add a check for this boundary condition. After the call to {\tt PyArray\_FromArray}, the code now checks whether the returned array is NULL. If so, a “ValueError” exception is raised with a message indicating that an array of the proper type fails to be created from the output array, and the function exits with a failure status. This correct handling of the boundary condition prevents the segmentation fault from occurring.


\vspace{0pt}
\find{
% In this study, we analyzed the root causes of multilingual bugs and found thirteen categories. 
The four primary root causes of native code bugs are memory safety violations (29.17\%), logic errors (11.57\%), data type issues (11.11\%), and boundary conditional errors (9.26\%). 
%The number of bugs rooted in memory safety errors far dominated over those due to any other categories of root causes. 
More specifically, the memory safety violations are mainly due to reference count misuse (38.1\%) and null pointer dereference (31.7\%).
%The quantity of bugs associated with memory safety exceeded the total of the second most common category, namely logic errors, by a multiplicative factor of two.
%
% The most prevalent bug was memory safety, emphasizing the significance of correct memory management, especially when dealing with languages that manage memory differently. Logic errors underline the need for comprehensive testing and code reviews to ensure the program behaves as intended. Data type bugs stress the importance of accurate understanding and handling of data types when data is passed between languages, while boundary conditional errors highlight the need to handle edge cases correctly.
}


==> RQ-root_cause.tex <==
\subsection{RQ4: Root Cause of CLBs}\label{RQ4}
%In this section, we dissect the root causes of cross-language bugs.
% We now dive deeper to dissect the root causes of cross-language bugs.
%, and present their distinctiveness.
We traced the data/control flow to determine the root causes of CLBs, and identified 18 (Python-C) and 12 (Java-C) root cause types.

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/rootcause.pdf}
	\caption{Distribution of root causes of cross-language bugs in Python-C (left) and Java-C (right) projects.}
	\label{fig:rootcause}
	\vspace{-4pt}
\end{figure}

\subsubsection{Statistics of Root Causes} 
As shown in Figure~\ref{fig:rootcause}. This analysis of root cause types shows that the most prevalent issues are related to logic errors, boundary conditional errors, and data type errors. 
% Logic errors, accounting for nearly 24.5\% and 32\% in Python-C and Java-C, are highlighted when integrating code written in different languages where complicated data/control flows are error-prone. 
% Boundary conditional errors, representing about 20\% and 23\% of the total bugs in Python-C and Java-C, remind developers to handle edge cases when integrating different languages correctly. 
% Data type error, comprising 10\% and 9.5\% of the total, point to the significance of correctly understanding and handling data types when data is passed between languages. 
The "other" category in our root cause analysis encapsulates some issues that are difficult to classify.
These are related to general concerns such as thread management issues, compilation errors, and compatibility errors.

\subsubsection{Root Causes (\textbf{RC})} 
Derived from the coding procedure, 
a comprehensive set of 
% 18 and 12 distinct 
categories had been identified. 
Subsequently, we presented definitions for these primary categories, conducting an in-depth analysis of their implications. 
Furthermore, we illustrated the concepts by including exemplar bugs representing instances within each category.


% \begin{figure}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=0.85\linewidth]{figure/root-cause-1-ref-misuse.pdf}
% 	\caption{A bug with a misused reference count~\cite{casestudy_reference}.}
% 	\label{fig:root-memory}
% 	\vspace{-12pt}
% \end{figure}

% \underline{{RC1: Memory safety (63).}} Memory safety is a critical characteristic of programming that prevents unintentional behaviors due to incorrect memory management. If a program is memory-safe, it efficiently averts bugs and security vulnerabilities where it erroneously accesses memory, allowing it to read from or write to unauthorized memory locations. 

% Given the substantial quantity of bugs linked to memory safety, surpassing the count of the second-most prevalent category (logic errors) by a factor of two,
% We undertook a more intricate classification of these bugs grounded in their distinct attributes. 
% The subcategories we have delineated encompass: Reference Count Misuse (24 cases), Null Pointer References (20 cases), Buffer Overflow (7 cases), Memory Allocation/Releasing (6 cases), Invalid Pointer (3 cases), Stack Overflow (2 cases), and Buffer Permission (1 case).

% This subdivision allows us to delve deeper into the various aspects of memory safety issues and develop more specific strategies to address each subcategory. For instance, with Null Pointer Reference issues, checking whether a pointer is null before dereferencing it is a helpful strategy. For Reference Count Misuse, precise reference count management ensures correct lifecycle management of objects. These specific strategies help us more effectively prevent and fix memory safety issues, thereby improving the reliability and security of our software.

% \textbf{Consequence.} These bugs cause erroneous behavior or crashes due to data corruption or invalid memory access. In certain cases, they even pose security vulnerabilities. For instance, an attacker exploits a buffer overflow to execute malicious code, or manipulate an invalid pointer to access sensitive data. Memory management errors, such as those arising from misuse of reference count or improper memory allocation or release, result in memory leaks or dangling pointers, deleting system performance over time, or leading to unpredictable behaviors.



% \textbf{Illustration.}
% Figure~\ref{fig:root-memory} depicts a memory leak bug resulting from improper reference count management in Numpy. The bug arises when performing a power operation on an array in Python (line p3). Initially, the native function {\tt array\_power} is called, followed by the faulty function {\tt is\_scalar\_with\_conversion} (line c6) in sequential order on the control flow path.
% Carried by the control flow, the Python object {\tt o2}, created from the integer 2 in Python (line p3), eventually reaches the bug function. At line c8, a new reference to {\tt o2} is established as {\tt value}, which continues to occupy memory even after it is no longer required beyond line c9. This occurs because the reference count has not been decremented. Over time, accumulating such memory leaks consumes amounts of memory, leading to system performance degradation or crashes.
% To rectify this bug, it is imperative to decrease the reference count of the Python object as soon as it becomes unnecessary (line c10).


\begin{figure}[tp]
	\vspace{-0pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-logicerror-2.pdf}
	\caption{A Python-C CLB case rooted in 'logic error'~\cite{casestudy_logic}.}
	\label{fig:root-logic}
	\vspace{-12pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-logicerror-2.pdf}
%     \caption{A Python-C CLB case with the root cause of 'logic error'~\cite{casestudy_logic}.}
%     \label{fig:root-logic}
% \end{wrapfigure}


\underline{{RC1: Logic error.}} A logic error is a type of runtime error that causes a program to deviate from its intended behavior through the cross-language information flow. 
Logic errors frequently stem from misconceptions or flawed presumptions made by the programmer during the development process. 
An instance of this is incorporating an incorrect algorithm—a situation where the algorithm devised to resolve a problem is either flawed or incomplete. 


\textbf{Consequence.} Logic errors, while not causing a program to crash outright, lead to negative outcomes, including incorrect output, data corruption, %poor user experience, 
and security vulnerabilities. 
% Logic errors have significant damage in more severe scenarios, particularly in systems dealing with sensitive data. Therefore, it's crucial to identify and rectify these errors. 


\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-logic}, the variable \texttt{keyfunc} is a parameter passed from Python. If this parameter is not NULL, then through the cross-language API \texttt{PyTuple\_New}, the variable \texttt{funcargs} is assigned a tuple object of size 0 (line c7). The purpose of creating \texttt{funcargs} is to receive a single parameter. However, creating a tuple of size 0 with \texttt{PyTuple\_New(0)} is incorrect. This could not only lead to runtime errors but also contradict the logic.

For fixing, the variable \texttt{funcargs} is assigned a tuple object of size 1 via cross-language API \texttt{PyTuple\_New}. This ensures that accessing the first element of \texttt{funcargs} will not result in an error. 



% As depicted in Figure~\ref{fig:root-logic}, 
% a scenario utilizes the caching \texttt{iternext} method of an iterator and then uses this cached method in a loop to get the next item. Caching is generally used to avoid the overhead of repeated operations by storing results that can be reused. However, in this code snippet, caching the \texttt{iternext} function does not provide a performance benefit. Caching the function might even be harmful in certain cases, e.g., the cached iterator could be shared across threads.

% For fixing, accesses the \texttt{iternext} method directly within the loop on each iteration (line c13), which does not use caching;
% thereby, each time the loop iterates, it obtains the \texttt{iternext} method by calling the foreign function \texttt{Py\_TYPE()}.


%  unfolds where a socket timeout is established, 
% and an endeavor is made to transmit a quantity of bytes exceeding the immediate transmission capacity. 
% In this context, the function prematurely throws an error, failing to adhere to the designated timeout duration. 
% To elaborate, if the intention is to transmit 2 bytes, 
% yet only one byte can be dispatched instantaneously, 
% the function proceeds to send just one byte. 
% This anomaly results from positioning the {\tt internal\_select()} call, responsible for monitoring the socket's readiness for transmission, outside the sending loop in its initial implementation.

% For fixing, {\tt internal\_select()} invocation is moved into the do-while loop (line c5);
% thereby, the function undergoes a transformation, 
% compelling it to await the full timeout interval prior to each transmission attempt, thus aligning with the expected behavior.



\ul{RC2: Boundary conditional error.} A boundary conditional error %, often called an edge case error, 
occurs when a condition at the boundary of an interval or at the extreme ends is not correctly handled on the cross-language information flow. These errors often manifest in scenarios like array indexing (accessing an element outside the bounds of an array), looping constructs (incorrect loop termination conditions), and numerical ranges (performing calculations at the limits of numerical ranges). 

\textbf{Consequence.}
These bugs result in incorrect program behavior, leading to inaccurate results or unpredictable operation. 
% In certain cases, these errors cause the program to crash, particularly if they result in attempts to access out of the specific range.
% Occasionally, these errors cause performance issues by unnecessarily overloading computational resources. 
% The potential severity of these outcomes underlines the importance of correctly handling boundary conditions in programming.

\textbf{Illustration.}
In Figure~\ref{fig:root-boundary}, the boundary condition error occurs when assigning the pointer for the implementation of the encryption algorithm obtained from \texttt{EVP\_aes\_128\_gcm()} to the variable \texttt{evp\_gcm\_cipher}.
There is a fixed key length for AES-GCM decryption without a mechanism to choose different versions of the AES-GCM algorithm based on the length of the key provided.

The fix for the bug was to add a check for this boundary condition. Before assigning the encryption pointer to the variable \texttt{evp\_gcm\_cipher}, the added switch-case structure allows the function to select the appropriate AES-GCM algorithm based on the length of the key. 
% This correct handling of the boundary condition prevents incorrect pointer usage from occurring.



% the boundary condition error occurs when the {\tt PyArray\_FromArray} function is called with an array and a data type descriptor that cannot be safely cast to each other. The {\tt PyArray\_FromArray} function is expected to create a new array from an existing array with a specified data type descriptor. However, when the existing array's data type cannot be safely cast to the specified data type descriptor, the function returns NULL (line c18). There was no check to see if {\tt "obj"} was NULL after the call to {\tt PyArray\_FromArray}. This meant that if {\tt PyArray\_FromArray} returned NULL, the code would continue to execute with {\tt "obj"} set to NULL, which leads to a segmentation fault.

% The fix for the bug was to add a check for this boundary condition. After the call to {\tt PyArray\_FromArray}, the code now checks whether the returned array is NULL. If so, a “ValueError” is raised with a message indicating that an array of the proper type fails to be created from the output array, and the function exits with a failure status. This correct handling of the boundary condition prevents the segmentation fault from occurring.


\begin{figure}[tp]
	\vspace{-4pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-boundary.pdf}
	\caption{A Java-C CLB case with the root cause of 'boundary conditional error'~\cite{casestudy_boundary_conditional}.}
	\label{fig:root-boundary}
	\vspace{-8pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-boundary.pdf}
%     \caption{A Java-C CLB case with the root cause of 'boundary conditional error'~\cite{casestudy_boundary_conditional}.}
%     \label{fig:root-boundary}
% \end{wrapfigure}


\underline{{RC3: Data type.}} These bugs manifest when an operation is executed in a manner that contradicts the data type of the value it operates upon. 
This is due to incorrect data type conversion between languages, incompatible data types resulting from assumptions made when integrating different languages, or incorrect usage of data types due to varying data type systems in different languages. 

\textbf{Consequence.} Data type bugs within a cross-language program trigger a cascade of predicaments, spanning from erroneous program conduct and system crashes to compromising security vulnerabilities. 
% Such bugs introduce subtle and elusive defects, making debugging and maintenance endeavors arduous and intricate.
% The intricacies of these issues are further amplified within a multi-language programming milieu, wherein data types are managed disparately across various languages. 

\begin{figure}[tp]
	\vspace{-0pt}
	\centering\includegraphics[width=0.7\linewidth]{figure/rootcause-datatype.pdf}
	\caption{A Python-C CLB case rooted in 'data type error'~\cite{casestudy_datatype}.}
	\label{fig:root-data-type}
	\vspace{-4pt}
\end{figure}
% \begin{wrapfigure}{r}{0.7\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{figure/rootcause-datatype.pdf}
%     \caption{A Python-C CLB case with the root cause of 'data type error'~\cite{casestudy_datatype}.}
%     \label{fig:root-data-type}
% \end{wrapfigure}

\textbf{Illustration.}
As depicted in Figure~\ref{fig:root-data-type}, a critical concern emerges when the variable {\tt offset} is initially defined as an {\tt int} (line c16) while the data is transmitted along the cross-language flow from Python. 
When {\tt offset} is used to navigate through these large data arrays, its insufficient range could lead to incorrect memory access. 
% For instance, if an {\tt offset} calculation results in a value that exceeds the maximum or minimum value an int can hold, it might wrap around to a negative value or overflow, leading to an attempt to access a memory location that is out of bounds of the intended data structure. 

This scenario underscores the significance of appropriately managing data types. To rectify this bug, the solution involves defining the variable {\tt offset} with the type {\tt npy\_intp}, which is designed to hold any array index in NumPy (A Python library). This ensures compatibility with large arrays and reduces the potential for overflow or wrap-around errors. 


 
% As depicted in Figure~\ref{fig:root-data-type}, a critical concern emerges when the variable {\tt offset} is initially defined as int (line c16), while the offset of type {\tt long} is transmitted along the data flow from Python, carrying a size surpassing 2GB. In this scenario, a precarious situation arises where an overflow of {\tt bytesread} at line c10 becomes possible, triggering an inexhaustible loop.
% This scenario underscores the significance of appropriately managing data types and ensuring compatibility across the programming interfaces. An oversight in data type compatibility, as demonstrated in this example, can lead to severe runtime issues, such as infinite loops, compromising the functionality and stability of the system.
% To rectify this bug, it is recommended to redefine the variable {\tt bytesread} with the type {\tt Py\_off\_t} (line c3). This adjustment ensures that the two compared variables possess the same data type, and their bit-width aligns with the functional requirements.



\vspace{-4pt}
\find{
% In this study, we analyzed the root causes of cross-language bugs and found thirteen categories. 
The three primary root causes of CLBs were logic errors, boundary conditional errors, and data type errors. 
The number of bugs rooted in logic errors far dominated over those due to any other categories of root causes. 
%The quantity of bugs associated with memory safety exceeded the total of the second most common category, namely logic errors, by a multiplicative factor of two.

% The most prevalent bug was memory safety, emphasizing the significance of correct memory management, especially when dealing with languages that manage memory differently. Logic errors underline the need for comprehensive testing and code reviews to ensure the program behaves as intended. Data type bugs stress the importance of accurate understanding and handling of data types when data is passed between languages, while boundary conditional errors highlight the need to handle edge cases correctly.
}


==> RQ-symptom-cai.tex <==
\subsection{RQ1: Symptoms of Multilingual Bugs}\label{RQ1}
% As shown in~\ref{tab:symptoms}, 
We found five main types of symptoms of multilingual bugs: 

{\ul{Sym1: Crash/abort (70).}} 
%This is the most dominant symptom, which is a critical one as it means that 
The program stops/exits unexpectedly. 
We also found that the vast majority of these crashes are related to memory safety issues (52), followed by boundary conditional errors (3) and then input/output handling issues (3). 
%This suggests that a large portion of these bugs might be related to improper memory management of foreign language objects, such as incorrect allocation or deallocation, or incorrect use of pointers. 
%In essence, preventing these crashes primarily involves robust, well-tested coding practices, proper use of APIs and functions, meticulous memory management, and effective error and exception handling.

{\ul{Sym2: Error messages (16).}} 
The program provides explicit notifications that it encounters a situation it cannot handle or when an operation fails. 
The symptom includes type errors, import errors, value errors, etc., which are related to issues like data type inconsistencies (6), API/function misuse (2), etc. 
%Error messages can be a diagnostic tool for developers, helping them understand where and why a problem occurred. Managing these effectively requires understanding and using APIs correctly, and ensuring data types are used consistently and correctly throughout the code.

{\ul{Sym3: Data corruption (11).}} 
%There are 11 cases of this symptom. It refers to errors in computer data that occur during writing, reading, storage, transmission, or processing, which
The program makes unintended changes to the original data. 
The related issues mainly include data type errors (5), logic errors (3), and API/function misuse (1). %This might indicate that the data is being manipulated incorrectly within the application, potentially due to misunderstanding the function's expected inputs/outputs, or errors in programming logic. These issues highlight the importance of thoroughly understanding data types, the correct usage of APIs, and maintaining stringent checks on logical flow in the code. Careful attention to these aspects can help prevent corruption and maintain the integrity of data.

{\ul{Sym4: Performance bottleneck (7).}} 
The performance or capacity of the entire system is limited by one or more of its components. 
We further found the related issues mainly concern 
%This can drastically reduce the performance of the software. The primary cause is 
resource management errors (4) and API/function misuse (2). 
%Addressing performance bottlenecks involves optimizing resource management, which could include more efficient memory usage, streamlining database queries, or effective task distribution among available processors. Additionally, correct usage of APIs or functions, and proper logical flow can prevent performance impediments, leading to faster, more efficient software.

{\ul{Sym5: Deadlock/hang (4).}} 
%This symptom only gets 4 cases. It is a particularly critical issue in concurrent programming. Deadlocks occur when 
Two or more operations in the program endlessly wait for the other to complete, or a process becomes unresponsive due to waiting indefinitely for some condition to be met. 
The associated issues are mainly concerned with improper exception handling (2) and 
API/function misuse (1). 
%Avoiding these situations involves careful design of concurrent processes, ensuring that dependencies between processes don't create cycles and that exception handling is robust enough to prevent indefinite waiting conditions, thereby ensuring smooth and responsive system operation.

In other cases, we could not determine the symptoms because the issue description/discussion does not provide the necessary information, nor does the commit message or code comment. 
%As a side note, here is that 
Moreover, we could not find necessary resources for actually running the program to 
reproduce the bugs (hence observing the symptoms by ourselves). 
There is a clear need for improvement in the reporting/documentation quality (at least via GitHub issues) of multilingual bugs. 

In all, symptoms of multilingual bugs do not appear to be unique or specific to multilingual software. 
However, as we revealed later, the associated issues and underlying root causes are often 
indeed specific to multilingual code (e.g., the type errors with foreign data objects and misuse of cross-language APIs/functions). 

\find{
Symptoms of the studied multilingual bugs include \textit{crash/abort}, \textit{error messages}, \textit{data corruption}, \textit{performance bottleneck}, and \textit{deadlock/hang}, which 
are commonly associated with issues like data type errors and API/function misuse. 
%The mitigation of multilingual bugs' symptoms primarily revolves around specific strategies. Preventing crashes or aborts requires meticulous memory management and correct use of APIs. Error messages, a critical diagnostic tool for developers, can be effectively managed by consistent use of data types and proper API utilization. To prevent data corruption, understanding the correct usage of APIs and maintaining stringent checks on logical flow in the code is key. Performance bottlenecks can be addressed by optimizing resource management and ensuring the correct usage of APIs or functions. Avoiding deadlocks or hang situations involves careful concurrent process design and robust exception handling. 
}

==> RQ-symptom.tex <==
\subsection{RQ1: Symptoms of multilingual bugs}\label{RQ1}
% As shown in~\ref{tab:symptoms}, 
We first summarize the symptoms of multilingual bugs.

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{The distribution of multilingual bugs symptoms}
%     \begin{tabular}{l|r}
%     \toprule
%     Symptom & \multicolumn{1}{l}{Total} \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{Crash/Abort} & \cellcolor[rgb]{ 1,  1,  1}70 \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{error msg} & \cellcolor[rgb]{ 1,  1,  1}16 \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{Data Corruption} & \cellcolor[rgb]{ 1,  1,  1}11 \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{Performance Bottleneck} & \cellcolor[rgb]{ 1,  1,  1}7 \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{DeadLock/Hang} & \cellcolor[rgb]{ 1,  1,  1}4 \\
%     \midrule
%     \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{14.355em}|}{Undecidable type} & \cellcolor[rgb]{ 1,  1,  1}108 \\
%     \midrule
%     Total & 216 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:symptoms}%
% \end{table}%

\subsubsection{Symptoms:} Multilingual bugs exhibit 6 types of symptoms:
\underline{\textbf{Sym1: Crash/Abort (70).}} This symptom is a significant category, as they cause programs to stop or exit unexpectedly. The vast majority of these crashes are related to memory safety issues(52), followed by boundary conditional errors(3) and input and output handling issues(3). This suggests that a large portion of these bugs can be related to improper memory management of host language objects, such as incorrect allocation or deallocation, or incorrect use of pointers. In essence, preventing these crashes primarily involves robust, well-tested coding practices, proper use of APIs and functions, meticulous memory management, and effective error and exception handling.

\underline{\textbf{Sym2: Error messages (16).}} This symptom, with 16 occurrences in our study, represents explicit notifications provided by the software when it encounters a situation it cannot handle or when an operation fails. The symptom includes type errors, import errors, value errors, etc. They often point to issues like data type inconsistencies(6), API/function misuse(2), etc. Error messages can be a diagnostic tool for developers, helping them understand where and why a problem occurred. Managing these effectively requires understanding and using APIs correctly, and ensuring data types are used consistently and correctly throughout the code.

\underline{\textbf{Sym3: Data Corruption (11).}} There are 11 cases of this symptom. It refers to errors in computer data that occur during writing, reading, storage, transmission, or processing, which introduce unintended changes to the original data. From our analysis, these mainly arise due to data type errors(5), logic errors(3), and API or function misuse(1). This can indicate that the data is being manipulated incorrectly within the application, potentially due to misunderstanding the function's expected inputs/outputs, or errors in programming logic. These issues highlight the importance of thoroughly understanding data types, the correct usage of APIs, and maintaining stringent checks on logical flow in the code. Careful attention to these aspects can help prevent corruption and maintain the integrity of data.

\underline{\textbf{Sym4: Performance Bottleneck (7).}} There are 7 cases related to this type. It represents situations where the performance or capacity of an entire system is limited by a single or limited number of components. This can drastically reduce the performance of the software. The primary cause is Resource Management Errors(4), and API or function misuse(2). Addressing performance bottlenecks involves optimizing resource management, which could include more efficient memory usage, streamlining database queries, or effective task distribution among available processors. Additionally, correct usage of APIs or functions, and proper logical flow can prevent performance impediments, leading to faster, more efficient software.

\underline{\textbf{Sym5: DeadLock/Hang (4).}} This symptom only gets 4 cases. It is a particularly critical issue in concurrent programming. Deadlocks occur when two or more operations are each waiting for the other to complete, creating a circle of dependencies that can never be fulfilled. Hangs, on the other hand, occur when a process becomes unresponsive because it's waiting indefinitely for some condition to be met. Most of these are due to improper exception handling(2) and API or function misuse(1). Avoiding these situations involves careful design of concurrent processes, ensuring that dependencies between processes don't create cycles and that exception handling is robust enough to prevent indefinite waiting conditions, thereby ensuring smooth and responsive system operation.

\underline{\textbf{Sym6: Undecidable type (108).}}
There are many commits' symptoms that are "Undecidable type" in my bug analysis is understandable given the following circumstances. We are conducting a manual analysis without the ability to run or reproduce each bug, relying solely on commit issues and code inspections for information. This approach naturally leads to ambiguity in certain cases, especially when dealing with complex bugs or when there's a lack of clear error messaging. Additionally, the quality of documentation, including commit messages and issue descriptions, can vary, further obscuring the true nature of some bugs. The combination of these factors—manual analysis, lack of execution context, the complexity of bugs, and inconsistent documentation—results in a large number of bugs being categorized as "Undecidable type", serving as an umbrella category for those cases that are difficult to pin down precisely. Despite its ambiguity, this category still offers valuable insights, hinting at areas where more specific error handling and reporting could improve the clarity of the system's behavior.


%---------------------------------------------------
%We can consider use following aspects to justify
%---------------------------------------------------
% Manual Analysis: The approach of manual analysis implies a human-driven process, where the interpretation of the bug, its causes, and its symptoms are dependent on the analyst's understanding. As such, ambiguous or complex bugs can be more likely to be classified under a broad category like "Undecidable type", especially when there's a lack of clear or explicit error messaging.

% Lack of Direct Execution: Since we are not able to run or reproduce each bug, we are relying on commit issues and code inspection to determine the symptom. Often, the type or nature of a bug becomes clear only when the code is executed and the error or malfunction is observed directly. In the absence of this direct evidence, it can be difficult to definitively decide the bug type, leading to a higher count of "Undecidable type" bugs.

% Variety and Complexity of Bugs: Bugs can be diverse and complex, arising from various programming constructs and scenarios. This complexity, coupled with the absence of a run-time environment, could lead to cases where it is not immediately clear what the exact issue is, making the "Undecidable type" a reasonable category for these cases.

% Documentation Quality: The quality of commit messages and issue descriptions also plays a significant role. If the developers who committed the fixes did not provide clear descriptions of the symptoms, it would be difficult to categorize the bug accurately.

\find{
The mitigation of multilingual bugs' symptoms primarily revolves around specific strategies. Preventing crashes or aborts requires meticulous memory management and correct use of APIs. Error messages, a critical diagnostic tool for developers, can be effectively managed by consistent use of data types and proper API utilization. To prevent data corruption, understanding the correct usage of APIs and maintaining stringent checks on logical flow in the code is key. Performance bottlenecks can be addressed by optimizing resource management and ensuring the correct usage of APIs or functions. Avoiding deadlocks or hang situations involves careful concurrent process design and robust exception handling. 
}

==> abstract-cai.tex <==
%!TEX root = paper.tex
\begin{abstract}
Multilingual systems are prevalent and broadly impactful, but also 
complex due to the intricate interactions between the heterogeneous programming languages the systems are developed in. 
This complexity is further aggravated by the diversity of cross-language interoperability across different language combinations, 
resulting in additional, often stealthy 
\textit{cross-language bugs}.  
%which are often stealthier than those contained in individual languages. 
Yet despite the growing number of tools aimed to discover 
cross-language bugs, a systematic understanding of such bugs is still lacking. 
To fill this gap, we conduct the first comprehensive study of cross-language bugs, characterizing them in five aspects including their symptoms, locations, manifestation, root causes, and fixes. 
%Assisted by a new static cross-language analyzer we developed, 
Through detailed analysis of 400 cross-language bugs in real-world multilingual projects classified from 54,356 relevant code commits in their GitHub repositories, we revealed not only bug characteristics of those five aspects but also how they compare between two top language 
combinations in the multilingual world (Python-C and Java-C). 
In addition to the empirical findings as well as 
its enabling tools and datasets, 
we also provide practical recommendations regarding 
the prevention, detection, and patching of cross-language bugs. 

% Developing a system using multiple %programming 
% languages is a norm in modern software practice, readily justified by the benefits of combining the strengths of individual languages. Yet this practice also brings about even greater quality-assurance challenges than using a single language due to the potentially additional and more complex bugs induced by the interaction between different languages (i.e., \textit{multilingual bugs}). 
% Yet despite existing relevant studies,  
% %on multi-language software and bugs in them, 
% there remains a lack of comprehensive understanding of real-world multilingual bugs. 
% %which are induced by cross-language code behaviors. 
% In this paper, we present the first in-depth study of such bugs, with a focus on systems built in Python and C as primary languages given the prevalence and impact of Python-C software. 
% Based on our extensive automated and manual analyses of 216 multilingual bugs in real-world Python-C projects on GitHub, 
% we obtained novel findings on their common \textit{symptoms}, introducing \textit{locations}, 
% \textit{manifestation} characteristics, \textit{root causes}, and \textit{fixes}. 
% These results further led to actionable insights into 
% practical strategies on multilingual bug prevention, detection, testing/debugging, and patching. 
\end{abstract}



% \begin{abstract}
% Developing a software system using multiple %programming 
% languages has become a norm in modern software practice, readily justified by the benefits of combining the strengths of individual languages. Yet intuitively this practice %(noted as \textit{multilingual development}) 
% also brings about even greater quality-assurance challenges than using a single language because of the potentially additional defects induced by the interaction between different languages. However, up to this date, we have little knowledge about such defects and there is a critical lack of tool support for multilingual developers to diagnose those bugs. To fill these gaps, in this paper we present the first in-depth study of real-world multilingual bugs, with a focus on systems built in Python and C as primary languages given the prevalence and impact of Python-C systems. Based on our extensive automated and manual analyses of 23 Python-C projects on GitHub and 352 real-world multilingual-bug-fixing commits (identified out of 60,180 code commits in those projects), we gained novel understandings and insights on the root causes, structural patterns of code location and context, and common fixing strategies of real-world multilingual bugs in practice. Following some of these insights, we further developed {\tech}, a learning-based line-level bug-detection technique and tool for localizing cross-language code defects, as a first step towards practical fault diagnoses for multilingual software. Using a pre-trained CodeT5 model, {\tech} features a novel relative position encoding scheme immediately informed by the strong relevance (as found in our study) of cross-language API calls to multilingual defects, which allows it to attend to code lines that are most likely responsible for cross-language faults. We have implemented {\tech} and applied it to 786 real-world Python-C functions. Our results demonstrate the merits of {\tech} for diagnosing multilingual bugs with 53.82\% top-5 precision, %and 70\% recall on overall average, 
% hence its superiority (123.81\% higher precision) %and 121.2\% higher recall) 
% over a state-of-the-art peer technique and an ablated version of {\tech} based on the original CodeT5 transformer.
% \end{abstract}

%\begin{IEEEkeywords}
%Software Vulnerability, Vulnerability Detection, Fair Comparison
%\end{IEEEkeywords} 



==> background-cai.tex <==
\section{Background}\label{sec:background}
A multilingual system consists of multiple code units each written in a different language, referred to as a \textit{language unit}~\cite{haoran22fsenier}, which   must interact with at least one of the other units. 
Software simply has multiple languages involved in 
its construction yet without interactions among its language units is not considered multilingual software in %, hence out of scope of, 
our study. 

There are different ways in which two language units can interact/interoperate (i.e., \textit{language interfacing mechanism}~\cite{wen22fsetool}). 
A dominating mechanism among various language combinations, especially Python-C and Java-C, is \textit{Foreign Function Interface (FFI)}~\cite{li2023multilingual}, provided by a programming language to allow code written in that language to call functions written in another language~\cite{wen22fse,lee2020broadening,grichi2020impactjni}. 
For Java-C, for instance, the most commonly used FFI %instance 
is the Java Native Interface (JNI).

%When using an FFI for language interfacing, 
Given an FFI, 
the interoperation between the two languages is realized by the FFI via 
a set of functions each written in one language $L1$ but either \textbf{(a)} to be called in another language $L2$ or to \textbf{(b)} serve the purpose of accessing (e.g., the capability offered by or data originated in) $L2$ from within an $L1$ unit.  
Each of these functions is referred to as a \textit{cross-language function}. 
In particular, if such a function is exposed/externalized for public use by the language other than the one it is written in, we also call it a \textit{cross-language API}. 

There are two main classes of cross-language APIs: 
native function and foreign function~\cite{yang2023demystifying}. 
In the situation (a) above, the API is typically written by the application developer in $L1$ but called in $L2$; this API is considered a \textit{native function} and accordingly $L1$ is considered a \textit{native language}. 
In the situation (b) above, the API is usually written by the language ($L2$)'s developer in $L1$ and also to be called in $L1$; this API is considered a \textit{foreign function} and $L2$ is considered a \textit{foreign language}. 
For instance, in Python-C and Java-C projects, C is a native language and Python and Java are foreign languages. 

% Also, non-API cross-language functions,  %that are \textit{not} cross-language APIs 
% referred to as \textit{NAX functions}, 
% are not uncommon---they often exist to serve as helper functions 
% to immediately support the functionalities of related cross-language APIs. 
% NAX functions are usually called by, but can also call, related 
% cross-language APIs. 




%In this paper, we focus on multilingual bugs in Python-C projects. 


% \subsection{Multi-Language Software and Multilingual Development}\label{ssec:mlmd}\vspace{-0pt} 

% \textbf{Multi-language software} utilizes multiple computer languages, irrespective of their classifications such as programming, modeling, or descriptive. In such systems, the code authored in each distinct language, also referred to as a language unit, is integral to the overall functionality of the system. The practice of creating such software, which incorporates various languages, is commonly known as \textbf{multilingual development}.


% \subsection{Language Interfacing Mechanism}\label{ssec:intmech}\vspace{-0pt}

% \textbf{Foreign Function Interfaces (FFIs)}: These are mechanisms provided by a programming language that allow code written in that language to call functions or procedures written in another language. FFIs are typically used when you want to call a function in a library written in a different language, or when you need to interface with low-level system APIs that are exposed through a language like C.

% \textbf{Cross-Language APIs}: These are interfaces designed to allow communication between software components written in different programming languages. Cross-language APIs can be implemented in various ways, but the common characteristic is that they provide a set of functions, procedures, data structures, or classes that can be called from another language. In C-Python projects, the APIs provided by FFI, Cython, ctypes, SWIG, and other interaction methods can all be referred to as cross-language APIs.

==> background.tex <==
\section{Background}\label{sec:background}
This section defines key concepts and terminologies used in
the rest of this paper that are necessary for understanding it

\subsection{Multi-Language Software and Multilingual Development}\label{ssec:mlmd}\vspace{-0pt} 

\textbf{Multi-language software} utilizes multiple computer languages, irrespective of their classifications such as programming, modeling, or descriptive. In such systems, the code authored in each distinct language, also referred to as a language unit, is integral to the overall functionality of the system. The practice of creating such software, which incorporates various languages, is commonly known as \textbf{multilingual development}.


\subsection{Language Interfacing Mechanism}\label{ssec:intmech}\vspace{-0pt}

\textbf{Foreign Function Interfaces (FFIs)}: These are mechanisms provided by a programming language that allow code written in that language to call functions or procedures written in another language. FFIs are typically used when you want to call a function in a library written in a different language, or when you need to interface with low-level system APIs that are exposed through a language like C.

\textbf{Foreign functions}: These are interfaces designed to allow communication between software components written in different programming languages. Foreign functions can be implemented in various ways, but the common characteristic is that they provide a set of functions, procedures, data structures, or classes that can be called from another language. In C-Python projects, the APIs provided by cffi, Cython, ctypes, SWIG, and other interaction methods can all be referred to as foreign functions.

==> bugdetection.tex <==
%!TEX root = paper.tex
\section{Detecting Multilingual Bugs}
%\sw{let us remove 'API-based' in all the references to our technique; because multilingual bugs in this paper are defined as based on cross-language APIs; we can say learning-based multilingual bug detection or just 'multilingual bug detection'}

\begin{figure*}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.9\linewidth]{figure/workflow.pdf}
	\caption{Overview of our multilingual bug localization technique {\tech}.}
	\label{fig:workflow}
	\vspace{-10pt}
\end{figure*}
In the previous sections, we understand the root causes, structural patterns of code location and context, as well as common fixing strategies of real-world multilingual bugs in practice. Given that multilingual bugs are prevalent and they have big impacts on multilingual software's stability and security, precisely locating multilingual bugs is crucial. In this section, we improve an existing technique for multilingual bug localization using our insights to show the \emph{usefulness} of our empirical findings. 

We hope to use a state-of-the-art technique that can easily apply our insights to show the usefulness of our empirical findings. Thus, the technique that we used to improve should have the following characteristics:
%Based on these insights, we hypothesis that an effective multilingual bug localization technique should have the following characteristics:
\begin{itemize}[leftmargin=*]
%\vspace{-3pt}
\item Since manual building the multilingual bug localization rules is difficult, the localization of multilingual bugs should be learning-based.
\item Since our insights show that some code elements (e.g., statements) are more relevant to the root causes of multilingual bugs, the technique should allow us to modify its focus on different code elements.
\item Since our task is multilingual bug localization, the technique should be able to understand the code syntactic and semantic information of different programming languages.
\end{itemize}

To satisfy the first characteristics, we did a literature review on learning-based software engineering (SE) techniques. Recently, deep learning (DL) based models are widely leveraged for SE tasks and they achieve big successes~\cite{liu2021reproducibility}. Among them, several different DL architectures are mostly widely used on SE tasks, including recurrent neural network (RNN)~\cite{medsker2001recurrent}, graph neural network (GNN)~\cite{zhou2020graph}, convolutional neural network (CNN)~\cite{li2021survey}, and Transformer~\cite{vaswani2017attention}. They achieve very good performance for different software tasks, including code generation~\cite{sun2020treegen},  code summarization~\cite{tang2021ast}, code translation~\cite{niu2022spt}, clone detection~\cite{zhang2021challenging}, and bug detection~\cite{zhu2022model,mecenero2022lightweight}. To show the usefulness of our insights on the state-of-the-art techniques for multilingual bug localization, we choose DL-based architectures as the candidate bases to improve.

To satisfy the second characteristic, we reviewed the several main-stream DL models above. Among them, Transformer uses the self-attention mechanism to learn the attentions between different elements (e.g., code tokens) in the model inputs~\cite{vaswani2017attention}. There are different designs for the self-attention mechanism. The original Transformer uses the encoding of the absolute position of the elements to bias the attention~\cite{vaswani2017attention}. Shaw et al.~\cite{shaw2018self} propose relative position encoding which uses the difference between token indexes to bias the attention. To make Transformer work better on programming languages, Peng et al.~\cite{peng2021integrating} propose TPTrans which integrates the paths on the abstract syntax tree (AST) of the code to bias the attentions. Given the flexibility of the Transformer attention mechanism design, we choose the Transformer architecture as the base to improve.

To satisfy the third characteristics, we hope that the Transformer model understands the code syntactic and semantic information before the training since the existing multilingual bug training data we can collect (<10K) may not be enough to train the model independently. Luckily, there are many pre-trained models based on Transformer which are proved to be effective on different domains of tasks (e.g., natural language processing ~\cite{chowdhary2020natural}, code understanding~\cite{niu2022spt}, code generation~\cite{sun2020treegen}). Among them, CodeT5~\cite{wang2021codet5} is the latest model which shows promising performance on semantic-aware code relevant tasks~\cite{fu2022vulrepair}. It has been pre-trained on millions of code samples of eight different popular programming languages, which means it has the capability to understand multilingual code syntactic and semantic information. Therefore, we finally choose CodeT5, a DL-based pre-trained Transformer model, as the base to improve the multilingual bug localization, to show the usefulness of our empirical findings. 

In our empirical findings above, we notice that multilingual API calls are often relevant to the root causes of multilingual bugs. However, while they are relevant to multilingual bugs, they are not always the root causes of such bugs. Instead, the root causes of the bugs are often at the statements which have close control flow relationship to the multilingual API calls. Thus, besides focusing on the multilingual function calls, we also hope that the bug localization model focuses on those relevant statements. Therefore, to apply our insights to the localization model, we improve CodeT5 for multilingual bug localization based on multilingual API calls, which is our new technique -- \tech. 


\subsection{Overview}
Figure~\ref{fig:workflow} shows the overview of \tech. It has the following main steps:

First, we obtain the multilingual API control flow graph given a code sample. 
We obtain the general control flow graph using a multilingual code parser Joern~\cite{yamaguchi2014modeling}.
On the graph, we filter the nodes which have multilingual API calls (MC), and get the control flow distance from the tokens to those API calls.

%extract the statements which have control flow dependencies to the multilingual API calls. All the tokens on those statements are marked with the control flow distance between the statements to the the respective multilingual API calls.

Then, we input the code sample to \tech~to fine-tune and test the model like the usage of the model is designed to be. We formulate the localization as a text-to-text prediction: the inputs are the code samples and the expected outputs are the lines (the whole line, not the line index) of the multilingual bugs. CodeT5 computes the attention with the bias computed from traditional relative position encoding, which is based on the differences between token indexes~\cite{shaw2018self}. However, to improve the performance of multilingual bug localization, we add a multilingual API relative position encoding for the bias.
%for the pairs of the marked tokens and their respective API calls' names, we use their control flow distances to compute another relative position encoding. 
The sums of the traditional relative position encoding and our API call-specified relative position encoding are used for the bias of the attention.

Finally, after the training, \tech~is expected to output the buggy lines given a sample. We use beam search to generate the possible buggy lines and compare them with the ground truths to evaluate the technique.

Next, we describe the design of \tech~in details.

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.8\linewidth]{figure/illustrate.pdf}
	\caption{An example of multilingual API call control flow.}
	\label{fig:illustrate}
	\vspace{-10pt}
\end{figure}

\subsection{Line-level multilingual bug localization}
\noindent
\textbf{Multilingual API call control flow graph extraction.} Given a code sample, we use a code parser to extract the control flow graph. There are many tools which can parse the code and extract the control flow graphs. We choose to use Joern~\cite{yamaguchi2014modeling} because: (1) it can parse the code and get the control flow graphs without compiling the whole projects, which saves much time and storage for us; (2) Joern supports parsing different programming languages which allows us to do multilingual code analysis. 

We first use Joern to parse the code and extract the general control flow graph given a code sample. 
A control flow graph is a multi-edge graph $g(V,E)$, 
where $V$ is a set of nodes which represent the statements in the code sample, 
and $E$ is a set the edges connecting the nodes in $V$, 
which represent the control flow relationship between different statements. 
Particularly, the control flow graph starts from the beginning of the program, branches at the conditional statements (e.g., if, for, while, switch) and terminates at the end of the program.

With the control flow graph, we then extract the nodes with multilingual API calls in the graph, named multilingual call (MC) nodes. The set of multilingual API calls are collected when we do the empirical study. Then, we do a graph traversal and query the nodes which can reach the MC nodes or can be reached by the MC nodes on the graph. These nodes are marked to be MC relevant. Each MC relevant node has a control flow distance to the respective MC node. The distances are collected as multilingual API relative positions and will be used in the API call-specified relative position in the Transformer model of \tech.

Figure~\ref{fig:illustrate} shows an example. The code is parsed into a control flow graph (CFG) using Joern. Then, we check each statement and notice that there is a multilingual API call {\tt Py\_ABS} in line/node 6 (marked green). Then we traversal the graph and get the distance from the multilingual API call to each node. For instance, the distance from the API call to line/node 2 (marked blue) is -2, thus each token in line 2 has an API call-specified relative position -2 to the API call token {\tt Py\_ABS}. The API call-specified relative positions of the tokens in line 7 can be computed in a similar way. These multilingual API relative positions will be used for biasing the Transformer attentions as follows.

\vspace{5pt}
\noindent
\textbf{Transformer-based bug localization.} 
In this phase, we improve the pre-trained Transformer-based model CodeT5 with the extracted multilingual API call control flow information. CodeT5 is a typical Transformer model where self-attention is one of the core components of the model. In short, the attention module uses \emph{key} and \emph{value} pairs to \emph{query} a dictionary which can be computed as follows:

\begin{equation}
Attention(Q,K,V)=softmax(\frac{QK^T}{\sqrt{d}})V
\end{equation}


where $Q,K,V$ are the previous layer hidden representations of query, key, and value respectively and $d$ is the dimension of the representations. For simplicity, we rewrite and expand the equation to better explain it:

\begin{equation}
z_i=\sum_{j=1}^{n}\frac{exp(a_{ij})}{\sum_{j'=1}^{n}exp(a_{ij'})}(x_jW^V+r_{ij}^V) 
\end{equation}


where $a_ij$ is the attention between the i-th token and the j-th token and can be further expanded as 

\begin{equation}
    a_{ij}=\frac{1}{\sqrt{2d}}(x_iW^Q)(x_jW^K+r_{ij}^{K})^T+\frac{1}{\sqrt{2d}}(a_i^Q)(a_j^K)^T
\end{equation}

To be consistent with CodeT5, in Equation (2) and (3), we have added the absolute position encoding which are represented as $a_i^Q$ and $a_j^K$ as well as the relative position encoding which are represented as $r_{ij}^V$ and $r_{ij}^K$.

CodeT5 uses traditional absolute and relative position encoding where the encoding is based on the indexes of the tokens in the input sequence. Specifically, absolute position encoding has $a_{i}^Q=p_iA^Q$ and $a_{j}^K=p_jA^K$ where $p_i$ and $p_j$ are the sine and cosine functions of the positions i and j and $A^Q$ and $A^K$ are the weight matrices of the encoding~\cite{vaswani2017attention}. The relative position encoding has $r_{ij}^V=(i-j)R^V$ and $r_{ij}^K=(i-j)R^K$ where $R^V$ and $R^K$ are the weight matrices of the encoding~\cite{wang2021codet5}. 

Since the traditional position encoding directly uses token indexes to compute the encoding, the attention layer may not be able to capture the syntactic and semantic position relationship between the tokens in the code. In our empirical findings, the multilingual API calls and the statements with close control flow to these API calls are important for the root causes of the multilingual bugs. Thus, we add our API call-specified relative position encoding to the model:

\begin{equation}
z_i=\sum_{j=1}^{n}\frac{exp(a_{ij})}{\sum_{j'=1}^{n}exp(a_{ij'})}(x_jW^V+r_{ij}^V+r_{ij}^{V_{API}}) 
\end{equation}
\begin{equation}
    a_{ij}=\frac{1}{\sqrt{2d}}(x_iW^Q)(x_jW^K+r_{ij}^{K}+r_{ij}^{K_{API}})^T+\frac{1}{\sqrt{2d}}(a_i^Q)(a_j^K)^T
\end{equation}

\vspace{5pt}
where $r_{ij}^{V_{API}}$ and $r_{ij}^{K_{API}}$ are the API call-specified relative position encoding. We define them as follows:

\begin{equation}
r_{ij}^{V_{API}}=API\_ctrl\_dist(i,j)R^{V_{API}}
\end{equation}
\begin{equation}
r_{ij}^{K_{API}}=API\_ctrl\_dist(i,j)R^{K_{API}}
\end{equation}


where $API\_ctrl\_dist(i,j)$ is the multilingual API control flow distance between the i-th and j-th tokens which is defined as:


\begin{equation}
\begin{footnotesize}
API\_ctrl\_dist(i,j)=
  \begin{cases}
    ctrl\_dist(i,j), & if\ ith\ or\ jth\ token\ is\ a\ MC \\
    0, &otherwise
  \end{cases}
\end{footnotesize}
\end{equation}


where $ctrl\_dist(i,j)$ is the control flow distance between the respective nodes of the i-th and j-th tokens as depicted in Figure~\ref{fig:illustrate}.

Since CodeT5 is a pre-trained text-to-text model for multiple programming languages, we directly fine-tune \tech~for multilingual bug localization. We pre-process our bug samples into a fine-tuning dataset $\mathcal{D}=\{(f_i,s_i)\}$ where each sample consists of a buggy function $f_i$ and a respective ground-truth buggy line $s_i$ to be predicted.
Both $f_i$ and $s_i$ are in text form to fit the text-to-text model. To fine-tune the model with parameters $\theta$, we minimize the following negative log-likelihood loss to maximize the likelihood estimation:

\begin{equation}
L(\mathcal{D};\theta)=\sum_{i=1}^{N}-log\ p(s_i|f_i;\theta)
\end{equation}

After the fine-tuning, \tech~is expected to output the buggy line given a multilingual buggy function. Since the model is probabilistic, it allows to predict multiple buggy lines with beam search size greater than 1. When setting the beam search size K, \tech~ output K lines that are the most likely ones to be buggy. Later we will use different beam search sizes to evaluate \tech~and the baseline techniques.

\subsection{Evaluation}
In this section, we evaluate \tech~as well as the original CodeT5 and another DL-based bug localization technique on our collected real-world multilingual bug dataset. We first describe the dataset, the baselines, as well as the metrics for evaluation. Then, we show the evaluation results and use several case studies to explain the results. Finally, we briefly discuss the insights we obtain from our technical experiments. 

\textbf{Dataset.}
We use the inter-language bug commits collected which are depicted in Figure~\ref{fig:datacollect} to build our evaluation dataset. Each bug commit is a pair of code which involves the versions before and after the commit. Based on this, we use the diff command provided by Git to get the lines modified and the modified lines are the buggy lines we want to locate. The commits are based on whole source code files and the code in the files is usually very long (e.g., > 5000 tokens). Since the Transformer model is sensitive to the input text length ~\cite{nong2022generating}, inputting the whole files may not be feasible. Thus, we extract the respective functions where the modified lines are in, and thus the buggy functions are the actual inputs to the model. For each sample, the expected output (ground truth) is the buggy line in the function. If there are multiple buggy lines, we use the first buggy line as the ground truth since it is usually the most important one and the rest of the lines may be directly located after it~\cite{li2021fault}.

We finally collected 7864 samples which are in C and Python languages for the dataset. We split the dataset 8:1:1 for training (fine-tuning), validation, and testing. 

\textbf{Baselines.}
Since \tech~is improved from CodeT5, we use the original \textbf{CodeT5} as the baseline. We use the same dataset to fine-tune the original CodeT5 for comparison.

However, CodeT5 is not directly designed for bug localization, thus we select another bug localization technique as the baseline for comparison. There are many state-of-the-art machine learning-based bug localization techniques, such as LineVul~\cite{fu2022linevul}, DeepFL ~\cite{li2019deepfl}, DeepRL4RL~\cite{li2021fault}. However, many of them need test cases~\cite{li2021fault} or only detect bugs at function level~\cite{li2019deepfl}. Thus, we select \textbf{LineVul} as the baseline because it supports line-level bug localization and only takes the buggy code to automatically output the possible buggy lines. It is also a technique using pre-trained model CodeBERT~\cite{feng2020codebert} to do the bug prediction/localization fine-tuning and then use the attention scores on the tokens of the testing samples to locate the buggy lines. Since LineVul needs non-buggy samples to learn the bug localization, we use the remaining commits collected in Figure~\ref{fig:datacollect} which are not in the inter-language bug type. We use the same way to pre-process the commits into a non-buggy dataset which has 17665 samples. The buggy training/validation data we used for \tech~and the non-buggy dataset are together used for training LineVul, but we keep the testing set the same for fair comparison.

\textbf{Metrics.}
Following other prior bug detection/localization studies~\cite{li2019deepfl,li2021fault}, we use \textbf{recall at top-K} and \textbf{precision at top-K} as the metrics to evaluate \tech~and the baselines. Specifically, when we set the beam search size as K, \tech~ outputs K predictions which are most likely to be the buggy lines. Once one of the number predictions matches the ground truth, we mark that sample to be true positive. The number of true positives is the recall at top-K, and the percentage of true positives in all the testing samples is the precision at top-K. We report top-1, top-3, and top-5 following the prior works~\cite{li2019deepfl,li2021fault}.

\textbf{Implementation.} We use the pre-trained model CodeT5 provided by HuggingFace~\cite{wolf2019huggingface} as the base and develop \tech~by directly modifying its source code. We use the default hyper-parameters of CodeT5 for training and testing. We perform our experiments on a workstation with an AMD Ryzen Threadripper 3970X (3.7GHz) CPU with 32 Cores, an Nvidia GeForce RTX 3090 GPU, and 256GB memory.

\begin{table}[t]
\center
\caption{Effectiveness of \tech~and the baselines (786 testing samples)}
\vspace{0pt}
\scalebox{0.8}{
\begin{tabular}{cccc}
    \hline
    \textbf{Technique} & \textbf{\tech} & \textbf{CodeT5} & \textbf{LineVul}\\
    \hline
    \textbf{Recall at Top-1} & 286 & 265 (7.92\%$\uparrow$) & 63 (353.97\%$\uparrow$) \\
    \textbf{Recall at Top-3} & 389  & 375 (3.73\%$\uparrow$) & 144 (170.14\%$\uparrow$) \\
    \textbf{Recall at Top-5} & 423 & 411 (2.92\%$\uparrow$) & 189 (123.81\%$\uparrow$) \\
    \hline
    \textbf{Precision at Top-1} & 36.39\% & 33.72\% (7.92\%$\uparrow$) & 8.02\% (353.97\%$\uparrow$) \\
    %\hline

    \textbf{Precision at Top-3} & 49.49\% & 47.71\% (3.73\%$\uparrow$) & 18.32\% (170.14\%$\uparrow$) \\
    %\hline

    \textbf{Precision at Top-5} & 53.82\%  & 52.29\% (2.92\%$\uparrow$) & 24.05\% (123.81\%$\uparrow$) \\

    \hline
    \end{tabular}}
\vspace{-10pt}
\label{tab:result}
\end{table}

\textbf{Results.}
Table~\ref{tab:result} shows the effectiveness of \tech~and the baselines on the 786 testing samples. The table shows the recall and precision of Top-K as we discussed before. The percentages in the parentheses show the improvement of \tech~compared to the two baselines. 

We notice that \tech~significantly outperforms the two baselines, with 2.92\%, 3.73\%, and 7.92\% improvements compared with the original CodeT5, and with 123.81\%, 170.14\%, and 353.97\% improvements compared with LineVul. This indicates that \tech~works better on multilingual bug localization since our added API call-specified relative position encoding builds the connection between the tokens and the multilingual API calls which helps the model find the buggy lines. 

In comparison, while CodeT5 also achieves promising effectiveness, its performance is a little bit lower than \tech. This is because it is pre-trained on millions of code samples covering eight different languages. The large pre-training dataset allows the model to comprehensively learn the syntactic and semantic features of different programming languages. Besides, CodeT5 leverages a bimodal dual generation as the pre-training task which helps a lot on the code translation task which translates code from one language to another language~\cite{wang2021codet5}. This is also a reason for the promising performance because CodeT5 has better understanding between different languages which is very useful for multilingual bug localization. 

However, CodeT5 uses traditional absolute and relative position encoding to bias the attention. It does not have programming language-specified position encoding and it simply uses the token indexes to compute position encoding. In this case, the code is treated as plain text and the syntactic and semantic features can be only learned by the hidden model parameters implicitly, which increases the difficulty for training. In comparison, \tech ~leverages the control flow graphs and focuses on the multilingual API calls, which explicitly supervises the model to pay attention to the statements that are more likely to be relevant to multilingual bugs. Therefore, \tech~outperforms the original CodeT5.

In comparison, LineVul fails to locate the buggy lines in many cases. It only achieves 8.02\%, 18.32\%, and 24.05\% precision at top-1, top-3, and top-5. One of the key reasons for the failure is that LineVul does not predict the buggy lines directly. It learns the difference between the buggy code and non-buggy code so that the model has more attention on the lines that can differentiate buggy and non-buggy code, which are usually the buggy lines. In this case, the learning of the localization is learned implicitly which significantly increases the training difficulty. 

Another key reason for the failure is that LineVul leverages CodeBERT as the pre-trained model. Compared with CodeT5, CodeBERT only pre-trains the encoder of the Transformer while CodeT5 pre-trains both the encoder and decoder~\cite{wang2021codet5}. Besides, while CodeBERT is also trained on different languages, it does not cover C, which is the programming language that many of our samples are in. Also, it does not leverage pre-training tasks like bimodal dual generation that help understand code semantics between different programming languages. These reasons make LineVul have disadvantages on multilingual bug localization.

\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/technique_case_study1.pdf}
	\caption{An example where \tech~succeeds while CodeT5 does not.
	}
	\label{fig:tech-case1}
	\vspace{-10pt}
\end{figure}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/technique_case_study2.pdf}
	\caption{An example where \tech~succeeds while CodeT5 does not.
	}
	\label{fig:tech-case2}
	\vspace{-10pt}
\end{figure}

\textbf{Case Studies.}
Next, we use two case studies to show the advantage of \tech. Figure~\ref{fig:tech-case1} shows an example where \tech~correctly locates line 3 (marked green) as the buggy line while the original CodeT5 locates line 5 (marked yellow). The bug is at line 3 because it is caused by not correctly checking {\tt self->pagerhist->max\_sz}. The max size checking should not use a simple constant {\tt MAX\_SIZE} but a secure checking function. \tech ~correctly locates line 3 as a multilingual bug spot because it leverages the control flow relationship between line 3 and line 5 which has multilingual API calls ({\tt PyBytes\_AS\_STRING and PyBytes\_GET\_SIZE}). Thus, while the buggy line has no multilingual API calls and the bug may be triggered at line 5 when executing the program, the control flow connection between line 3 and line 5 helps the model correctly locate the buggy line. However, the original CodeT5 simply learns that the lines with multilingual API calls are more likely to be buggy, which makes it fail on this example.

Figure~\ref{fig:tech-case2} shows another example where \tech~correctly locates line 11 as the buggy line while the original CodeT5 locates line 6. The bug is at line 11 because the parsed object from line 6 may not be correct and needs a sub-object by sub-object checking  before the assignment. The original CodeT5 locates line 6 because it is an if statement checking and the function is returned if the API call {\tt PyArg\_ParseTuple} does not execute correctly. However, since real bug is in the assignment statement at line 11 which has a close control flow relationship with line 6. The API call-specified position encoding helps \tech~build the connection and makes it succeed in this example.


\textbf{Discussion}
In the original CodeT5, the code is treated as a sequence of tokens and without considering the code syntactic and semantic structures. Thus, it may predict the results based on the token itself (e.g., identifier name) and the traditional position information from the token indexes (e.g., traditional absolute and relative position encoding). However, because of the complexity of the code structures, the traditional position information may be difficult for the model to learn the relationship between tokens. For example, each statement has different numbers of tokens. If the model only uses traditional position encoding, the syntactic and semantic distance between two statements may be confusing for the model because there is no regular token index pattern between them. In comparison, \tech~leverages control flow-based position encoding and is specified with multilingual API calls, making the model more likely to succeed on multilingual bug localization. 



==> casestudy.tex <==
%!TEX root = paper.tex

%\section{Case/Characteristics Studies}
\vspace{-4pt}
\section{Understanding Multilingual Bugs}
We intend to %comprehend the difficulties and issues 
understand multilingual bugs 
in Python-C projects via case studies. 
%developed in several languages. 
This type of case study can assist in identifying common patterns and causes of multilingual bugs and shed light on how to avoid them in future software development. The case study of multilingual defects can provide a comprehensive analysis of the bugs' root causes, the location of bugs, and the methods taken to fix them. This information is valuable for other developers and organizations. It can also provide a greater understanding of the intricacies of multilingual systems, which can inform future development best practices. In general, our case study on multilingual issues can enhance the quality and dependability of multilingual software and provide significant insights for future development.

%\noindent
We study the following aspects of multilingual bugs:

\begin{itemize}[leftmargin=12pt,topsep=2pt]
	\item \ul{\textit{What are the common root causes of multilingual code defects?}} This study will provide a basic understanding of real-world multilingual bugs and guide bug detection research.
	
	\item \ul{\textit{Where do multilingual code defects typically occur?}} This study will shed light on the context in which multilingual bugs may happen hence helping developers understand where to avoid such bugs; knowing the context also helps further bug detection, in particular, helping localize bugs.
	
	\item \ul{\textit{How are multilingual bugs fixed?}} This study will reveal the pattern of bug fixing and help inform the development of bug-repair techniques for multilingual code.
\end{itemize}

\noindent
The result of this study is shown in Table~\ref{tab:casestudy}.

\begin{table*}[htbp]
  \centering
  \caption{Categorization for Sections ~\ref{section:3.2} – ~\ref{section:3.4} }
    \includegraphics[width=0.9\linewidth]{figure/casestudy_table.pdf}
    \begin{tablenotes}
    \footnotesize
     \item * A single commit may be classified into multiple categories under these questions.
    \end{tablenotes}
  \label{tab:casestudy}%
\end{table*}%


\subsection{Study Data}
Considering the typically substantial time cost of manually inspecting even one commit, we randomly selected about 29\% of 352 bug-related inter-language commits, resulting in 102 commits that need to be manually confirmed in the case study. This sample size is statistically significant at 90\% CL and 6.75\% ME. 



\subsection{Root Cause of Multilingual Bugs}
\label{section:3.2}
There are many potential root causes for the multilingual bug, such as the incorrect implementation of API and not correctly handling data conversions between different languages. Another common cause is encountering problems when managing memory via other languages, which can result in segmentation faults.

Our study shows that only a couple of root-cause categories cover the majority of real-world multilingual bugs in our research. Detailed results are displayed in Table~\ref{tab:casestudy}.

%\vspace{-2pt}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/rootcause_bondary.pdf}
	\caption{A bug without value checking~\cite{casestudy_boundary}
	}
	\label{fig:rootcause-boundary}
	\vspace{-12pt}
\end{figure}

%\vspace{-2pt}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/rootcause_dataformat.pdf}
	\caption{A bug using the wrong type in foreign function~\cite{casestudy_format}
	}
	\label{fig:rootcause_dataformat}
	\vspace{-12pt}
\end{figure}

%\vspace{-2pt}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1\linewidth]{figure/rootcause_reference.pdf}
	\caption{A bug with a misused reference count~\cite{casestudy_reference}
	}
	\label{fig:rootcause-reference}
	% \vspace{-12pt}
\end{figure}
\vspace{0pt}

\underline{\textit{Missed boundary check for foreign function calls.}} 
%\noindent
24.51\% of the multilingual bugs in our study are caused by missing checking the boundary value of variables that foreign functions may return.

In a multilingual project, it is necessary to perform boundary checks to ensure the data remains within the correct range of values. Boundary checks should be performed whenever a foreign function uses the variables, or data is converted from one data type to another. 
\yu{This sentence does not make sense. As the format in Figure 2 is first used, please describe what '+' and '-' mean in the Code.} As shown in Figure~\ref{fig:rootcause-boundary}, the line starting with '+' represents the line added to fix the bug. The line starting with '-' represents the line deleted to fix the bug. The line without a symbol in front of it indicates that it has not been changed (This also applies to Figure~\ref{fig:rootcause_dataformat} and Figure~\ref{fig:rootcause-reference}). The foreign function PyDict\_GetItemString is used for retrieving the item in the Python dictionary associated with the key. If the key is not found in the dictionary, then the function returns "NULL" without raising an exception.\yu{Also, the description in Figure 2 needs rewriting. Current version is redundant and not clear.} However, the developer ignored that the foreign function can return NULL; that is, the corresponding key (string ”\_\_module\_\_“) was not found in the dictionary. Thus, the variable mod can be returned as NULL and then raise an issue.

\underline{\textit{Inconsistent data type returned by function calls.}} 
%
%\noindent
\yu{This sentence is also redundant and not clear. Please rewrite it.}
21.57\% of the multilingual bugs in our study are caused by a variable assigned a data type by a foreign function, but the type is not intended.

In this case,\yu{Please do not present continuous tense because it makes the sentense hard to read. Use simple present tense instead.} the developers may incorrectly convert values between languages or use the wrong data type for a parameter. As a result, the code may produce unexpected results, or errors may be thrown at runtime. Figure~\ref{fig:rootcause_dataformat} specifies that the foreign function\yu{This sentence is hard to read. Also, please do not use "can" in such case} PyTuple\_SET\_ITEM can insert a reference to an object. The value of "val" is converted from a 64-bit "ssize\_t" type to a 32-bit "long" type. However, in the 64-bit Python for Windows, it is problematic to convert 64-bit data to 32-bit. This may result in data loss because the value stored in the 64-bit data type is too large to fit into a 32-bit data type.

% Haoran note: merge 'initialization incorrectly' to 'data format issue'.
% \underline{\textit{Initialization incorrectly}} Around 10\% of the multilingual bugs in our study are caused by the initialization variable type being wrong, which leads to the argument in the interoperation process or the initial values assigned being incorrect or inappropriate for the intended use.

\underline{\textit{Cross-language reference count function misuse.}}\yu{What is reference count function?} 6.86\% of the multilingual bugs in our study are caused by the cross-language reference count manage functions missing or inappropriate using.
\noindent
\yu{what is reference count? what is manage function? Without the definition, I cannot understand the whole paragraph.}
This happens when an object's reference count, which keeps track of the number of references to that object, is not maintained correctly. The reference count error can lead to memory leaks, crashes, or other unpredictable errors in the multilingual project. Figure~\ref{fig:rootcause-reference} shows that the foreign function PyLong\_AsSsize\_t is called to convert variable "value" in type "ssize\_t" to type "long," but the variable "value" is not decremented in its reference count, causing a memory leak.

\underline{\textit{Others}}.\yu{Are these relevant to multilingual bugs? If so, please use some vocabulary to build the connection.} A variety of reasons cause the remaining  50  bugs. Some use the wrong algorithm. Some are caused by logic errors. For example, it is very complex for a break statement to jump out accurately in multiple for-loops, which easily leads to errors because of chaotic logic. So developers choose to use the goto statement after a foreign function to control the timing of jumping out to the specified location.

% \underline{\textit{Reference count misuse}} A reference count error in a multilingual project occurs when an object is incorrectly referenced, causing memory management issues. This happens when an object's reference count, which keeps track of the number of references to that object, is not maintained correctly. The reference count error can lead to memory leaks, crashes, or other unpredictable behavior in the multilingual project.

% \underline{\textit{Data format error}} A data format error in a multilingual project can occur when a variable or data structure is assigned a value of a different data type than what was intended. This can happen when a developer works with multiple programming languages, each with its syntax, data types, and type conversion rules. In these cases, the code may be incorrectly converting values between languages or using the wrong data type for a particular operation. As a result, the code may produce unexpected results, or errors may be thrown at runtime. These errors can be especially tricky to diagnose and fix, especially in a large multilingual project, as they may be caused by issues that are difficult to trace back to their source. 

% \underline{\textit{Data format error}} In a multilingual project, it is essential to thoroughly check the boundary values of input and output data, as different languages have different requirements for character encoding and string length. Failing to check these values properly can result in various types of errors, such as buffer overflows, integer overflows, and input validation errors.

% \underline{\textit{Out-of-range access}} An out-of-range access error in a multilingual project occurs when the program tries to access a memory location that is not within the bounds of an array or buffer. This can occur when the index used to access the array is too large or too small, causing the program to access memory that it should not have access to. This can result in unexpected behavior, such as crashing the program or causing incorrect results to be generated.

\subsection{Where Multilingual Bugs Often Occur}
\label{section:3.3}
\yu{You have discussed the rationale in the beginning of Section 3, please do not repeat because it causes logic redundant.}
We have studied the bug location and checked the context in each of the different commit versions to understand where the defects occur. 
There are mainly two patterns for the bug location. First, the bug occurs at the line where the cross-language API function is. Second, the bug appears at the lines following the foreign function.
% This information can guide code reviews, improve testing processes, and provide insight into best practices for developing multi-lingual software. And also, developers and organizations can better understand the complexities involved in multi-lingual systems and take steps to prevent similar defects in the future. Finally, researchers and developers can help improve the quality of multi-lingual software by creating new tools and processes specifically designed to address these defects. 
Detailed results are displayed in Table~\ref{tab:casestudy}.


\yu{The order of the paragraphs should be consistent with the one in the table.}
\underline{\textit{Right at cross-language API callsite}}.
Multilingual bugs most frequently happen at the statement 
%in which cross-language API is. 
where a cross-language API is called. 

\yu{Grammar issue.}
More specifically, the bug lies in that the type of argument used in the cross-language API is unsuitable for the intended purpose. Figure~\ref{fig:rootcause_dataformat} shows that the developer performs type conversion in the foreign function to meet the argument type requirements. However, the compatibility problem between the type and the operating system results in errors.

Developers should exercise cautions to avoid the above-mentioned error when utilizing the cross-language APIs.

\yu{I tend to use "statements after foreign function calls" as the title.}
\underline{\textit{%"Statements after 
Immediately following 
foreign function calls}}. 
The second most frequent\yu{Use plurals for the general nouns} occurrence of multilingual bugs is located immediately after a foreign function call.   

\yu{I tend to use "The first situation is that ..."}
The first situation is that developers improperly\yu{Use simple present tense} handle the return value of the foreign function. As shown in Figure~\ref{fig:rootcause-boundary}, the developer failed to consider the possibility that the foreign function could return "NULL" and did not specifically handle this edge case. This often stems from a lack of understanding of the foreign function on the part of the developer.

The second situation is that the foreign function is called based on an existing object, but the existing object is not decremented in its\yu{Again, what is reference count} reference count. Figure~\ref{fig:rootcause-reference} specifies\yu{that} that the foreign function is invoked using the variable "value," but the reference count of "value" is not decreased. It causes an error in the if-statement. 

Developers should be more cautious about argument variables used by foreign functions and variables returned. For argument variables,\yu{Developers, not "you"} developers should consider increasing or decreasing the reference count and be more sensitive about some particular values for returned variables.

\underline{\textit{Others}} Apart from the Cross-language API callsite and Following a foreign function call, there are also other locations where multilingual bugs may occur. Interestingly,  some multilingual bugs may also be similar to single-language bugs. For example, an if-statement in C lacks a condition and then passes an inappropriate value to Python, but we can only get this error from Python. As a result, a multilingual defect\yu{cause of -> causing} causing the error may be similar to that of a single language bug. Still, the resulting visible symptom  differs because the data is passed through the language boundary.



% \underline{\textit{Reference count error}} 
% Around the bug location, there will be some API functions such as Py\_DECREF, Py\_XINCREF(), and other functions to manage reference count. Defects with reference count errors are among the most common causes of memory leaks in multi-lingual systems, mainly when using dynamic programming languages such as Python. Because Python uses a garbage collector to manage memory, while C relies on manual memory management, the mechanism used by Python to manage memory can be difficult to manage correctly when working with C code. Reference counting is implemented through API functions such as Py\_DECREF and Py\_XINCREF, which must be used correctly to avoid memory leaks. 

% Overall, reference count errors can occur more easily when Python interacts with C code due to differences in memory management and the complexity of reference counting. These API functions for reference count management often appear in the context of bugs. Intuitively, we can also understand that multilingual defects occur near these functions due to different memory management mechanisms. It's essential for developers to be aware of these challenges and to follow best practices for managing memory in multi-lingual systems to avoid reference count errors and improve the performance and stability of their software.

% \underline{\textit{Data format error}}
% This type of bug can occur when initializing variables or receiving return values from API functions. If the data types between the two languages are different, errors can occur during data transmission, leading to data format errors. This is because Python and C may have different representations for data types, and the data must be converted between the two languages to ensure compatibility. Therefore, it's important to consider the data types involved in each API call carefully and to perform proper data conversion when necessary. This can help to avoid data format errors and improve the reliability of multi-lingual systems.

% In summary, data format errors can generally occur at variable initialization or surrounding API functions with value return. In summary, data format errors in multi-lingual systems are often a result of differences in data types between the two languages, particularly when initializing variables or receiving return values from API functions. It's important for developers to be aware of these potential issues and to carefully consider the data types involved in each API call to ensure compatibility and avoid data format errors. 

\subsection{How Multilingual Bugs Are Fixed}
\label{section:3.4}
We conducted a manual review of the final patches to address two questions: Are there standard strategies for fixing multilingual bugs, and how complex are the patches? 

Our findings are opposite the assumption that multilingual patches are complex and lack clear patterns.

%\underline{\textit{Fixing strategies}}.
\textbf{Fixing strategies}.
Table~\ref{tab:casestudy} shows two common strategies for fixing multilingual bugs.

The most frequently used strategy is\yu{changing} 
%the "Change Condition", which involves modifying a condition in an if or switch statement. 
to \ul{\textit{change the condition against a foreign function call return value}}. 
This strategy was used to fix 52 bugs and is effective in addressing bugs caused by missing checking the value returned by the foreign function call (e.g., as shown in Figure~\ref{fig:rootcause-boundary}). Generally, a bug does not occur immediately after the cross-language function returns the value. Instead,\yu{This sentence does not make sense.} bugs happen when the code calls the stored returned value; this result also\yu{confirmed what? what did you mention? Also, grammar issue!} confirmed that we mentioned the bug occurrence\yu{Why is this uppercase? A new sentence? What is "a foreign function call in Section 3.3"?} "Statements after foreign function calls" in section~\ref{section:3.3}. In other words, we need to change the conditional statement since it is error-prone in handling the cross-language returned value.

The second most common strategy is\yu{changing} %"Change API function", 
to \ul{\textit{replace a misused cross-language API with a correct one}}, 
which\yu{is} is used in 50 commits. This strategy involves changing a\yu{argument} argument of a cross-language API function in the code, adding a new foreign function, or modifying a buggy function to a proper one. For example, it may involve changing the type of\yu{argument} argument in a foreign function call (Figure~\ref{fig:rootcause_dataformat}) or decreasing the reference count of variables by adding an API function call (Figure~\ref{fig:rootcause-reference}). In this case, the bug is usually caused by improper use of the original cross-language API function or\yu{The lack of the function? You mean the function is not enough?} missing the cross-language API function.

%\underline{\textit{Complexity of patches}}.
\textbf{Complexity of patches}. 
The majority of multilingual bugs in our study can be resolved with simple modifications. Of the 102 bug patches, 66 contained ten or fewer lines of code changes. The median patch size for all bugs analyzed was seven lines of code.

This small patch size is due to the simplicity of the fixing strategies.\yu{Half of the changing conditions require ...} Half of the "Change Condition" requires no more than ten lines of code to be altered. Similarly, 29 out of the 50 "Change API Function" patches\yu{use simple present tense} require ten or fewer lines of code changes.

%\subsection{Discussion}
\subsection{Lessons Learned from Our Study}
In our research, we discovered that three primary root causes account for more than 50\% of all the issues encountered in the multilingual project. These three main root causes are linked with the cross-language API functions.\yu{Avoid using "believe", use "Our findings indicate that if a developer ..." instead.} Our
findings indicate that if a developer lacks proper knowledge about the cross-language API,\yu{... API, it can ...} it can lead to incorrect usage and cause issues. To overcome these problems, it is important that developers have a thorough understanding of the API functions and their correct usage in the multilingual project.
% Cross-language API functions can introduce bugs in several ways:
% 1. Incorrect argument type: If the argument type passed to the API function is incompatible with the intended requirement, it may result in errors.
% 2. Return value not handled: If an API function's return value is not handled correctly, it can result in bugs, particularly if the function is expected to return NULL in some cases.
% 3. Improper reference management: Cross-language API functions often involve managing references to objects across different programming languages. If the reference management is not done correctly, it can result in memory leaks or other bugs.

Bugs mainly occur in the statements of the cross-language API functions or in the following lines of code. Because cross-language API functions cause most bugs, we can naturally think that bugs will occur near these API functions. Because the results of the root causes and bug locations collaborate each other,\yu{Again, do not use "believe". Start this sentence with the words after "that"} our findings show that multilingual bugs are largely related to cross-language API functions. Our hypothesis\yu{is} is further validated by a subsequent study on bug fixing. Although the fix strategy "Change Condition" does not seem to have much to do with the cross-language API function,\yu{I think you want to say "the changes are usually right after the API functions"} the changes are usually right after the API functions. The reason for part of the code being changed is that an API function's return value is not handled correctly, so it needs some additional conditional statements to process. Therefore, we believe that the "Change Condition" is also related to the cross-language API function. As with the other fixing strategy "Change API function", this approach immediately updates the statement in which the cross-language API function is situated; thus, it must have a direct connection to it.

In the study, we also found that foreign functions are the main cause of cross-language problems. In other words, most of the problems appear in the C language. In a Python-C project, foreign functions may be more susceptible to bugs compared to native Python functions due to differences in the underlying implementation. Some reasons for this include:
\begin{itemize}[leftmargin=6pt,topsep=2pt]
	\item \textit{Memory Management:} 
	C code has to explicitly manage memory, whereas, in Python, this is handled automatically by the interpreter's garbage collector. This can lead to memory leaks or segmentation faults if the C code is incorrectly written. 
	
	\item \textit{Type System:} 
	\yu{Are you sure? I believe the bugs in C programs are more likely to be detected when compiling.} Python has a dynamically typed language, whereas C is statically typed. This means that type errors in Python can often only be detected at runtime, whereas in C, they are usually caught by the compiler before the code is executed.
	
	\item \textit{Exception Handling:} 
	C code typically uses return codes or error codes to indicate success or failure, whereas Python raises exceptions to show errors. If the C code does not correctly check for and handle errors, it may lead to unexpected behavior.
\end{itemize}
However, it is worth noting that well-written C code can be just as robust as Python code, and the use of C in a Python-C project can bring significant performance benefits. Improving code quality and developers' abilities are both approaches to offer greater drive to the advantages of multilingual projects.

Overall, we are adamant that cross-language API functions are the primary source of errors in multilingual projects. Therefore, this feature can be used extensively to detect multilingual project defects. To avoid bugs when developing multilingual projects, developers need to be very careful when using cross-language API functions, especially foreign functions.



==> conclusion-cai.tex <==
\section{Conclusion}\label{sec:conclude}
We presented the first comprehensive study of real-world cross-language bugs.
Using our new tool along with manual analysis, we 
collected and dissected 
the first set of 400 such bugs carefully labeled from real-world Python-C and Java-C repositories on GitHub. 
We thus identified the symptoms, locations, manifestation characteristics, 
root causes, and fixing strategies of those bugs, discovering both the common and 
different bug patterns between the two language combinations. 
Based on our findings, we also provide actionable insights into 
how to prevent, detect, and fix cross-language bugs. 


% We presented the first comprehensive study of real-world multilingual bugs induced by cross-language behaviors. 
% Using our tool followed by manual confirmation, we 
% collected the first set of 1039 multilingual bugs in real-world Python-C projects on GitHub. 
% We then conducted in-depth case studies for 216 of these bugs, 
% classifying their symptoms, introducing locations, and manifestation characteristics while 
% dissecting their root causes and fixing strategies. 
% Based on our study findings, we provide actionable insights into 
% how to prevent, detect, test/debug, and fix multilingual bugs. 

% Multilingual bugs as we studied are those induced by explicit interaction (via cross-language API calls) between different languages. 
% These bugs have been ignored in prior works on software defects, and tool support for diagnosing them has been lacking. 
% To fill these gaps, we conducted an in-depth study of 102 multilingual bugs in a range of real-world systems hosted on GitHub, hence revealing common code patterns of \textit{where} and \textit{why} they have occurred and \textit{how} developers have fixed them. 
% Our findings led to a variety of insights into future research on multilingual software assurance, concerning the detection/localization and repair of 
% multilingual bugs. 
% Informed by some of these insights, 
% we further developed a learning-based technique and tool that learn 
% to locate code lines bearing multilingual bugs via a custom transformer attention mechanism featured with a novel, multilingual-code-specific position encoding scheme. 
% Our evaluation results have shown substantial advantages of this technique over 
% state-of-the-art baselines in both precision and recall. 
% We situate our study and tool as a first step towards multilingual bug understanding and diagnosis, potentially bringing more attention to research on these bugs. 




% \section{Data Availability}
% We released all of our code and datasets to facilitate reproduction, replication and reuse, as found in our %at https://github.com/hcrestlab/androidincompat/.
% %\href{https://www.dropbox.com/s/h515kgfufyi2mr1/Multilanguage_Tool.zip?dl=0}
% \href{https://figshare.com/s/1b171f5e00d064085645}{\underline{artifact package}}.


==> discussion-cai.tex <==

\section{Discussion}
\subsection{Implications and Actionable Insights}
%-------------------------------------------------
% From the aspects corresponding to how each RQ is justified/motivated
% - How to prevent 
% - How to detect multilingual bugs
%     - Detection challenge
% - How to fix
%-------------------------------------------------
Based on our findings, %regarding the five aspects of multilingual bugs, 
we provide actionable suggestions to researchers and developers of multi-language software on preventing, detecting/testing, and fixing multilingual bugs.

\subsubsection{Multilingual Bug Prevention/Avoidance}
Our results ($\S$\ref{RQ1}) revealed that nearly one-third of the studied bugs were symptomized as crashes or abortions, suggesting \textbf{multilingual bugs led to critical software failures}. Thus, given the greater cost of dealing with defects found later, developers should make the best effort possible to prevent these bugs from happening in the first place. 

%\textbf{Multilingual bugs are commonly introduced at cross-language API callsites, pointing to the importance of using these APIs correctly.}
\textbf{Use cautions against function calls involving cross-language behaviors.}
In $\S$\ref{RQ2}, we found that the most common location where multilingual bugs were introduced is cross-language API callsite. This is primarily due to the differences in how each programming language handles data types, memory management, and exceptions, as well as differences in syntax and semantics. Other sensitive locations include callsites of functions that are not cross-language APIs but still involved in cross-language information flow, as well as assignments and return sites that are related to such flows. 
Thus, to avoid introducing multilingual bugs, developers should pay peculiar attentions to these locations. For instance, a concrete step to be taken is to gain a correct and systematic understanding of a foreign or native function before invoking it, including its semantics, input/output data types, and return values. 

%prevent bugs in these locations, the following measures can be adopted: i) Understanding Cross-Language API. Having a thorough understanding of the API functions being used is critical. This includes knowledge of what each function does, its input and output data types, possible return values, and any side effects it might have. ii) Proper Data Type Conversion. When passing data across language boundaries, ensure that data is converted correctly between the types of the two languages. Some languages may implicitly cast types in a way that others do not, leading to unexpected results.

%\textbf{Future research should invest in cross-language API recommendations.} 
\textbf{Need for cross-language API and usage recommendations.}
In our study, we also noticed that language interfacing is complex and diverse: even within the single mechanism of FFI for Python-C software, there are at least four specific instances of such a mechanism (cffi, SWIG, Cython, and ctypes) with each coming with a large and different set of cross-language APIs. 
These complexity and diversity can be easily confounding factors that impede developers' full and correct understanding of each of those APIs. 
Thus, automated API recommendations would be quite helpful here. 
While various API recommendation tools already exist, none of the existing ones 
address cross-language APIs in multilingual software. 
Future researchers are encouraged to fill this critical gap. 

%, for which data-driven (e.g., machine learning based) approaches may be explored while leveraging our MCC tool to curate sizable training data
%
%
%In \ref{RQ2}, we observe that some symptoms are raised due to API misuse. To prevent this situation, API recommender of multilingual projects is a possible way. Regrettably, current API recommendation research doesn't generally accommodate multilingual development contexts. The advanced API recommendation methods are anchored in machine learning, requiring substantial training data~\cite{chen2021holistic,gu2016deep}. The data we get in the data collection process can be used for training model. Future researchers can use our dataset for multilingual projects and then model the API recommendation for multilingual development, leveraging methods from previous studies~\cite{chen2021holistic,nguyen2015graph}.

\subsubsection{Multilingual Bug Detection/Testing and Debugging}
%Intuitively, 
Our extensive findings on the symptoms, manifestation characteristics, and root causes of multilingual bugs provide concrete guidance on developing multilingual bug detection/testing/debugging solutions. 

\textbf{Leverage major symptoms for high-level/first-step detection/testing.}
Our results ($\S$\ref{RQ1}) indicate that multilingual bugs did often have strong/explicit symptoms such as crashes, error messages, and data corruptions. 
These signals can be leveraged to develop {first-step detection/testing of multilingual bugs}: e.g., when one of these primary symptoms are observed, it is likely that a multilingual bug has occurred.

\textbf{Exercise key manifestation semantics to trigger multilingual bugs.}
In $\S$\ref{RQ3}, we revealed that the majority of multilingual bugs were manifested in %cross-language 
code semantics related to reference counting, objection manipulation, and exception handling. 
Thus, multilingual software testing techniques can benefit from focusing on exercising these types of semantics in order to expose/trigger multilingual bugs. 
For instance, a directed greybox fuzzer can be devised to target respective code entities (e.g., foreign functions for reference management). Similarly, such bugs can be more efficiently covered by guiding the fuzzer towards exploring exceptional control flow constructs like those handling errors/exceptions. 

\textbf{Exploit common root causes for multilingual bug localization.}
According to our results in $\S$\ref{RQ4} versus those in $\S$\ref{RQ2}, 
where a multilingual bug is introduced may not always be where the root cause lies. 
For instance, while a substantial portion of these bugs in our study were introduced at assignment statements related to cross-language behaviors, there may be too many such statements in a multilingual program to examine them all. 
Moreover, based on our results in $\S$\ref{RQ5}, only a minor portion of these bugs were fixed by changing assignment statements. Thus, even examining all cross-language information flow related assignments may not effectively lead to locating the real bug. 
Thus, multilingual fault localization techniques should exploit the major kinds of root causes we discovered towards more effective debugging. 
%(e.g., ranking the real root cause statements at the top of the list of candidate faulty locations). 
In particular, given the dominant root cause is memory safety issues, 
the debugger may benefit from cross-language memory profiling and sanitizing. 


%\textbf{Future research is encouraged to develop techniques and tools to profile memory in multilingual projects.} Tracing bugs across the language boundary between Python and C, which have different memory management, requires knowledge of both languages. In \ref{RQ4}, we reveal that memory safety (RC1) is the main problem in multilingual development. Python has automatic memory management (garbage collection), while C requires manual memory management. Bugs that involve memory allocation, deallocation, or access can manifest differently in each language and become challenging to trace when control or data crosses from one to the other. So profiling and monitoring the memory of multilingual projects, which can help track memory usage over time and detect potential leaks or inefficiencies, is very emergency for developers. Memory profiling tools like {\tt memory-profiler} for Python and {\tt Massif} for C can be helpful in this regard. However, cross-language memory profiling tools are still lacking. The complexity of dealing with multiple languages and the disparity in their memory management makes this a challenging task. One approach would be to improve interoperability between language-specific memory profilers. This solution would involve creating a set of standards or APIs for exchanging memory profiling data. Developers could then use these APIs to combine data from different language-specific profilers into a comprehensive cross-language memory profile. Another possibility could be the development of a unified memory profiling framework. This framework would abstract the memory profiling features of individual languages into a common set of concepts. By providing a uniform interface, such a tool would enable developers to analyze memory usage patterns across different languages. This would require collaboration among different language communities to develop and maintain.
%Garbage Collection Debugging. In Python, the {\tt gc} module can be used to interface with the garbage collector, allowing you to manually run garbage collection, detect reference cycles, and obtain debug information about objects in memory.

\subsubsection{Multilingual Bug Fixing/Patching}
Our findings in $\S$\ref{RQ5} provide immediate guidance on fixing/patching multilingual bugs through the common fix locations and fixing approaches. 
%we revealed. 

\textbf{Prioritize cross-language API callsite and branching structures.}
Our results indicate these two types of locations dominated contexts that collectively fostered nearly half of the bug fixes we studied. 
Thus, developers may pay first and foremost attention to these places to identify effective fixes of multilingual bugs for prioritized debugging. 
Likewise, automated bug repair techniques based on deep neural networks (as most such extant peer tools are designed) may learn particular attentions towards those locations to better predict repair locations. These techniques may further leverage our MCC tool to help curate sizable training datasets.
%multilingual bug datasets to meet training needs. 

\textbf{Start with the common strategies for multilingual bug patching.}
In $\S$\ref{RQ5}, we revealed four common approaches developers have adopted for fixing multilingual bugs. 
This result provides clear guidance on what kinds of code changes may be fruitful for writing 
multilingual bug patches. 
For instance, developers may attempt to fix a logic-error-induced multilingual bug by identifying a correct cross-language API to replace the current one at the fault location. 


%\textbf{Our findings reveal the bug-fixing location for multilingual development often near the language boundary and developers should be aware of them when starting fixing bugs. } In \ref{RQ5}, one fixing approach is using appropriate data types and casting. This implies that bugs occur when a data type from one language is processed and transformed after crossing the language boundary into another language. In \ref{RQ2}, we reveal that bugs are most frequently introduced at the sites where APIs from different languages interact, which is on the language boundary. In addition, some bugs occurred after a foreign function call. Thus, when starting to fix multilingual bugs, developers can first consider troubleshooting from the language boundary.



\input{threats-cai}

% \subsection{Threats to Validity}
% \textbf{Threats to internal validity}. 
% The code of our tools and models is a critical component in ensuring the validity of our research findings. Despite our efforts to avoid bugs and errors through code reviews, there is still a possibility that undetected bugs could exist in the code. These bugs could affect the performance of the tools and models and lead to incorrect results or findings. 

% We depend heavily on manual analysis, and our hand labeling is subject to personal prejudice. To reduce human bias throughout the labeling process, two authors examined the commits and labeled the root cause and bug location independently, with discrepancies discussed until consensus was established. 


% \textbf{Threats to external validity} 
% We focused on analyzing Python-C projects for our study; our findings may not be generalizable to other language combination projects. However, Python and C are popular languages for developers, and many projects are programmed with the combination of Python - C, so we think it is representative. We encourage future research to investigate the problem via other language combinations. 

% Our research results and findings are based on data collected from the Python-C projects with the high stars. While this data may provide insights into the top-performing projects, it may not represent other Python-C projects that were not included in the analysis. This limited data source potentially threatens the validity of the results. It highlights the need to consider other data sources or criteria when evaluating the generalizability of the findings.






==> discussion.tex <==

\section{Discussion}
\subsection{Implication}
%-------------------------------------------------
% From the aspects corresponding to how each RQ is justified/motivated
% - How to prevent 
% - How to detect multilingual bugs
%     - Detection challenge
% - How to fix
%-------------------------------------------------
\subsubsection{Multilingual bug prevention/avoidance}
\textbf{Bugs often occur at foreign function callsites, pointing to the importance of handling such interactions correctly.} In \ref{RQ2}, the location most likely to introduce a bug is the foreign function callsite. This is primarily due to the differences in how each programming language handles data types, memory management, and exceptions, as well as differences in syntax and semantics. To prevent bugs in these locations, the following measures can be adopted: i) Understanding foreign function. Having a thorough understanding of the API functions being used is critical. This includes knowledge of what each function does, its input and output data types, possible return values, and any side effects it might have. ii) Proper Data Type Conversion. When passing data across language boundaries, ensure that data is converted correctly between the types of the two languages. Some languages may implicitly cast types in a way that others do not, leading to unexpected results.

\textbf{Future research should prioritize enhancing the recommendation of accurate APIs and their usage.} In \ref{RQ2}, we observe that some symptoms are raised due to API misuse. To prevent this situation, API recommender of multilingual projects is a possible way. Regrettably, current API recommendation research doesn't generally accommodate multilingual development contexts. The advanced API recommendation methods are anchored in machine learning, requiring substantial training data~\cite{chen2021holistic,gu2016deep}. The data we get in the data collection process can be used for training model. Future researchers can use our dataset for multilingual projects and then model the API recommendation for multilingual development, leveraging methods from previous studies~\cite{chen2021holistic,nguyen2015graph}.


\subsubsection{Multilingual bug detection/testing and debugging}
\textbf{Future research is encouraged to develop techniques and tools to profile memory in multilingual projects.} Tracing bugs across the language boundary between Python and C, which have different memory management, requires knowledge of both languages. In \ref{RQ4}, we reveal that memory safety (RC1) is the main problem in multilingual development. Python has automatic memory management (garbage collection), while C requires manual memory management. Bugs that involve memory allocation, deallocation, or access can manifest differently in each language and become challenging to trace when control or data crosses from one to the other. So profiling and monitoring the memory of multilingual projects, which can help track memory usage over time and detect potential leaks or inefficiencies, is very emergency for developers. Memory profiling tools like {\tt memory-profiler} for Python and {\tt Massif} for C can be helpful in this regard. However, cross-language memory profiling tools are still lacking. The complexity of dealing with multiple languages and the disparity in their memory management makes this a challenging task. One approach would be to improve interoperability between language-specific memory profilers. This solution would involve creating a set of standards or APIs for exchanging memory profiling data. Developers could then use these APIs to combine data from different language-specific profilers into a comprehensive cross-language memory profile. Another possibility could be the development of a unified memory profiling framework. This framework would abstract the memory profiling features of individual languages into a common set of concepts. By providing a uniform interface, such a tool would enable developers to analyze memory usage patterns across different languages. This would require collaboration among different language communities to develop and maintain.
%Garbage Collection Debugging. In Python, the {\tt gc} module can be used to interface with the garbage collector, allowing you to manually run garbage collection, detect reference cycles, and obtain debug information about objects in memory.

\subsubsection{Multilingual bug fixing/patching}
\textbf{Our findings reveal the bug-fixing location for multilingual development often near the language boundary and developers should be aware of them when starting fixing bugs. } In \ref{RQ5}, one fixing approach is using appropriate data types and casting. This implies that bugs occur when a data type from one language is processed and transformed after crossing the language boundary into another language. In \ref{RQ2}, we reveal that bugs are most frequently introduced at the sites where APIs from different languages interact, which is on the language boundary. In addition, some bugs occurred after a foreign function call. Thus, when starting to fix multilingual bugs, developers can first consider troubleshooting from the language boundary.



\input{threats-cai}

% \subsection{Threats to Validity}
% \textbf{Threats to internal validity}. 
% The code of our tools and models is a critical component in ensuring the validity of our research findings. Despite our efforts to avoid bugs and errors through code reviews, there is still a possibility that undetected bugs could exist in the code. These bugs could affect the performance of the tools and models and lead to incorrect results or findings. 

% We depend heavily on manual analysis, and our hand labeling is subject to personal prejudice. To reduce human bias throughout the labeling process, two authors examined the commits and labeled the root cause and bug location independently, with discrepancies discussed until consensus was established. 


% \textbf{Threats to external validity} 
% We focused on analyzing Python-C projects for our study; our findings may not be generalizable to other language combination projects. However, Python and C are popular languages for developers, and many projects are programmed with the combination of Python - C, so we think it is representative. We encourage future research to investigate the problem via other language combinations. 

% Our research results and findings are based on data collected from the Python-C projects with the high stars. While this data may provide insights into the top-performing projects, it may not represent other Python-C projects that were not included in the analysis. This limited data source potentially threatens the validity of the results. It highlights the need to consider other data sources or criteria when evaluating the generalizability of the findings.


%--------------------------------------------
% Adding conditions to handle edge cases: 	
% Software applications frequently comprise a substantial quantity of logical pathways and edge cases. These applications necessitate the contemplation of a vast array of conditions. The inherent challenge lies in comprehending these conditions and authoring code that adeptly manages them. Often, this necessitates the deployment of conditional logic, such as 'if' statements, to scrutinize specific conditions and execute the corresponding action.
	
	
% Comprehending the variable utilized in functions: 	
% A variable is employed across multiple functions or modules in extensive code repositories. The variable's value shifts throughout the program's execution, and deciphering how and when these alterations occur poses a substantial challenge. This is particularly the case when the variable's utilization entails complexity, for instance, when it is conveyed as a parameter to functions, retrieved from functions, or disseminated among threads.



==> intro-cai.tex <==
%!TEX root = paper.tex

%\vspace{-3pt}
\section{Introduction}\label{sec:intro}
%\vspace{-2pt}
%% == High-level introduction to the topic of this paper
%
%% problem context (multi-language software is prevalent, and they are bug prone)
%
%Multi-language systems that are built in two mainstream programming languages (e.g., among Java, Python, and C) have seen widespread presence and impact (e.g., in machine-learning frameworks and mobile/cloud platforms)~\cite{li2023multilingual}. 
{{Multilingual software development}}~\cite{yang2024multi} (i.e., developing one software project with multiple programming languages that \textit{interact}) is ubiquitous~\cite{jones2010software,delorey2007programming,ray2014large} and still on the rise~\cite{tomassetti2014empirical,mayer2015empirical,valverde2015punctuated,li2021understanding}. 
Thus, the vast and growing majority of real-world systems are 
\textit{multilingual}, 
hence the paramount importance of assuring their quality~\cite{chisnall2013challenge}. 
While fostering a productive software process in various ways~\cite{abidi2019behind,bissyande2013popularity}
(e.g., combining the strengths of different languages~\cite{meyerovich2013empirical,vasilescu2013babel}), 
multilingual development also leads to great complexity of the resulting software. This is not just the result of adding per-language complexities up, but particularly due to the intricate \textit{interactions} between heterogeneous languages. 
The extra complexity tends to make multilingual software more buggy~\cite{abidi2021multi,wen22fse}. 

%A number of studies have suggested that software written in multiple programming languages (i.e., {\em multi-language} software) is prevalent.
%For instance, 20\% of the 9,997 projects sampled on SourceForge~\cite{sourceforge} %during the years of 2000---2005
%used two languages while 12\% of them used three~\cite{delorey2007programming}.
%A later, industrial report found that most of applications developed by top companies were written in 2 to 15 languages~\cite{jones2009software}.
%This is consistent with more recent studies finding that more than half of the randomly sampled open-source projects on GitHub were developed in two or more languages, despite the largely varying sample sizes (e.g., 729~\cite{ray2014large}, 1,150~\cite{mayer2015empirical}, and 15,000~\cite{tomassetti2014empirical}).
%
%% justification for multi-language software
%Intuitively, %the prevalence of using multiple languages in a single project hints about impetus (e.g., benefits or even necessity) of doing so.
%the prevalence and dominance of multi-language software is justifiable given the impetus (e.g., benefits or even necessity) of using multiple languages in a single software project~\cite{abidi2019behind}.
%Indeed, different languages have their own peculiar strengths and weaknesses~\cite{chen2005empirical,meyerovich2013empirical}. Thus, combining various languages could be a natural consideration by developers for building software that requires capabilities each %meritoriously
%best offered by one of the languages. For example, a web application may use Python, a general-purpose language (GPL), and HTML,
%a domain-specific language (DSL) like CSS to combine their productivity and presentation merits, respectively.
%Similarly, an IoT software developer may use Java for plug-in development to exploit its portability advantage, along with C for implementing system-level features to leverage its efficiency advantages.

%% the problem (general motivation): talk about bugs in multilingual systems, define multingual bugs, and then the importance of understanding those bugs--understanding bugs in such software helps developers avoid or deal with the bugs

Even worse, the multilingual world is diverse, both in terms of the large number/variety of languages that can be used in tandem~\cite{jones2010software,li2021understanding} and concerning 
the varying ways the heterogeneous languages used may \textit{interact}~\cite{mayer2017taxonomy,wen22fsetool,li2023multilingual}. 
This diversity further aggravates the complexity of multilingual software, 
explaining their bug-proneness, both qualitatively~\cite{mayer2017multi} 
and statistically~\cite{wen22fse,abidi2021multi}. 
In fact, this bug-proneness is often translated to 
actual and real bugs~\cite{kochhar2016large,grichi2020impactjni,wen23usenixsecurity,wen22usenixsecurity,sultana2016understanding,hu2023empirical}, especially stealthy ones borne in faulty cross-language information flow induced by the interactions 
between various languages (i.e., \textit{cross-language bugs}).

Yet in contrast to the increasing number of tools each having discovered 
only a few of them~\cite{youn2023declarative,dinh2021favocado,wen22usenixsecurity,wen23usenixsecurity,hu2023empirical}, 
cross-language bugs have not been comprehensively studied. 
% existing works and insufficiencies (what has been done and what is still the gap)
Earlier research that contributed relevant understandings does exist, which has examined the general characteristics of bugs induced by language use~\cite{zhang2019study} and interoperation~\cite{bae2019towards}. 
However, the extant works fall far short in at least three folds. 
First, most of current relevant studies are only concerned about \textit{individual} languages each used separately from others, not really concerning \textit{multilingual} software (i.e., 
with multiple languages used together with \textit{interactions})~\cite{ray2014large,berger2019impact,zhang2019study}. 
Second, studies that do address {multilingual} software are either qualitative or at best statistical---they investigate bug-related human opinions (e.g.,developers'  perception~\cite{mayer2017multi,abidi2019behind}) or defect \textit{proneness} (e.g., in terms of statistical associations between language combination and likely bug indicators~\cite{wen22fse,kochhar2016large,grichi2020impactjni}), not 
really based on \textit{factual} bugs in real-world multilingual code. 
Likewise, the most recent relevant works are either based on developers discussions~\cite{yang2023demystifying}---and the issues examined are not necessarily code-level bugs, or limited to high-level characteristics 
%(open/reopen timing) 
of bugs in systems using multiple languages~\cite{li2023understandinga,li2023understandingb}---the systems are not necessarily multilingual and the bugs may not be induced by language interactions. 
Third, studies addressing language interoperability are closer to understanding 
cross-language bugs, yet existing ones are only limited to cross-language API misuses~\cite{sultana2016understanding,hu2023empirical}.

% As it stands, there is still a lack of understanding of bugs in multilingual software that are induced by \textit{cross-language} code behaviors (noted as {\em multilingual bugs}).  
% Thus, %intuitively 
% it is crucial to understand those bugs (e.g., regarding
% \textit{where} and \textit{why} they occur as well as \textit{how} to fix them) 
% %and provide tool support for diagnosing them---two essential steps 
% an essential first step toward multilingual software quality assurance. 

%
% There also have been a few current techniques/tools supporting multilingual 
% software testing and debugging~\cite{haoran22fsenier,binkley2014orbs,wen22usenixsecurity,wen23usenixsecurity,lee2020broadening,hwang2021justgen}. 
% Unfortunately, these existing options are insufficient for two reasons. 
% First, the majority of them %the second category of studies 
% are limited to one particular case of language combination---Java and C~\cite{xue2018ndroid,lee2020broadening,hwang2021justgen,bae2019towards}, 
% which does not work with nor is readily extensible for other, more prevalent 
% cases (e.g., Python-C). 
% However, Java-C may not be even among the top-20 most popularly used 
% language selection, at least in the open-source world as sampled from GitHub as per recent studies~\cite{wen22fsetool,wen22fse,li2021understanding}. 
% Second, the very few remaining tools are %address a single type of bugs (e.g.,
% dynamic (meaning they could not reveal bugs that are not exercised at runtime)~\cite{bai2018bridgetaint,xue2018ndroid,wen22usenixsecurity,wen23usenixsecurity}, and/or 
% impractical to use due to scalability barriers~\cite{binkley2014orbs,haoran22fsenier}.

%The use of programming languages in software development has been studied, concerning the factors that affect the success of a language~\cite{chen2005empirical}, the popularity of different languages~\cite{karus2011study,bissyande2013popularity,meyerovich2013empirical,ray2014large},
%interactions/relationships (e.g., similarity) across languages~\cite{bissyande2013popularity,karus2011study,vasilescu2013babel}, and evolution of languages in these regards~\cite{chen2005empirical,karus2011study}.
%Relevant studies also have addressed the effects of language use on the defect-proneness~\cite{ray2014large}, quality risk of the lack of maintenance~\cite{vasilescu2013babel}, and bug resolution characteristics (e.g., bug fix size and time)~\cite{zhang2019study} of the resulting software.
%However, these prior studies {\em mainly} targeted single-language software, focusing on how individual languages were used.

%
%Studies looking at language use in multi-language software do exist, which addressed the prevalence of such software~\cite{mayer2017multi,tomassetti2014empirical} as well as good/bad practices for various quality factors in developing software~\cite{abidi2019behind}.
%Few of these studies looked into the possible rationale behind developers' choice of languages and justifications of language
%selections in multi-language projects.
%Moreover, several of these studies were based on developers' perceptions through surveys~\cite{abidi2019behind,mayer2017multi} rather than examined the actual artifacts of multi-language software projects.
%Two studies~\cite{mayer2015empirical,delorey2007programming} investigated the associations among chosen languages in multi-language software
%based on actual project data.
%Yet, like other peer studies, they did not examine how the language selections in a multi-language project may be justified %explained
%with respect to development decisions %(e.g., via characteristics, such as topics or functionalities, of the project).
%(e.g., functionality category/domain or project topic).
%In particular, the more recent study~\cite{mayer2015empirical} (as performed five years ago) did not
%apply an evolutionary perspective but rather considered the dataset (1,150 projects) as one single selection of GitHub.
%The other considered the evolution of language use during the years of 2000---2005; since it was conducted 15 years ago,
%%Also, as they were conducted five or even over ten years ago,
%the relevance of the results might have significantly %critically diminished.
%deteriorated.

%Prior relevant work mostly addresses how {\em individual languages} were used, including success factors of a language~\cite{chen2005empirical}, popularity of different languages~\cite{karus2011study,bissyande2013popularity,meyerovich2013empirical,ray2014large}, relationships across languages~\cite{bissyande2013popularity,karus2011study,vasilescu2013babel}, defect-proneness~\cite{ray2014large},
%quality risks~\cite{vasilescu2013babel}, and bug resolution characteristics~\cite{zhang2019study}.
%
% Current relevant work mostly addresses how {\em individual languages} were used, including the popularity~\cite{karus2011study,bissyande2013popularity,meyerovich2013empirical,ray2014large},
% success factors~\cite{chen2005empirical}, defect-proneness~\cite{ray2014large}, relationships~\cite{bissyande2013popularity,karus2011study,vasilescu2013babel},
% quality risks~\cite{vasilescu2013babel},
% and bug resolution characteristics~\cite{zhang2019study} of various languages.
% %
% A few others looked at language use in multi-language software, concerning the prevalence~\cite{mayer2017multi,tomassetti2014empirical} and good/bad practices for quality~\cite{abidi2019behind}. %of such software~\cite{abidi2019behind}.
% Several of these studies were based on developers' perceptions through surveys~\cite{abidi2019behind,mayer2017multi} rather
% than the actual software artifacts. %of multi-language software.
% Three studies~\cite{mayer2015empirical,delorey2007programming,kochhar2016large} investigated the associations among chosen languages %in multi-language software
% based on actual project data.
% Yet they did not examine how the language selection (i.e., combination) in a multi-language project may be justified %explained
% with respect to security concerns %(e.g., via characteristics, such as topics or functionalities, of the project).
% (e.g., code vulnerability).
% We also lack a recent %, evolutionary
% view of how these characteristics evolved.

This paper presents the first comprehensive study of real-world \textit{cross-language} bugs (\textbf{CLB}s), focusing on those in two dominating language combinations~\cite{li2023multilingual} that have seen widespread presence and impact: Python-C (e.g., in machine-learning frameworks such as PyTorch/ TensorFlow and NumPy/SciPy) and Java-C (e.g., in mobile/Web/database platforms such as Android, Tomcat, MySQL). 
For each language combination, we randomly sampled 200 CLBs, filtered and classified from a total of 865,680 commits in 2,428 repositories on GitHub. 
For each of the 400 confirmed CLBs, we then carefully examined the commit log, the code changed and those impacted by the change, directly associated and indirectly linked bug/issue reports, and relevant official/external documentation. 
Both of the automated commit classification/labeling and manual 
CLB inspection are enabled by our novel static cross-language analyzer. 
The main goal of our study is to provide multilingual software 
developers and users with findings and insights 
%on the characteristics of CLBs in five aspects: their \textit{symptoms}, \textit{locations} (in terms of structural/syntactic code contexts), \textit{manifestation} (concerning the type and semantics of involved {cross-language functions} and the direction/complexity of cross-language information flow), \textit{root causes}, and \textit{fixing strategies}. 
on \textit{where} and \textit{why} CLBs occur as well as \textit{how} to fix them. 
Accordingly, our study aims to answer the following research questions: 
%
% % what we do
% In this paper, we set out to fill this critical gap, focusing on real-world \textit{cross-language} bugs 
% %bugs induced by cross-language interaction via explicit function calls  
% in software written in Python and C as primary languages (noted as 
% {\em Python-C} software). 
% We start with collecting and labeling the first set of 1,039 automatically mined and then manually confirmed multilingual-bug-fixing commits from 200 Python-C projects on GitHub, using a new tool we developed to enable our study. 
% Then, we conducted a comprehensive study of 216 multilingual bugs randomly sampled from those commits, systematically examining their \textit{symptoms}, \textit{introducing locations} (in terms of structural/syntactic code contexts), \textit{manifestation characteristics} (concerning the type and semantics of \textit{cross-language APIs} and the direction/complexity of inter-language information flow), \textit{root causes}, and \textit{fixing strategies}. 
\begin{itemize}[leftmargin=*,topsep=2pt]
\vspace{-0pt}
\item \textbf{\textit{RQ1: What are the symptoms of CLBs?}}
We identify how CLBs are %symptomized or 
externalized (as observed by developers or users) by examining 
the bug/issue reports. 
%The understanding not only serves an initial step of high-level detection of multilingual bugs, but also informs about their severity and consequences. 

\item \textbf{\textit{RQ2: Where do CLBs occur?}}
We identify the location (in terms of structural/syntactic code contexts) where 
CLBs appear by forward tracking the cross-language information flow from the 
bug-fixing locations indicated in the associated CLB-fixing commit.
%This RQ aims to discover where these bugs are introduced in terms of code structural/syntactic contexts. The result can shed light on the context in which multilingual bugs may happen hence helping developers understand where to avoid introducing such bugs.

\item \textbf{\textit{RQ3: What are the manifestation characteristics of CLBs?}}
We identify how CLBs are manifested, concerning the 
%type (e.g., native versus foreign function) and 
categories 
of functional semantics (e.g., memory access versus I/O) of the cross-language functions on, as well as the direction/complexity of, the 
CLB's underlying information flows (control/data dependencies). 
%This RQ aims to elucidate the code-level attributes regarding how these bugs are manifested, concerning the type (e.g., native versus foreign function) and functional semantics (e.g., memory access versus I/O) of the cross-language APIs/functions involved as well as the direction and complexity of underlying control/data flows. The result can help design effective testing techniques to expose multilingual bugs. 

\item \textbf{\textit{RQ4: What are the root causes of CLBs?}} 
We identify the reasons why CLBs occur by backwardly tracking the 
cross-language information flow paths from the bug location (identified for RQ2) until the flow source (i.e., CLB origin). 
%This RQ aims to dissect the underlying causes of these bugs. The result provides a basic understanding of multilingual bugs and immediate guidance for preventing, detecting/locating, and resolving them. 

\item \textbf{\textit{RQ5: How are CLBs fixed?}} 
We identify the CLB fixing strategies, including fix locations, 
immediately based on the bug fixes indicated by the associated 
CLB-fixing commit. 
%This RQ aims to reveal how developers have fixed these bugs. The result may help inform the development of better multilingual code debugging/repair tools and improve the patching process of multilingual bugs.
\end{itemize}

% We start with
% a comprehensive %empirical 
% study of 102 real-world multilingual bugs %(randomly sampled out of 352) 
% mined from 23 popular Python-C projects on GitHub, using our novel mining tool that automatically retrieves 
% likely-multilingual-bug-fixing commits followed by manual validation. %confirmation. 
% Through in-depth manual inspection, we identified the major \textit{root causes} of these bugs, structural patterns of code locations \textit{where the bugs occur}, and \textit{common strategies for fixing} them as used by developers. 

%\vspace{2pt}\noindent
%\textbf{Major findings.}
\noindent
Our study led to several noteworthy findings. 
First, CLBs were most often symptomized as incorrect results/outputs and error/warning messages and mostly occurred at 
assignments and cross-language API callsites,   
commonly to both Java-C and Python-C; but Java-C CLBs were more often symptomized as performance bottlenecks than Python-C CLBs. 
%
Second, cross-language APIs responsible for the Python-C CLBs exhibited much more diverse semantics compared to those responsible for the Java-C CLBs. 
%
Third, the studied CLBs were most commonly manifested in cross-language semantics related to foreign object manipulation, 
cross-language memory management, and inter-language exception handling. 
%
Fourth, these CLBs were usually rooted in logic errors, boundary conditional errors, and data type errors, which are dominating and common root causes for both Python-C and Java-C CLBs. 
%
Finally, %for patching these multilingual bugs, (6) 
the dominating fixing locations of CLBs were true/false branch and cross-language function callsites, while the common fixing strategies to both language combinations were to fix data types and/or logical errors, adding missing (e.g., boundary) checks, and properly handling cross-language exceptions. 
 

% Across all of the 102 bugs, the most prominent commonality lies in
% their location-wise \textit{\ul{vicinity} to cross-language APIs}---code entities closer to such API callsites tend to be more prone to multilingual defects. 
% Following this insight, we developed {\tech}, a deep learning (DL) based fault-localization technique for multilingual bug detection. 
% By formulating this task as a language-translation problem, 
% we may overcome the lack of static cross-language analysis facilities for 
% Python-C programs. 
% Thus, we designed {\tech} based on Transformer, which is the 
% most powerful DL model architecture today for language translation. 
% Given our relatively (to DL training needs) small %number of samples of multilingual bugs we have, 
% defect dataset, {\tech} uses a pre-trained Transformer (CodeT5~\cite{wang2021codet5}), followed by fine-tuning 
% against the buggy samples. 
% At the inference time, {\tech} takes a multilingual function as input 
% and outputs the location of multilingual bugs, if any, in the function. 

% Since this design treats the input program as a token sequence, one 
% could just use existing DL-based (single-language) 
% bug detectors (e.g.,~\cite{li2019deepfl,li2021fault,fu2022linevul,li2022fault}). 
% However, most of them are dynamic hence relying on test cases, which are 
% not available to us---in our study, tests triggering multilingual bugs are rarely found. 
% The few others, while working for us technically, may not be 
% effective because they ignore the input's multilingual nature. 
% Thus, we designed a \textit{multilingual-code-specific position encoding} for the Transformer in {\tech} as immediately informed by the above insight on cross-language API vicinity. 
% This novel design enables {\tech} to attend to code lines that are more likely to be responsible for multilingual bugs, hence achieving potentially higher bug-localization accuracy. 

% To evaluate our approach, we implemented {\tech} and applied it to 786 testing samples (functions). 
% Our results show that {\tech} achieved promising accuracy for line-level 
% multilingual bug detection (33.72\%@Top-1, 47.71\%@Top-3, 52.29\%@Top-5 precision), which are 2.92$\sim$7.92\% higher than the original CodeT5~\cite{wang2021codet5} (i.e., without the novel position encoding) and 170.14$\sim$353.97\% higher than a state-of-the-art baseline detector~\cite{fu2022linevul}. 
% Meanwhile, {\tech} also detected more bugs (i.e., with higher recall) than both baselines. 

\vspace{2pt}\noindent
\textbf{Contributions.}
To the best of our knowledge, this is the \ul{first comprehensive study} of real-world CLBs that examines where they are introduced and why, as well as how they are manifested and fixed. 
Our \ul{novel empirical findings} can help researchers and developers gain a systematic and in-depth understanding of such stealthy bugs hence guide their countermeasures.  
Based on these findings, we also offer \ul{actionable insights/recommendations} on how to avoid, detect, test/debug, and repair CLBs, which can inform design of practical tooling support of respective capabilities. 
We also contribute the first high-quality (i.e., accurate and diverse) 
\ul{dataset} of CLBs 
and an automated \ul{tool} to assist with curating more of them, 
which can be immediately reused for future researchers to conduct further relevant studies. 

%to support developing those tools with data-driven approaches. 
%Our automated tool based on static code analysis may also help collect more of such datasets when needed. 

% In summary, this work makes three main contributions:
% \begin{itemize}%[leftmargin=9pt]
% [leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
% %\denseitems
% \item 
% We conducted the first (to the best of our knowledge) comprehensive study of real-world multilingual bugs in Python-C code, resulting in novel findings on their root causes, occurrence locations, and fixing strategies, as well as new insights based on those findings, while also contributing a new bug dataset.
% %($\S$\ref{sec:tech})

% \item 
% We developed {\tech}, a Transformer-based (line-level) bug detection technique for Python-C software, particularly designed for localizing multilingual bugs through a novel position encoding, which demonstrated the usefulness of (part of) our study findings. 
% To the best of our knowledge, this is also the first bug detection/localization technique of its kind. 

% \item 
% We implemented {\tech} as a practical tool and evaluated it against 
% real-world Python-C projects, which revealed large superiority of 
% our technique over state-of-the-art baselines in terms of both precision and recall advantages, while justifying our custom Transformer design featured with the new position encoding. 

% \end{itemize}
% \vspace{-0pt}

\vspace{2pt}\noindent
\textbf{Open science.}
All of the source code and datasets used in and produced from our study are publicly available at

\href{https://figshare.com/s/1b171f5e00d064085645}{\underline{https://figshare.com/s/1b171f5e00d064085645}}.





==> introduction.tex <==
\section{Introduction}
%Problem context [ topic ]
Quality assurance and cost-effectiveness are essential considerations in the software development process. However, bugs can cause the software to behave unexpectedly, leading to poor user experiences and even security vulnerabilities. Finding and fixing bugs helps ensure that the software is stable and reliable and also early can be significantly less expensive than waiting until the software is released and then having to fix them. So bug detection is a critical part of developing software that helps ensure that the software is of high quality.

%Problem [ motivation ]
Multilingual bug detection refers to the process of identifying and resolving bugs in software projects that use multiple programming languages. Developers may use manual and automated techniques to identify defects in multilingual projects, including code reviews, testing, and debugging tools. Multilingual bug detection can be challenging because different languages have different syntaxes and semantics. So the first challenge is {\bf language difference}; Each programming language has its own syntax, semantics, and idioms, making it difficult to understand how different parts of the code interact. The second challenge is {\bf complexity}; A multi-programming language project may have a huge and complicated codebase, making it difficult to browse and comprehend the interactions between the various code components. {\bf Lack of documentation} is another challenge; If the documentation is insufficient or nonexistent, it may be difficult to understand how the code is supposed to behave and what it is supposed to be used for.

%Current works related and why they are not sufficient



%Our solutions and results


==> methodology-cai.tex <==
\section{Methodology}\label{sec:methodology}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=1.0\linewidth]{figure/methodology-overview.pdf}
	\caption{Overview of our study methodology (process).}
	%Overview of the data processing}
	\label{fig:studyprocess}
	\vspace{-12pt}
\end{figure}
Our study is governed by the overall process outlined in Figure~\ref{fig:studyprocess}. 
Given the lack of existing datasets on CLBs, we start with CLB collection via \ul{repository mining} (targeting Python-C and Java-C projects) on GitHub, the most popular source of open-source (multilingual) software~\cite{li2023multilingual}.  
Then, based on the resulting list of \textit{candidate repositories} and their \textit{associated commits}, we aim to curate CLBs from potential cross-language-bug-fixing (\textbf{CLBF}) commits identified using our \ul{CLBF commit classification} (\textbf{CCC}) tool. 
CCC works in three steps: 
(1) \textit{bug-fixing commit identification} to produce 
any commit aimed to fix a bug, 
(2) \textit{cross-language code revision identification} to 
ensure the revision corresponding to a bug-fixing commit 
includes cross-language interactions, 
and (3) \textit{cross-language-bug-fixing commit identification}
to determine if the commit is intended to fix a CLB. 
Finally, guided by our {research questions}, 
we perform \ul{manual bug analysis} to confirm and analyze CLBs to obtain the eventual \textit{study results}, following an \textit{open coding} process after \textit{codebooks creation}. 

\subsection{Repository Mining}\label{ss:repomining}
% The reason why we choose Java, Python, C
Given the vast diversity of the multilingual world~\cite{ray2014large,li2021understanding}, it is infeasible to cover many language combinations while aiming at a comprehensive and in-depth bug study in one paper. 
We start with Python-C and Java-C as they are the most popular and impactful language combinations~\cite{yang2024multi,li2023multilingual}
where most of existing CLBs are reported~\cite{wen22fse,wen22usenixsecurity,wen23usenixsecurity,lee2020broadening,hu2023empirical}.


% Justify important thresholds/numbers/selection criteria
For each candidate project, we use the GitHub API~\cite{github_api} to retrieve its set of languages used and the code size of each language unit. 
Based on this information, we collect projects per 
two criteria summarized and justified below: 
\begin{itemize}[leftmargin=*,topsep=2pt]
%\denseitems
\vspace{-0pt}
\item 50\% or more of the entire project is written in Python/Java and C combined in terms of code size (SLOC)---such projects can be reasonably considered Python-C or Java-C software per earlier studies~\cite{wen22usenixsecurity, wen23usenixsecurity,hu2023empirical}. 
\item The project's repository has $n$ stars. While not a perfect indicator of 
the true quality of a project~\cite{borges2018s}, \#stars has been widely used as a  popularity indicator to select software projects in many prior studies~\cite{bonifro2021content,di2020multinomial,romano2021g,ray2014large,papamichail2016user,wen22fse,li2021understanding,li2023multilingual}. 
Projects with a larger $n$ tend to gain more attention, thus the bugs in them likely have broader impacts. Thus, the larger the $n$, the better. Meanwhile, a larger $n$ implies fewer projects to be collected. 
However, a greater number and diversity of projects would make our study findings more representative. 
With this trade-off in mind and per our preliminary repository mining outcome, we chose $n=50$ to strike a good balance between the two competing concerns. 
\end{itemize}

\noindent
Following these criteria, we obtained a list of 4,185 repositories. 
Then, considering their entire history, 
we mined a total of 886,526 commits associated with these repositories. 


\subsection{CLBF Commit Classification (CCC)}\label{ss:ccc}
Not all the projects and commits obtained in $\S$\ref{ss:repomining} will be relevant for our study. Relevant are CLBF commits each meeting 3 requirements outlined and justified below: 
\begin{itemize}[leftmargin=*,topsep=2pt]
\vspace{-0pt}
\item \textbf{R1}: The commit is associated with (aimed for) \textit{fixing a bug}, because we intend to retrieve bug cases from such commits. 
\item \textbf{R2}: The commit is made to a project revision (version) that is multilingual (i.e., having interactions between its programming languages)---the commit can be a CLBF commit only if it aims to fix a bug {in truly multilingual software}. 
%while the language use and multilingual nature of a project may change across revisions~\cite{li2021understanding,wen22fse}. 
\item \textbf{R3}: The bug to be fixed by the commit involves interactions between languages (i.e., cross-language behaviors).
\end{itemize}

\noindent
%Accordingly, 
Our CCC tool has three major steps, labeled as \textcircled{2}, \textcircled{3}, and \textcircled{4} in Figure~\ref{fig:studyprocess},  
to check a commit against R1, R2, and R3, respectively, as elaborated next. 
CCC follows this specific order of these steps because of their 
descending levels of overhead---\textcircled{2} is the fastest and 
\textcircled{4} is the most expensive. 
Thus, the order enables filtering out more irrelevant commits earlier and 
letting the least candidate CLBF commits enter the most costly step, hence the lowest overall cost. 

\subsubsection{Bug-Fixing Commit Identification}\label{sss:bfci}
A CLBF commit must be a bug-fixing commit in the first place. 
Thus, we first check against R1 the commits mined so far. 
For each commit, we start by looking for its associated issue (id) and dismiss those 
for which we can not find any. 
Otherwise, we further use a set of bug related keywords to check against the issue tags, 
including 'error', 'bug,' 'defect,' 'patch', 'mistake', 'fault', 'failure', 'fix', 'issue', 'incorrect', and 'flaw'. 
Then, a commit is considered a bug-fixing commit if its associated issue's tag name contains any of these keywords. 
Developers do not always associate a bug-fixing commit with an issue, though. 
Thus, CCC may miss some true positives here.
However, our approach is precise (e.g., more than those based on matching commit messages against such keywords~\cite{ray2016naturalness}). 
We prioritize precision over recall in our study as justified by our goal of 
studying cross-language bugs (that are actually so). 
%
By the end of this step, we obtained 54,356 bug-fixing commits.

\subsubsection{Cross-Language Code Revision Identification}\label{sss:ccri}
Now we check each bug-fixing commit against R2: the underlying bug may not be 
a CLB unless the commit is made to a project revision/version that is indeed multilingual (i.e., with cross-language interactions). 
Moreover, checking such interactions at the project level may not suffice because the language use and multilingual nature of a project may change across revisions~\cite{li2021understanding,wen22fse}, as we indeed encountered. 

We developed an automaton-based module in CCC to detect whether a project revision has language interactions via common Python-C or Java-C FFIs (e.g., {\tt Python C Extension} and {\tt JNI}), by extending PolyFax~\cite{wen22fsetool}, a language interfacing mechanism detector. The automaton transitions between states based on the presence of respective FFI's characteristics within the code. The automaton's entry into its final state signifies that the revision uses the particular FFI hence is multilingual. 
% Polyfax~\cite{wen22fsetool}, 
% Our module is based on PolyFax~\cite{wen22fsetool}, which supports only the first two types of FFI for Python/Java-C projects. 
% We extended it to support the other three types in order to comprehensively identify/classify any Python-C interaction in the given repository revision. 
After this step, we have 55,120 commits. 

\subsubsection{Cross-Language-Bug-Fixing Commit Identification}\label{sss:clbfci}
To ensure each commit (that satisfies R1 and R2) is further associated with a \textit{cross-language} bug, 
the changed code should be part of the cross-language behaviors of the revision. 
Such behaviors can be modeled by cross-language information flows/dependencies. 
Moreover, in an FFI-based Python-C or Java-C revision, language interactions are realized through cross-language APIs. 
Thus, a bug-fixing commit in a multilingual project (revision) is a CLBF commit 
if at least one of the changed code lines has a (transitive) dependence (backward or forward) relationship with code entities of the other language via at least one of the cross-language APIs. 

However, a static information flow/dependence analysis tool widely applicable to real-world Python-C or Java-C programs is not available~\cite{youn2023declarative}. 
The closest available one is Joern~\cite{yamaguchi2014modeling}, which supports intraprocedural control flow analysis for Python, Java, and C. 
Based on these capabilities, we extended Joern to build a whole-program cross-language interprocedural control flow graph (\textbf{CICFG}) for a given project (revision). 
A CICFG is directed graph where each node represents a statement in any of the two language units and each edge represents the control flow between two nodes. 

To construct the CICFG, CCC first obtains the control flow graph (CFG) of each method in each language unit as Joern immediately provides. 
Next, CCC builds the intra-language call graph for each language unit by traversing 
the per-method CFGs of that unit, and then builds the cross-language call graph from the two intra-language call graphs and call edges across the two languages. 
To identify the cross-language call edges, CCC uses calling-relation rules defined as per the respective FFI used (e.g., Python C Extension or JNI) according to their official specifications (e.g., cross-language function naming/calling conventions). 
Finally, based on the cross-language call graph and per-method CFGs, CCC builds the 
CICFG following the classical ICFG construction approach~\cite{sinha01apr}. 
To facilitate forward/backward traversal on it, the CICFG is annotated 
with function names and line numbers. 

CCC checks if a commit is CLBF as described earlier, but using CICFG to approximate cross-language dependencies (information flow). The resulting imprecision is resolved by our final confirmation during the manual bug analysis. The CICFG may also be incomplete (e.g., due to the lack of pointer/reference analysis in construction), which is acceptable for our bug collection purposes. 
After this step of CCC, we have 5,941 (likely CLBF) commits. 




% \subsection{Manual Confirmation}\label{ss:manconfirm}
% Through the three filters in CCC, the resulting commits are still likely to be false positives as CLBF commits, due to the (conservative) control flow approximation discussed above. 
% %Due to the lack of more advanced static analysis tools 
% Thus, we proceed with a manual confirmation process, during which 
% we manually check if each of those resulting commits is a true CLBF commit. 
% Specifically, given such a commit, we follow each control flow path (as produced by CCC) between one of the commit change locations and one of its reachable cross-language APIs, 
% identifying if the changes impact any of the API callsites through data flow hence data/control dependencies along the control-flow path. 
% If the impact exists, we confirm the commit as a CLBF commit and include it in our final CLBF commit set, and dismiss it from that set otherwise. 
% Initial decisions for each commit were made independently by three authors, followed by meetings/discussions to resolve any disagreements hence reaching a consensus. 
% %By manually dissecting how the commit impacts the cross-language information flow during this process, we also obtain a good understanding of how the associated bug occurs (e.g., how a data object created in Python is passed to and manipulated in C), which immediately facilitates our case study in the next step. 
% After this manual analysis, we have 1,237 confirmed CLBF commits.

% \subsection{Research Questions}\label{ss:rqs}
% The overarching goal of our study is to offer a comprehensive understanding of real-world multilingual bugs with respect to 
% their \textbf{5 aspects}: \textit{symptom}, \textit{location}, \textit{manifestation}, \textit{root cause}, and \textit{fixing strategy}. 

% Accordingly, we formulated the following five research questions, as outlined and justified below: 

% \textbf{\textit{RQ1: What are the symptoms of multilingual bugs?}} 
% This RQ aims to understand how these bugs are commonly 
% %symptomized or 
% externalized (as observed by developers or users). 
% The understanding not only serves an initial step of high-level detection of multilingual bugs, but also informs about their severity and consequences. 

% \textbf{\textit{RQ2: Where are multilingual bugs introduced?}} 
% This RQ aims to discover where these bugs are introduced in terms of code structural/syntactic contexts. 
% The result can shed light on the context in which multilingual bugs may happen hence helping developers understand where to avoid introducing such bugs.

% \textbf{\textit{RQ3: What are the manifestation characteristics of multilingual bugs?}} 
% This RQ aims to elucidate the code-level attributes regarding how these bugs are manifested, concerning the type (e.g., native versus foreign function) 
% and functional semantics (e.g., memory access versus I/O) of the cross-language APIs/functions involved as well as the direction and complexity of 
% underlying control/data flows. 
% The result can help design effective testing techniques to expose multilingual bugs. 

% \textbf{\textit{RQ4: What are the root causes of multilingual bugs?}} 
% This RQ aims to dissect the underlying causes of these bugs. 
% The result provides a basic understanding of multilingual bugs
% and immediate guidance for preventing, detecting/locating, 
% and resolving them. 

% \textbf{\textit{RQ5: How are multilingual bugs fixed?}} 
% This RQ aims to reveal how developers have fixed these bugs. 
% The result may help inform the development of better multilingual code debugging/repair tools and improve the patching process of multilingual bugs. 


\subsection{Manual Bug Analysis}\label{ss:studyprocedure}
To answer our RQs, we manually examine the CLBs associated with the confirmed, associated CLBF commits via case studies. 
The answers would involve terms/phrases that we had no full prior knowledge about. Thus, we adopted an open coding approach for each RQ, first 
deriving a codebook and then applying it to characterize each bug in each of the 5 aspects---both by three of the authors following 
a common inter-agreement and consensus procedure. 

\textit{\textbf{Random sampling for codebook.}}
To create the codebooks, we first randomly sampled 364 out of the 5,941 commits for analysis. This sample size is statistically significant at 95\% confidence level (CL) and 5\% margin of error (ME). 

\textit{\textbf{Derive codebooks.}}
We need a codebook %(e.g., for root cause taxonomy) 
for each RQ. %(e.g., RQ4). 
To that end, each author independently curated an initial catalog (e.g., of root cause) based on the 364 commits. 
Subsequently, they reconciled any differences until agreeing upon a finalized codebook. In particular, each participant (1) meticulously reviewed the commits, (2) evaluated whether each commit fell within the existing categories, and (3) forged a fresh category if necessary.
%
When formulating a new category, the initial step involved defining a label to encapsulate the bug aspect (e.g., root cause) presented in the commit. Following this, we crafted detailed descriptions for this new category, and identified that bug aspect that would appropriately fall under this category. The commit was then incorporated into the codebook, serving as an illustrative example for this new category.

%The codebooks for all of the other aspects of the cross-language bugs (e.g., symptom) were generated using a similar procedure.

\textit{\textbf{Random sampling for study.}}
Given the great time cost of manually examining even a single commit, we randomly sampled commits (other than the 364 for creating per-RQ codebooks) 
until we had 200 Python-C and 200 Java-C CLB cases, 400 \textit{confirmed} CLBs in total for the bug analysis. 
This sample size %(200) 
is statistically significant at 95\% CL and 5\% ME.  
%for each language combination. 

As during the sampling for codebook creation, the confirmation of a potential CLBF commit (identified by CCC) as corresponding to a true CLB is subsumed in the 
sampling here too. %, following a similar consensus procedure.  
The confirmation is to verify that the %cross-language interprocedural control flow 
underlying CICFG path actually bears relevant information flow. 

\textit{\textbf{Coding process.}} 
For each RQ, we applied the respective codebooks to answer it against each of the 400 CLBs. To ensure the reliability of this process, we utilized a negotiated agreement approach, which is often adopted when the main goal is to generate novel insights~\cite{morrissey1974sources}, as needed in our study.

For {RQ1}, we identify CLB symptoms per the issue/bug reports and any related documents they link to, developer-user discussions, bug-inducing code, and expected outputs, etc. 

For RQ2, we start with a forward traversal on the CICFG from the bug-fixing location,  
carefully examining the information flow (data/control dependencies), to pinpoint the bug location and name it per the respective codebook. 


For RQ3, starting from the bug location, a backward traversal on the CICFG is conducted until reaching the bug's source/origin in the other language. We identify cross-language functions encountered during the traversal, and then classify each as foreign, native, or NAX and its semantics as per its code (along with any comments and project documentation), language interfacing definitions, and official specification on foreign functions. 
The direction of responsible cross-language information flow is determined as follows:  
\begin{itemize}[leftmargin=*,topsep=2pt]
\item \textbf{Foreign language$\rightarrow$native language}: 
% The bug occurs in the foreign language unit, \textit{before} calling relevant native functions whose definition %(in the native language unit) 
% is reachable from the bug location via forward, but not via backward, traversal on the CICFG. 
The bug occurs in the foreign language unit, \textit{before} calling (returning to) relevant native functions whose definition %(in the native language unit) 
is reachable from the bug location via forward (backward) traversal on the CICFG. 
\item \textbf{Native language$\rightarrow$foreign language}:
\textcircled{1}The bug occurs in the native language unit, \textit{before} returning to the foreign language unit which is thus reachable from the bug location via either backward or forward CICFG traversal; OR 
%Thus, backward and forward traversal starting from the bug location will both reach Python code.
\textcircled{2}The bug occurs in the foreign language unit, \textit{after} calling relevant native functions whose definition %(in the native language unit) 
is reachable from the bug location via backward, but not via forward, CICFG traversal. 
%in C
%Thus, backward traversal starting from the bug location will reach C code, but forward traversal won’t reach C.
\end{itemize}

For RQ4, a deeper examination of the backward cross-language information flows from the bug location back to its source/origin is carried out to identify the bug's root cause, which is named per the respective codebook. 

For RQ5, the code changes in the associated CLBF commit are examined. The bug-fixing location is immediately identified and then named using the same codebook as in RQ2; the fixing strategy is summarized based on the semantic impact of the bug-fixing changes on the bug location. 

==> methodology-data.tex <==
\section{Methodology}\label{sec:methodology}

\subsection{Tool}

\subsubsection{Identify the interfacing types for Python-C}
Study for interaction method (total: 511)
28.57\% is inter-language project (146)
CE: 48.63\%
ctypes: 39.04\%
Cpython: 28.08\%
cython: 19.86\%
SWIG: 6.84\%
cffi: 7.53\%

Rule study, Priority: CE, ctypes, Cpython, cython, SWIG, cffi.


Evaluated this step of our tool on 100 samples 
Precision: 97\%, recall: 94\%,  F1: 95\%

==> methodology-old.tex <==
%
\section{Methodology}
% \subsection{Data Collection}
\subsection{Data Collection}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.9\linewidth]{figure/data_collection.pdf}
	\caption{The flow of our data collection process.}
	%Overview of the data processing}
	\label{fig:datacollect}
	\vspace{-12pt}
\end{figure}

\subsubsection{Limitation of Current Dataset}
With the rise of machine learning, a significant amount of data is required for model training. To fulfill this need, many researchers have provided an abundance of bug datasets. These datasets cover a wide array of programming languages and problem domains, assisting researchers and developers in better training and optimizing their models. For example,
Defects4J~\cite{just2014defects4j} is a rich dataset comprising 395 real-world bugs from various open-source Java projects, serving as a valuable resource for debugging and testing research. Codeflaws~\cite{tan2017codeflaws} includes 3,902 bugs of C programs extracted from the Codeforces competitive programming platform, providing an excellent basis for evaluating automated program repair tools. BugsInPy~\cite{widyasari2020bugsinpy} presents a carefully curated collection of 493 bugs derived from 17 diverse open-source Python projects, offering a comprehensive dataset for studying bugs in Python code. 

However, the bugs in these datasets primarily originate from projects using a single programming language. This implies that these datasets may not provide substantial assistance for multilingual software development. Particularly in today's globalized environment, software development often involves the combined use of multiple programming languages. Hence, there is an increasing demand for bug data and corresponding solutions that cater to multilingual environments.

\subsubsection{Repository mining}
Due to the lack of existing multilingual bug datasets, we need to collect such datasets in the first place for understanding/detecting multilingual bugs. %found in those projects. 
We chose GitHub as a data source because it is a widely-used platform for software development and version control, which means that it contains a large amount of real-world project code and associated metadata that can be used for various research purposes. Besides, we took Python and C as a starting point to address multilingual bugs for three reasons. 
First, Python and C are both top-10 popular languages, %so they are very popular. Therefore, 
and %Python and C 
have large, active communities that provide support and resources for developers. 
Second, C is a low-level programming language that is known for its %fast execution speeds 
high execution performance  
and efficient memory management. Python, on the other hand, is a high-level programming language that is known for its ease of use and readability. 
Third, Python and C, when combined, have a large ecosystem of libraries and modules that can be used for various tasks, such as machine learning (ML) and artificial intelligence (AI). 
It is well-known that the leading AI/ML frameworks, along with the huge corpus of applications based on them, are Python-C software~\cite{grichi2020impact}. 
Thus, Python-C software has a significant impact on modern lives and our society.
%By using both languages, one can access a wider range of libraries and modules that can be used to extend the functionality of your project.


% This \ul{\textit{first step}} aims to grab Python-C projects from GitHub. We decided to filter projects according to the number of stars because this number for %the number of stars on 
% a project can be used as a rough gauge of its popularity, as well as a way to gauge its activeness. %the activity of a project. 
% The higher the number of stars, the more people will pay attention to them and the more potential commits. Having a high number of stars on a GitHub project can suggest that the project is well-regarded by the community or widely used, and that its potential quality or usefulness may be higher compared to projects with lower numbers of stars. 
% According to the number of stars, we selected the top 23 popular projects, %most of which are widely used, including the {\tt Numpy} and {\tt pandas}. 
% These projects have a total of 60,180 commits. % at the time of our retrieval. 
% We totally found about 9871 projects using Python and C concurrently (more than 50 stars).

This \ul{\textit{first step}} aims to grab Python-C projects from GitHub. We decided to sort projects according to the number of stars because this number for a project can be used as a rough gauge of its popularity~\cite{ray2014large}, as well as a way to gauge its activeness. The higher the number of stars, the more people will pay attention to them and the more potential commits. Having a high number of stars on a GitHub project can suggest that the project is well-regarded by the community or widely used, and that its potential quality or usefulness may be higher compared to projects with lower numbers of stars. On the other hand, we hope to obtain more commits, which naturally requires more repositories. We do not want the number of repositories we fetch to be limited due to excessively high star count requirements. Therefore, to ensure an adequate quantity for trade-off, we have set the threshold for the number of stars at 10. We have obtained a list composed of 'x' repositories in total. Then we fetched 200 repositories. 

The \ul{\textit{second step}} is to fetch the commits from these repositories. During this step, in order to more conveniently determine whether the code changes in the commits were made to fix bugs, we must also obtain the issue number corresponding to each commit. We have obtained 'x' commits in total. In this step, we got 35,000 commits.


\subsection{Inter-language Bug-Fixing Commit Identification}
Inter-language bug-fixing commits in GitHub refer to the code commits that are not only in a multilingual project but also involve interaction between (i.e., code across) two languages. 
This definition of \ul{\textit{inter-language bug-fixing commit}} aims to distinguish it from other commits in multilingual projects in which two languages are used but do not interact with each other, as well as from the code commits that are irrelevant to any language interaction. Furthermore, for a commit to be classified as an "inter-language bug-fixing commit", it should also be specifically intended to address and rectify bugs in the system.
Accordingly, this \ul{\textit{second step}}, which aims to identify inter-language bug-fixing commits (per our definition), includes three substeps: (i) recognize the bug commits from all categories commits; (ii) fetch multilingual projects in which the languages do interact with each other; (iii) (only) in those projects, further identify code commits where the changed code involves language interaction.

These three filtering substeps, correspond to the three requirements:
\begin{itemize}[leftmargin=10pt,topsep=2pt]
\item The commits must be bug-related. This means that the changes made in these commits are intended to fix bugs in the code.

\item The version of the project in which the commits are located must be multilingual. This means the project uses multiple programming languages with language interaction.

\item There must be language interaction flow within the code change of commits. This means that the changes made in these commits involve interaction between different programming languages.
\end{itemize}

The time cost of these steps increases from the first to the third. By placing the most time-consuming step at the end, we can improve the efficiency of obtaining commits. This is because we can quickly filter out a large number of irrelevant commits in the early stages, reducing the amount of commits that needs to be processed in the more time-consuming final step. This order of operations allows us to maximize our efficiency and minimize unnecessary work.

% \textit{\textbf{Get inter-language commits}}. Inter-language commits in GitHub 
% %may not only refer to commits to a project that involves changes in multiple 
% %programming 
% %languages, but also the code that changes in the commits can cross the boundary between two languages. 
% refer to the code commits that are not only in a multilingual project but also 
% involve interaction between (i.e., code across) two languages. 
% Our definition of \ul{\textit{inter-language commit}} aims to distinguish it from other commits in multilingual 
% projects in which two languages are used but do not interact with each other. It is important to note that while some code defects %simple problems with code 
% in multilingual projects can also occur in single-language projects, the added complexity of working with multiple languages 
% %can increase the likelihood of such issues. 
% can still increase the likelihood that such issues occur. 
% Yet, we can tell if a bug in a multilingual project is indeed induced by language interaction according to whether one language can reach another via inter-language dependencies. Concerning efficiency, these dependencies may be approximated through whole-program control flow. 
% %So we can reflect the bugs caused by language interaction in multilingual projects by whether CFG can cross the language boundary to another language. 
% %We got 60,180 commits from the 23 projects.
% % We got 6,047,038 commits from the 9871 projects.

% First, we designed a state machine to detect whether there are common Python-C interaction behaviors and classify the interaction types---again, %because 
% a project may be programmed in Python and C at the same time, but there is no interaction between the two languages. Common interaction types include {\tt ctypes}, {\tt Cython}, {\tt SWIG}, and so on. Then, according to the interaction types adopted by the current project, we curated the list of cross-language API (i.e., function used for two languages to interact) names. 
% %the API function names that can interact between the two languages via our tool. 
% Next, we use our Joern-based~\cite{yamaguchi2014modeling} tool to query which statements are reachable from the changed code %in its original language 
% via (whole-program) control flow. Suppose these statements contain the interactive API function names we have obtained, we assume that the commit version of the project belongs to inter-language commits. After the two steps, we got 1,012 inter-language commits.


\textbf{\textit{Bug issue association}}. 
% The obtained commits contain various types of code changes, including bugs, clean-up, and additions of new features. Manually checking each commit would be time-consuming. %so instead, 
% Thus, the \ul{\textit{third step}} of our data collection 
% %our approach 
% aims to identify inter-language bug-fixing commits, starting with identifying
% relevant commits that are associated with an issue. When submitting a commit, developers sometimes associate the issue solved with the commit. And there is a label (i.e., tag) to classify the issue. We recorded the issue tags that are used to classify \textit{bugs}---not all issues correspond to code bugs, and took the names of those tags as keywords to filter our inter-language commits. 
% Such bug-related keywords we used include: {\tt 'error', 'bug,' 'defect,' 'patch', 'mistake', 'fault', 'failure', 'fix', 'issue', 'incorrect', 'flaw'}. 
% Then, we recognize an inter-language commit as a bug-fixing commit if it has any associated issue and the issue tag name includes any of the keywords. 
% Finally, we obtained 352 potential multilingual-bug-fixing commits. 
The commits we have obtained encompass a wide range of code changes, such as bug fixes, code clean-up, and the introduction of new features. Manually sifting through each commit would undoubtedly be a labor-intensive and time-consuming process. Given this, the first substep (i) of our data collection process is designed to pinpoint bug-fixing commits. We begin by identifying relevant commits that are associated with a particular issue. 

Refer to \cite{ray2016naturalness}, a commit is considered bug-relevant if its message contains keywords (such as "error", "bug", etc.). In the software development process, developers often associate the resolution of an issue with a specific commit when they submit it. Furthermore, the issues themselves often have labels (i.e., tags), which classify their nature. So we think the keywords in the label of a commit offer a more accurate reflection of the commit's type. Consequently, we specifically recorded the issue tags used to classify bugs, and used the names of these tags as keywords to filter our commits. 

The bug-related keywords we utilized for this process include terms such as 'error', 'bug,' 'defect,' 'patch', 'mistake', 'fault', 'failure', 'fix', 'issue', 'incorrect', and 'flaw'. With these keywords, we are able to filter through the commits effectively. After this filtration process, we categorize a commit as a bug-fixing commit if it is associated with an issue and if the issue's tag name contains any of the aforementioned keywords. After filtering via bug issue, we ended up with 11,000 commits.

\textbf{\textit{Automaton-based language interaction}}.
We observed that some repositories may have language interaction at a certain period (e.g., via ctypes). However, due to version updates and design changes, they may have removed the language interaction in later versions (i.e., no longer using ctypes). To avoid this situation, we perform identification on the repository of each commit's version. This helps to filter out unnecessary commits for substep (iii).

Specifically, for substep (ii), we designed an automaton-based identification machine (following the design in PolyFax~\cite{wen22fsetool}) 
to detect whether there are common Python-C interaction behaviors and classify the interaction types---%again, %because 
a project may be programmed in Python and C at the same time, but there is no interaction between the two languages. Common Python-C interaction types include {\tt ctypes}, {\tt Cython}, {\tt SWIG}, etc.. %According to the interaction types adopted by the 23 projects, we curated the list of cross-language API (i.e., function used for the two languages to interact) names for %Python-C software. 
%each type. 
%the API function names that can interact between the two languages via our tool.
% Based on these lists, the language interfacing classification engine recognizes a given multilingual project 
% as having any language interaction (i.e., at least one of those interaction types) 
% or not (i.e., none of the types is identified). 
%Further details of the statement machine design can be found in~\cite{wen22fsetool}. 
Based on these types, the automaton-based identification machine (ABIM) recognizes a given multilingual project 
as having any language interaction (i.e., at least one of those interaction types) or not (i.e., none of the types is identified). 

ABIM consists of two collaborating modules: identification encode and identification scan. The ABIM takes a multi-language project repository as input and provides the set of interfacing mechanism labels as output. The identification encode module encodes the source code files of the input repository into a feature vector representation. The identification scan module then uses the encoded feature vectors to identify the interfacing mechanisms used in the input repository. And then output a label that can show whether the repository has language interaction. Filtering with the ABIM left us with 4,300 commits.

\textbf{\textit{Joern control-flow reachability based identification}}. 
% For substep (ii), ideally we need to check whether one language can reach another via inter-language dependencies. Yet concerning efficiency, we approximate these dependencies via whole-program control flow. 
% Then, we consider a code commit involves language interaction if any cross-language API in the curated list (for the respective interaction type identified in substep (i)) is reachable from any of the changed code lines in the commit. 
% To that end, we developed a dedicated tool based on 
% Joern~\cite{yamaguchi2014modeling}---expanding it by adding whole-program control flow reachability analysis.
% After both substeps, we obtained 1,012 inter-language commits.
Since this situation exists where, in the inter-language repository, the code changes occurring in its commits do not involve interaction between languages. Once we have obtained the inter-language repository, our next step is to ascertain if one language can reach another via inter-language dependencies in a commit. This exploration is vital in understanding the interoperability of different languages within a system. However, due to concerns about efficiency, we make an approximation of these dependencies using whole-program control flow. This approach provides a broad overview of how control passes between different parts of the program, thereby offering insights into potential points of inter-language interaction.

Following this, we evaluate whether a bug-fixing commit involves language interaction. We make this determination based on whether any cross-language API from our curated list, which corresponds to the identified interaction type in the inter-language repository, is reachable from any of the lines of code altered in the commit. In other words, if a code change can potentially affect or is affected by a cross-language API, we consider that bug-fixing commit to involve language interaction.

To facilitate this process, we have developed a dedicated tool, which is based on Joern~
\cite{yamaguchi2014modeling} - a powerful platform for the analysis of code. We have expanded Joern's capabilities by integrating whole-program control flow reachability analysis into it. This new feature enables us to trace the potential propagation of changes across the entire codebase, thereby allowing us to better identify and understand the points of inter-language interaction in the system.

Through the Joern-based identification, we have filtered out commits that exclude language interaction from the inter-language project, i.e., only left inter-language bug-fixing commits. These commits constitute the Inter-language Bug Dataset. After filtering via joern-based identification, we ended up with 1,700 commits.


\subsection{Manual confirmation}
In our previous collection step, we chose to use a Joern-based identification that evaluates based on control flow. Control flow is a model that describes the order in which the operations in a program are executed and exposes the structure of the program through its branches and loops. By analyzing control flow, we can determine under which conditions code blocks are executed and their order of execution, thereby revealing potential language interactions. For instance, if a Python function calls a C function, this interaction would be represented as an edge from the Python code block to the C code block in the control flow graph.

However, the control flow-based analysis method also has its limitations. While control flow can illustrate the execution paths of the code, it doesn't accurately represent how data flows through a program. This is particularly important in a multi-language environment, as data interaction between different languages can lead to unexpected behavior or bugs. For example, if a Python variable is passed to a C function and modified there, this data flow would not be directly visible in the control flow graph.

Due to the lack of tools specifically designed for multi-language interaction, we need to manually analyze the code changes in commits to determine whether they exist in the data flow of language interaction. By analyzing data flow, we can gain a more comprehensive understanding of how different languages interact, especially how they share and manipulate data. Consequently, we can more accurately identify potential sources of bugs, such as type errors that may occur when data is passed from one language to another, or memory management issues that may arise when C code manipulates Python objects. Additionally, data flow analysis can also help us identify potential optimization points, such as improving code efficiency by reducing unnecessary data conversions or copies. Through the manual analysis, we got 1,039 commits.


\subsection{Research Question}
We intend to understand multilingual bugs in Python-C projects via case studies. This type of case study can assist in identifying common patterns and causes of multilingual bugs and shed light on how to avoid them in future software development. The case study of multilingual defects can provide a comprehensive analysis of the bugs' root causes, the location of bugs, and the methods taken to fix them. This information is valuable for other developers and organizations. It can also provide a greater understanding of the intricacies of multilingual systems, which can inform future development best practices. In general, our case study on multilingual issues can enhance the quality and dependability of multilingual software and provide significant insights for future development.

Using the inter-language bug-fixing commits, we seek to answer three research questions in relation. Below, we clarify the aim and justification for each question with respect to our study goal.% and describe our approach to answering it. 

\textbf{\textit{RQ1: What are the symptoms of multilingual bugs?}} This RQ aims to understand the general symptoms of multilingual bugs. It is designed to delve deeper into the characteristics of these bugs in different coding languages. The understanding obtained through this RQ could provide valuable context and a broader perspective when investigating and resolving such issues. Furthermore, it could contribute to the development of more efficient and effective prevention and mitigation strategies in the multilingual programming environment.

\textbf{\textit{RQ2: where do multilingual bugs typically introducing?}} This study aims to shed light on the context in which multilingual bugs may happen hence helping developers understand where to avoid such bugs.

\textbf{\textit{RQ3: What are the manifestation characteristics of multilingual bugs?}} This RQ aims to elucidate the distinct attributes and patterns that define multilingual bugs. In particular, focusing on two primary factors - the semantic type of the cross-language API involved and the data/control flow direction and complexity. By examining these, this research question intends to paint a comprehensive picture of the manifestation characteristics of multilingual bugs, which could guide more effective strategies for their detection and resolution.

\textbf{\textit{RQ4: What are the root causes of multilingual bugs and how are they specific to multilingual projects?}} This RQ aims to delve into the underlying causes that give rise to multilingual bugs. We are particularly intrigued by those unique and unconventional root causes that have not been addressed or captured in previous studies. By understanding these causes, we can gain a more comprehensive understanding of the complexities and challenges associated with multilingual projects, and potentially develop more effective strategies for bug prevention and resolution.

\textbf{\textit{RQ5: How are multilingual bugs fixed?}} This study aims to help inform the development of better and more efficient debugging tools for multilingual software. Multilingual bugs can affect the functionality, usability, and user experience of software applications. Hence, it's crucial to understand the ways these bugs are fixed, to facilitate the development of more effective debugging tools.


\subsection{Case study procedure}
For the next step, we need to derive a codebook and then apply it for the categorization of inter-language bug-fixing commits.
\textit{\textbf{Random sampling for codebook}}
To manually generate the codebook, we first randomly sampled 281 out of the 1,039 commits for analysis. This sample size is statistically significant at 95\% confidence level (CL) and 5\% margin of error (ME). 

\textit{\textbf{Derive codebook}}
As for root cause code book: three of the authors independently curated an initial catalog of root cause categories, basing it on the 281 commits. Subsequently, we reconciled any differences until we agreed upon a finalized codebook. In greater detail, each participant (1) meticulously reviewed the commits, (2) evaluated whether each commit fell within the existing issue categories, and (3) forged a fresh category if the need arose.

In the process of formulating a new category, the initial step involved defining a label to encapsulate the root cause presented in the commit. Following this, we crafted detailed descriptions for this new category, and identified root cause that would appropriately fall under this category. The commit was then incorporated into the codebook, serving as an illustrative example for this new category.

Note that: the codebooks for other aspects of the analysis (e.g., symptom) were generated using similar methods.


\textit{\textbf{Random sampling for study}}
Taking into account the considerable time expenditure often associated with manually reviewing even a single commit, we randomly selected 216 commits requiring manual verification during the coding procedure. This sample size is statistically significant at 90\% CL and 5\% ME. 

\textit{\textbf{Coding process}}. 
In order to guarantee the reliability of our coding process, we utilized a negotiated agreement approach. This strategy is especially advantageous in research contexts such as ours, where the primary goal is to generate novel insights~\cite{morrissey1974sources}.

==> methodology.tex <==
%
\section{Methodology}
% \subsection{Data Collection}
\subsection{Data Collection}
\begin{figure}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.9\linewidth]{figure/data_collection.pdf}
	\caption{The flow of our data collection process.}
	%Overview of the data processing}
	\label{fig:datacollect}
	\vspace{-12pt}
\end{figure}

\subsubsection{Limitation of Current Dataset}
With the rise of machine learning, a significant amount of data is required for model training. To fulfill this need, many researchers have provided an abundance of bug datasets. These datasets cover a wide array of programming languages and problem domains, assisting researchers and developers in better training and optimizing their models. For example,
Defects4J~\cite{just2014defects4j} is a rich dataset comprising 395 real-world bugs from various open-source Java projects, serving as a valuable resource for debugging and testing research. Codeflaws~\cite{tan2017codeflaws} includes 3,902 bugs of C programs extracted from the Codeforces competitive programming platform, providing an excellent basis for evaluating automated program repair tools. BugsInPy~\cite{widyasari2020bugsinpy} presents a carefully curated collection of 493 bugs derived from 17 diverse open-source Python projects, offering a comprehensive dataset for studying bugs in Python code. 

However, the bugs in these datasets primarily originate from projects using a single programming language. This implies that these datasets may not provide substantial assistance for multilingual software development. Particularly in today's globalized environment, software development often involves the combined use of multiple programming languages. Hence, there is an increasing demand for bug data and corresponding solutions that cater to multilingual environments.

\subsubsection{Repository mining}
Due to the lack of existing multilingual bug datasets, we need to collect such datasets in the first place for understanding/detecting multilingual bugs. %found in those projects. 
We chose GitHub as a data source because it is a widely-used platform for software development and version control, which means that it contains a large amount of real-world project code and associated metadata that can be used for various research purposes. Besides, we took Python and C as a starting point to address multilingual bugs for three reasons. 
First, Python and C are both top-10 popular languages, %so they are very popular. Therefore, 
and %Python and C 
have large, active communities that provide support and resources for developers. 
Second, C is a low-level programming language that is known for its %fast execution speeds 
high execution performance  
and efficient memory management. Python, on the other hand, is a high-level programming language that is known for its ease of use and readability. 
Third, Python and C, when combined, have a large ecosystem of libraries and modules that can be used for various tasks, such as machine learning (ML) and artificial intelligence (AI). 
It is well-known that the leading AI/ML frameworks, along with the huge corpus of applications based on them, are Python-C software~\cite{grichi2020impact}. 
Thus, Python-C software has a significant impact on modern lives and our society.
%By using both languages, one can access a wider range of libraries and modules that can be used to extend the functionality of your project.


% This \ul{\textit{first step}} aims to grab Python-C projects from GitHub. We decided to filter projects according to the number of stars because this number for %the number of stars on 
% a project can be used as a rough gauge of its popularity, as well as a way to gauge its activeness. %the activity of a project. 
% The higher the number of stars, the more people will pay attention to them and the more potential commits. Having a high number of stars on a GitHub project can suggest that the project is well-regarded by the community or widely used, and that its potential quality or usefulness may be higher compared to projects with lower numbers of stars. 
% According to the number of stars, we selected the top 23 popular projects, %most of which are widely used, including the {\tt Numpy} and {\tt pandas}. 
% These projects have a total of 60,180 commits. % at the time of our retrieval. 
% We totally found about 9871 projects using Python and C concurrently (more than 50 stars).

This \ul{\textit{first step}} aims to grab Python-C projects from GitHub. We decided to sort projects according to the number of stars because this number for a project can be used as a rough gauge of its popularity~\cite{ray2014large}, as well as a way to gauge its activeness. The higher the number of stars, the more people will pay attention to them and the more potential commits. Having a high number of stars on a GitHub project can suggest that the project is well-regarded by the community or widely used, and that its potential quality or usefulness may be higher compared to projects with lower numbers of stars. On the other hand, we hope to obtain more commits, which naturally requires more repositories. We do not want the number of repositories we fetch to be limited due to excessively high star count requirements. Therefore, to ensure an adequate quantity for trade-off, we have set the threshold for the number of stars at 10. We have obtained a list composed of 'x' repositories in total. Then we fetched 200 repositories. 

The \ul{\textit{second step}} is to fetch the commits from these repositories. During this step, in order to more conveniently determine whether the code changes in the commits were made to fix bugs, we must also obtain the issue number corresponding to each commit. We have obtained 'x' commits in total. In this step, we got 35,000 commits.


\subsection{Inter-language Bug-Fixing Commit Identification}
Inter-language bug-fixing commits in GitHub refer to the code commits that are not only in a multilingual project but also involve interaction between (i.e., code across) two languages. 
This definition of \ul{\textit{inter-language bug-fixing commit}} aims to distinguish it from other commits in multilingual projects in which two languages are used but do not interact with each other, as well as from the code commits that are irrelevant to any language interaction. Furthermore, for a commit to be classified as an "inter-language bug-fixing commit", it should also be specifically intended to address and rectify bugs in the system.
Accordingly, this \ul{\textit{second step}}, which aims to identify inter-language bug-fixing commits (per our definition), includes three substeps: (i) recognize the bug commits from all categories commits; (ii) fetch multilingual projects in which the languages do interact with each other; (iii) (only) in those projects, further identify code commits where the changed code involves language interaction.

These three filtering substeps, correspond to the three requirements:
\begin{itemize}[leftmargin=10pt,topsep=2pt]
\item The commits must be bug-related. This means that the changes made in these commits are intended to fix bugs in the code.

\item The version of the project in which the commits are located must be multilingual. This means the project uses multiple programming languages with language interaction.

\item There must be language interaction flow within the code change of commits. This means that the changes made in these commits involve interaction between different programming languages.
\end{itemize}

The time cost of these steps increases from the first to the third. By placing the most time-consuming step at the end, we can improve the efficiency of obtaining commits. This is because we can quickly filter out a large number of irrelevant commits in the early stages, reducing the amount of commits that needs to be processed in the more time-consuming final step. This order of operations allows us to maximize our efficiency and minimize unnecessary work.

% \textit{\textbf{Get inter-language commits}}. Inter-language commits in GitHub 
% %may not only refer to commits to a project that involves changes in multiple 
% %programming 
% %languages, but also the code that changes in the commits can cross the boundary between two languages. 
% refer to the code commits that are not only in a multilingual project but also 
% involve interaction between (i.e., code across) two languages. 
% Our definition of \ul{\textit{inter-language commit}} aims to distinguish it from other commits in multilingual 
% projects in which two languages are used but do not interact with each other. It is important to note that while some code defects %simple problems with code 
% in multilingual projects can also occur in single-language projects, the added complexity of working with multiple languages 
% %can increase the likelihood of such issues. 
% can still increase the likelihood that such issues occur. 
% Yet, we can tell if a bug in a multilingual project is indeed induced by language interaction according to whether one language can reach another via inter-language dependencies. Concerning efficiency, these dependencies may be approximated through whole-program control flow. 
% %So we can reflect the bugs caused by language interaction in multilingual projects by whether CFG can cross the language boundary to another language. 
% %We got 60,180 commits from the 23 projects.
% % We got 6,047,038 commits from the 9871 projects.

% First, we designed a state machine to detect whether there are common Python-C interaction behaviors and classify the interaction types---again, %because 
% a project may be programmed in Python and C at the same time, but there is no interaction between the two languages. Common interaction types include {\tt ctypes}, {\tt Cython}, {\tt SWIG}, and so on. Then, according to the interaction types adopted by the current project, we curated the list of cross-language API (i.e., function used for two languages to interact) names. 
% %the API function names that can interact between the two languages via our tool. 
% Next, we use our Joern-based~\cite{yamaguchi2014modeling} tool to query which statements are reachable from the changed code %in its original language 
% via (whole-program) control flow. Suppose these statements contain the interactive API function names we have obtained, we assume that the commit version of the project belongs to inter-language commits. After the two steps, we got 1,012 inter-language commits.


\textbf{\textit{Bug issue association}}. 
% The obtained commits contain various types of code changes, including bugs, clean-up, and additions of new features. Manually checking each commit would be time-consuming. %so instead, 
% Thus, the \ul{\textit{third step}} of our data collection 
% %our approach 
% aims to identify inter-language bug-fixing commits, starting with identifying
% relevant commits that are associated with an issue. When submitting a commit, developers sometimes associate the issue solved with the commit. And there is a label (i.e., tag) to classify the issue. We recorded the issue tags that are used to classify \textit{bugs}---not all issues correspond to code bugs, and took the names of those tags as keywords to filter our inter-language commits. 
% Such bug-related keywords we used include: {\tt 'error', 'bug,' 'defect,' 'patch', 'mistake', 'fault', 'failure', 'fix', 'issue', 'incorrect', 'flaw'}. 
% Then, we recognize an inter-language commit as a bug-fixing commit if it has any associated issue and the issue tag name includes any of the keywords. 
% Finally, we obtained 352 potential multilingual-bug-fixing commits. 
The commits we have obtained encompass a wide range of code changes, such as bug fixes, code clean-up, and the introduction of new features. Manually sifting through each commit would undoubtedly be a labor-intensive and time-consuming process. Given this, the first substep (i) of our data collection process is designed to pinpoint bug-fixing commits. We begin by identifying relevant commits that are associated with a particular issue. 

Refer to \cite{ray2016naturalness}, a commit is considered bug-relevant if its message contains keywords (such as "error", "bug", etc.). In the software development process, developers often associate the resolution of an issue with a specific commit when they submit it. Furthermore, the issues themselves often have labels (i.e., tags), which classify their nature. So we think the keywords in the label of a commit offer a more accurate reflection of the commit's type. Consequently, we specifically recorded the issue tags used to classify bugs, and used the names of these tags as keywords to filter our commits. 

The bug-related keywords we utilized for this process include terms such as 'error', 'bug,' 'defect,' 'patch', 'mistake', 'fault', 'failure', 'fix', 'issue', 'incorrect', and 'flaw'. With these keywords, we are able to filter through the commits effectively. After this filtration process, we categorize a commit as a bug-fixing commit if it is associated with an issue and if the issue's tag name contains any of the aforementioned keywords. After filtering via bug issue, we ended up with 11,000 commits.

\textbf{\textit{Automaton-based language interaction}}.
We observed that some repositories may have language interaction at a certain period (e.g., via ctypes). However, due to version updates and design changes, they may have removed the language interaction in later versions (i.e., no longer using ctypes). To avoid this situation, we perform identification on the repository of each commit's version. This helps to filter out unnecessary commits for substep (iii).

Specifically, for substep (ii), we designed an automaton-based identification machine (following the design in PolyFax~\cite{wen22fsetool}) 
to detect whether there are common Python-C interaction behaviors and classify the interaction types---%again, %because 
a project may be programmed in Python and C at the same time, but there is no interaction between the two languages. Common Python-C interaction types include {\tt ctypes}, {\tt Cython}, {\tt SWIG}, etc.. %According to the interaction types adopted by the 23 projects, we curated the list of cross-language API (i.e., function used for the two languages to interact) names for %Python-C software. 
%each type. 
%the API function names that can interact between the two languages via our tool.
% Based on these lists, the language interfacing classification engine recognizes a given multilingual project 
% as having any language interaction (i.e., at least one of those interaction types) 
% or not (i.e., none of the types is identified). 
%Further details of the statement machine design can be found in~\cite{wen22fsetool}. 
Based on these types, the automaton-based identification machine (ABIM) recognizes a given multilingual project 
as having any language interaction (i.e., at least one of those interaction types) or not (i.e., none of the types is identified). 

ABIM consists of two collaborating modules: identification encode and identification scan. The ABIM takes a multi-language project repository as input and provides the set of interfacing mechanism labels as output. The identification encode module encodes the source code files of the input repository into a feature vector representation. The identification scan module then uses the encoded feature vectors to identify the interfacing mechanisms used in the input repository. And then output a label that can show whether the repository has language interaction. Filtering with the ABIM left us with 4,300 commits.

\textbf{\textit{Joern control-flow reachability based identification}}. 
% For substep (ii), ideally we need to check whether one language can reach another via inter-language dependencies. Yet concerning efficiency, we approximate these dependencies via whole-program control flow. 
% Then, we consider a code commit involves language interaction if any cross-language API in the curated list (for the respective interaction type identified in substep (i)) is reachable from any of the changed code lines in the commit. 
% To that end, we developed a dedicated tool based on 
% Joern~\cite{yamaguchi2014modeling}---expanding it by adding whole-program control flow reachability analysis.
% After both substeps, we obtained 1,012 inter-language commits.
Since this situation exists where, in the inter-language repository, the code changes occurring in its commits do not involve interaction between languages. Once we have obtained the inter-language repository, our next step is to ascertain if one language can reach another via inter-language dependencies in a commit. This exploration is vital in understanding the interoperability of different languages within a system. However, due to concerns about efficiency, we make an approximation of these dependencies using whole-program control flow. This approach provides a broad overview of how control passes between different parts of the program, thereby offering insights into potential points of inter-language interaction.

Following this, we evaluate whether a bug-fixing commit involves language interaction. We make this determination based on whether any cross-language API from our curated list, which corresponds to the identified interaction type in the inter-language repository, is reachable from any of the lines of code altered in the commit. In other words, if a code change can potentially affect or is affected by a cross-language API, we consider that bug-fixing commit to involve language interaction.

To facilitate this process, we have developed a dedicated tool, which is based on Joern~
\cite{yamaguchi2014modeling} - a powerful platform for the analysis of code. We have expanded Joern's capabilities by integrating whole-program control flow reachability analysis into it. This new feature enables us to trace the potential propagation of changes across the entire codebase, thereby allowing us to better identify and understand the points of inter-language interaction in the system.

Through the Joern-based identification, we have filtered out commits that exclude language interaction from the inter-language project, i.e., only left inter-language bug-fixing commits. These commits constitute the Inter-language Bug Dataset. After filtering via joern-based identification, we ended up with 1,700 commits.


\subsection{Manual confirmation}
In our previous collection step, we chose to use a Joern-based identification that evaluates based on control flow. Control flow is a model that describes the order in which the operations in a program are executed and exposes the structure of the program through its branches and loops. By analyzing control flow, we can determine under which conditions code blocks are executed and their order of execution, thereby revealing potential language interactions. For instance, if a Python function calls a C function, this interaction would be represented as an edge from the Python code block to the C code block in the control flow graph.

However, the control flow-based analysis method also has its limitations. While control flow can illustrate the execution paths of the code, it doesn't accurately represent how data flows through a program. This is particularly important in a multi-language environment, as data interaction between different languages can lead to unexpected behavior or bugs. For example, if a Python variable is passed to a C function and modified there, this data flow would not be directly visible in the control flow graph.

Due to the lack of tools specifically designed for multi-language interaction, we need to manually analyze the code changes in commits to determine whether they exist in the data flow of language interaction. By analyzing data flow, we can gain a more comprehensive understanding of how different languages interact, especially how they share and manipulate data. Consequently, we can more accurately identify potential sources of bugs, such as type errors that may occur when data is passed from one language to another, or memory management issues that may arise when C code manipulates Python objects. Additionally, data flow analysis can also help us identify potential optimization points, such as improving code efficiency by reducing unnecessary data conversions or copies. Through the manual analysis, we got 1,039 commits.


\subsection{Research Question}
We intend to understand multilingual bugs in Python-C projects via case studies. This type of case study can assist in identifying common patterns and causes of multilingual bugs and shed light on how to avoid them in future software development. The case study of multilingual defects can provide a comprehensive analysis of the bugs' root causes, the location of bugs, and the methods taken to fix them. This information is valuable for other developers and organizations. It can also provide a greater understanding of the intricacies of multilingual systems, which can inform future development best practices. In general, our case study on multilingual issues can enhance the quality and dependability of multilingual software and provide significant insights for future development.

Using the inter-language bug-fixing commits, we seek to answer three research questions in relation. Below, we clarify the aim and justification for each question with respect to our study goal.% and describe our approach to answering it. 

\textbf{\textit{RQ1: What are the symptoms of multilingual bugs?}} This RQ aims to understand the general symptoms of multilingual bugs. It is designed to delve deeper into the characteristics of these bugs in different coding languages. The understanding obtained through this RQ could provide valuable context and a broader perspective when investigating and resolving such issues. Furthermore, it could contribute to the development of more efficient and effective prevention and mitigation strategies in the multilingual programming environment.

\textbf{\textit{RQ2: where do multilingual bugs typically introducing?}} This study aims to shed light on the context in which multilingual bugs may happen hence helping developers understand where to avoid such bugs.

\textbf{\textit{RQ3: What are the manifestation characteristics of multilingual bugs?}} This RQ aims to elucidate the distinct attributes and patterns that define multilingual bugs. In particular, focusing on two primary factors - the semantic type of the cross-language API involved and the data/control flow direction and complexity. By examining these, this research question intends to paint a comprehensive picture of the manifestation characteristics of multilingual bugs, which could guide more effective strategies for their detection and resolution.

\textbf{\textit{RQ4: What are the root causes of multilingual bugs and how are they specific to multilingual projects?}} This RQ aims to delve into the underlying causes that give rise to multilingual bugs. We are particularly intrigued by those unique and unconventional root causes that have not been addressed or captured in previous studies. By understanding these causes, we can gain a more comprehensive understanding of the complexities and challenges associated with multilingual projects, and potentially develop more effective strategies for bug prevention and resolution.

\textbf{\textit{RQ5: How are multilingual bugs fixed?}} This study aims to help inform the development of better and more efficient debugging tools for multilingual software. Multilingual bugs can affect the functionality, usability, and user experience of software applications. Hence, it's crucial to understand the ways these bugs are fixed, to facilitate the development of more effective debugging tools.


\subsection{Case study procedure}
For the next step, we need to derive a codebook and then apply it for the categorization of inter-language bug-fixing commits.
\textit{\textbf{Random sampling for codebook}}
To manually generate the codebook, we first randomly sampled 281 out of the 1,039 commits for analysis. This sample size is statistically significant at 95\% confidence level (CL) and 5\% margin of error (ME). 

\textit{\textbf{Derive codebook}}
As for root cause code book: three of the authors independently curated an initial catalog of root cause categories, basing it on the 281 commits. Subsequently, we reconciled any differences until we agreed upon a finalized codebook. In greater detail, each participant (1) meticulously reviewed the commits, (2) evaluated whether each commit fell within the existing issue categories, and (3) forged a fresh category if the need arose.

In the process of formulating a new category, the initial step involved defining a label to encapsulate the root cause presented in the commit. Following this, we crafted detailed descriptions for this new category, and identified root cause that would appropriately fall under this category. The commit was then incorporated into the codebook, serving as an illustrative example for this new category.

Note that: the codebooks for other aspects of the analysis (e.g., symptom) were generated using similar methods.


\textit{\textbf{Random sampling for study}}
Taking into account the considerable time expenditure often associated with manually reviewing even a single commit, we randomly selected 216 commits requiring manual verification during the coding procedure. This sample size is statistically significant at 90\% CL and 5\% ME. 

\textit{\textbf{Coding process}}. 
In order to guarantee the reliability of our coding process, we utilized a negotiated agreement approach. This strategy is especially advantageous in research contexts such as ours, where the primary goal is to generate novel insights~\cite{morrissey1974sources}.

==> related-cai.tex <==
%!TEX root = paper.tex

\section{Related Work}
%\vspace{-2pt}
% \noindent
% \textbf{Studies on multilingual software}. 
% A notable and increasing number of studies have targeted multilingual software, of which many are mainly focused on the diversity~\cite{tomassetti2014empirical} 
% and usage of languages~\cite{jones2009software,vasilescu2013babel,steffen2019language,mayer2015empirical} as well as their evolution~\cite{karus2011study,chen2005empirical,li2021understanding}. 
% A few others looked further into language companionship~\cite{bissyande2013popularity} and 
% linkage/interaction between languages~\cite{mayer2017multi}, as well as 
% the effects of multilingual development on the maintenance/comprehension~\cite{kontogiannis2006comprehension,grichi2020impact} or  
% quality of resulting software~\cite{kochhar2016large,grichi2020impactjni,abidi2021multi}.
% Most of these studies are based on multilingual code, but some of them 
% are performed from human-factor perspectives~\cite{abidi2019behind,mayer2017multi}. 
% %
% Our study clearly differs from these prior relevant ones in that it focuses on multilingual bugs, based on real-world software code and comprehensively examining root causes, fault location patterns, and how to fix the bugs. 
%
%\vspace{2pt}\noindent
%\textbf{Studies on code defects}. 
%
%Researchers have investigated various aspects (e.g., presence, causes, manifestation, and/or fixing strategies) of particular kinds of bugs in different software application domains. For instance, 
%
% In~\cite{jin2012understanding} the authors examined various aspects (e.g., presence, causes, fixes) of performance bugs in %real-world systems such as 
% GCC, Mozilla, and MySQL. 
% Following a similar methodology, %therein, as we also did in this paper, 
% the study in~\cite{liu2014characterizing} targeted performance bugs too, but concerning those in Android apps. 
% Our study also addresses the same aspects, yet with a focus on those in multilingual software and a broad scope of bugs instead of performance bugs only. 

%Several related studies~\cite{wen22fse,grichi2020impactjni,kochhar2016large} are aimed to discover statistical associations of interest based on potential defect indicators, rather than on actual code bugs. 
%And a few others~\cite{berger2019impact,ray2014large,zhang2019study} 
%are not really concerned about multilingual code---instead, they mainly addressed single-language software despite looking at a variety of languages. 
Several studies
~\cite{berger2019impact,ray2014large,zhang2019study} 
are not really concerned about multilingual code---instead, they mainly addressed single-language software despite looking at a variety of languages. 
In contrast, we study cross-language defects that have been confirmed as bugs at code level. 
%
% \vspace{2pt}
% \noindent
% \textbf{Fault detection/localization}. 
% Existing approaches in this line are either mainly based on program analysis or largely data-driven (e.g., based on machine/deep learning (DL)). 
% The first category predominantly focuses on JNI (i.e., Java-C) programs as one particular case of multilingual software~\cite{hwang2021justgen,lee2020broadening, xue2018ndroid,bai2018bridgetaint,bae2019towards}, with fewer ones targeting Python-C software~\cite{wen22usenixsecurity,wen23usenixsecurity} which are dynamic techniques. 
% The second category is represented on emerging DL-based fault localization techniques~\cite{fu2022linevul,li2019deepfl,li2021fault,li2022fault}. 
% In comparison with most of these existing techniques, which cannot work 
% with multilingual (Python-C) code as the only input (e.g., they require test cases), {\tech} is a transformer-based \textit{static} Python-C bug detector that only needs that input. 
% Our approach is also different from 
% the most similar prior technique (i.e.,~\cite{fu2022linevul}) in its novel position encoding design tailored for capturing \textit{multilingual} bugs. 
%
%\vspace{2pt}\noindent
%\textbf{Studies on issues/bugs in multilingual software}. 
%A few latest works attempted to examine development issues with multilingual software and bugs in those systems. 
%In particular, 
Yang et al.~\cite{yang2023demystifying} manually inspected 586 Stack-Overflow posts related to those issues, while dissecting challenges behind the issues and summarizing current solutions. The study is based on developers' discussions rather than multilingual code. 
%and addresses a range of issues concerning system design, build, and construction. 
Li et al. investigated %looked into bugs in multilingual software, focusing on 
characteristics of bug resolution (e.g., bug open time and reopen rate) in 54 Apache projects~\cite{li2023understandinga} and those of bugs themselves (e.g., code change complexity) in 3 machine-learning frameworks~\cite{li2023understandingb}. 
Like ours, these two studies are based on code artifacts. %; but, the bugs examined are not necessarily \textit{multilingual} bugs as we defined---fixing them may involve changing code of different languages~\cite{li2023understandinga}, yet each bug itself may not be induced by cross-language code behaviors. 
Yet neither the bugs nor the projects were necessarily \textit{multilingual}---they were defined by involving multiple languages without concerning 
%cross-language behaviors based on 
language interactions. %~\cite{li2023understandinga,li2023understandingb}. 
Also, unlike these works, we address code-level root cause, location, manifestation, and fixing strategies of multilingual code bugs without being limited to specific software domains. 

Sultana et al.~\cite{sultana2016understanding} conducted a case study of interoperability issues in 20 C/Fortran applications, focusing on the declaration, data sharing, and parameter passing in language interfacing, 
rather than code bugs induced by C-Fortran interactions. 
Similarly, Hu et al.~\cite{hu2023empirical} identified 9 common bug patterns concerning Python/C API usage. 
%The same authors also developed a call-graph construction approach applied to Python/C and JavaScript/C applications~\cite{hu2023cross}, which is limited to use in IDEs as it relies on IDE capabilities.  
%The recent study~\cite{hwang2024empirical} on language interoperability aims to understand JVM bugs triggered by erroneous Java/C interoperations. 
Our study concerns bugs induced by faulty cross-language information flow, 
including but not limited to those caused by API misuses. 

==> threats-new.tex <==
\subsection{Limitations and Threats to Validity}
%\textbf{Threats to internal validity}. 
Our study relies on several tools for data crawling and filtering, which are subject to implementation errors that may have led to incorrect multilingual bug collection.
%These errors might have lead to incorrect results and findings. 
One mitigating factor is that these tools have either been widely used by fellow researchers and/or in multiple related studies before. 
To further mitigate this threat, we conducted careful code reviews of 
each tool, especially the extension we made, and manually validated their correctness against small test samples. 

Also, our study results are subject to manual labeling/analysis errors and human biases. 
To reduce this threat, we followed a rigorous coding process for describing the 
results for each RQ. 
Moreover, we adopted inter-rater and/or negotiated agreement protocols to 
resolve any diverged decisions, which help reduce human biases 
via cross checking. 

%\textbf{Threats to external validity}
Our study results are based on Python-C projects that met our repository mining criteria. %(e.g., with a threshold number of stars)
These projects may not be representative of all existing real-world Python-C software. Accordingly, the bugs we examined do not necessarily represent all of the bugs across Python and C. 
Thus, our findings and conclusions are only best interpreted against the  
projects and multilingual bugs in them that we have actually studied. 
To mitigate this threat, we considered a sizable number of projects of various domains while using random sampling with statistically significant sample sizes.
On the other hand, the scale of our study is indeed limited by the lack of 
more capable tools and the tedious nature of manual analysis. 

Similarly, we cannot claim that our results generalize to non-Python-C software. Future work may use our methodology but extend our datasets to address other language combinations. 





==> threats.tex <==
%!TEX root = paper.tex

\subsection{Threats to Validity}
\textbf{Threats to internal validity}. 
The code of our tools and models is a critical component in ensuring the validity of our research findings. Despite our efforts to avoid bugs and errors through code reviews, there is still a possibility that undetected bugs could exist in the code. These bugs could affect the performance of the tools and models and lead to incorrect results or findings. 

We depend heavily on manual analysis, and our hand labeling is subject to personal prejudice. To reduce human bias throughout the labeling process, two authors examined the commits and labeled the root cause and bug location independently, with discrepancies discussed until consensus was established. 


\textbf{Threats to external validity} 
We focused on analyzing Python-C projects for our study; our findings may not be generalizable to other language combination projects. However, Python and C are popular languages for developers, and many projects are programmed with the combination of Python - C, so we think it is representative. We encourage future research to investigate the problem via other language combinations. 

Our research results and findings are based on data collected from the top 23 Python-C projects with the most stars. While this data may provide insights into the top-performing projects, it may not represent other Python-C projects that were not included in the analysis. This limited data source potentially threatens the validity of the results. It highlights the need to consider other data sources or criteria when evaluating the generalizability of the findings.
